Implicit Geometry of Next-token Prediction: From Language Sparsity Patterns to Model Representations

Next-token prediction (NTP) over large text corpora has become the go-to paradigm to train large language models. Yet, it remains unclear how NTP influences the mapping of linguistic patterns to geometric properties of the resulting model representations. We frame training of large language models as soft-label classification over sparse probabilistic label vectors, coupled with an analytical approximation that allows unrestricted generation of context embeddings. This approach links NTP training to rank-constrained, nuclear-norm regularized optimization in the logit domain, offering a framework for analyzing the geometry of word and context embeddings. In large embedding spaces, we find that NTP implicitly favors learning logits with a sparse plus low-rank structure. While the sparse component captures the co-occurrence frequency of context-word pairs, the orthogonal low-rank component, which becomes dominant as training progresses, depends solely on the sparsity pattern of the co-occurrence matrix. Consequently, when projected onto an appropriate subspace, representations of contexts that are followed by the same set of next-tokens collapse, a phenomenon we term subspace-collapse. We validate our findings on synthetic and small-scale real language datasets. Finally, we outline potential research directions aimed at deepening the understanding of NTP's influence on the learning of linguistic patterns and regularities.

==> Arxiv_NewTempl/sections/AR-2.tex <==
% \tina{moved from the earlier AR file}
% \begin{definition}
%     The UFM for \textbf{autoregressive} NTP training over training set $\Tc = \{\{\pih_{t,j},\ph_{t,j,z\in\Vc}\}_{j\in[m_t]}\}_{t\in[T-1]}$ refers to the following problem:
%     \begin{align}\label{eq:ufm-ar}
%         \min_{\W,\hd_{t,j}} ~~\left\{ - \sum_{t\in[T-1]}\sum_{j\in[m_t]}\pih_{t,j}\sum_{z\in\Sc_j}\ph_{t,j,z}\log\left(\sfti{z}{\W \hd_{t,j}}\right)\right\}+\la\|\W\|^2 + \la\sum_{t\in[T-1]}\|\Hb_t\|^2,%\tag{NTP-UFM}
%     \end{align}
%     where the minimization is over $\W\in\R^{V\times d}$ and $\Hb_t:=[\hd_{t,1},\ldots,\hd_{t,m_t}]\in\R^{V\times m_t}$. Here, $m_t, t\in[T-1]$ is the number of distinct contexts of size $t$. Note that $m_1\geq m_2 \geq \cdots \geq  m_{T-1}.$ Accordingly, $\hd_{t,j}, t\in[T-1],j\in[m_t]$ is the $j$-th distinct embedding of $t$-long context $\xd_{t}:=(z_1,\ldots,z_t)$.
% \end{definition}

% \new{Note that by renumbering the context embeddings, the AR UFM matches the UFM defined on fixed-length sequences. Specifically, define $m=\sum_{t\in[T-1]} m_t$, and let $\Hb_{d\times m} = [\Hb_1,\cdots,\Hb_{T-1}]$. Then, the objective in  \eqref{eq:ufm-ar} equals the objective in \ref{eq:ufm}. This holds true since UFM assumes the language model is expressive enough to learn approximately uncorrelated embeddings.
% % to efficiently model any mappings from the input to the context embedding space. 
% We hypothesize that as long as the model is large enough, whether training on fixed-length sequences or auto-regressively, the nature of the training remains unchanged, particularly due to teacher-forcing\tina{??} during training. This means that during training, the model always has access to the true history of the context sequence when making predictions for the individual next-token. Thus, as long as the model has adequate expressiveness, a model can be trained to learn different context embeddings for a sequence and any of its partial subsequences, especially when the corresponding support sets (i.e., next tokens) differ significantly. 
% Consequently, the Thms.~\ref{thm:reg path}, \ref{thm:reg path finite} similarly hold for the AR scenario: the structural properties of the data described by $\smat$ and $\Pb$ describe the geometry of the embeddings close to the end of training.}\tina{meh... reads hand wavy}


% \tina{let's add some experiments on AR that works: TF, RNN/LSTM/whatever works}


% \textbf{\ct{the AR definition is too repetitive to go to main body. I think it is kind of obvious that the model extends to AR and ohow. Sure it might not be bad idea to make this explicit, but if so, do in the appendix. Experiments can stay in main body. Regarding the above discussion: ``We hypothesize that as long as the model is large enough, whether training on fixed-length sequences or auto-regressively, the nature of the training remains unchanged, particularly due to teacher-forcing\tina{??} during training.'' hmmmm... what does this mean? It can be missinterpreted. AR nature will reflect to the nature of $\smat$ and prob. mat..}}

==> Arxiv_NewTempl/sections/Lmm_conj.tex <==
\new{In Sec\ref{}, we used $\smat^\top\smat$ and $\smat\smat^\top$ as proxies for the geometric patterns of the optimal context and word embeddings, respectively. We found a high correlation between the Gram matrix of $\smat^\top$ (resp. $\smat$) with that of $\W$ (resp. $\Hb$) empirically in the synthetic setup \ref{}. We then used these heuristic metrics as a reference for the optimal word and context embeddings in our larger-scale experiments of \ref{??}. We relied on this approach because, in our large-scale experiment, calculating the optimal $\Lbmm$ is not feasible, and even if it were, performing the SVD on the optimal logit for recovering the optimal $\W$ and $\Hb$ would be computationally expensive. In contrast, the heuristic metrics $\smat\smat^\top$ and $\smat^\top\smat$ are easier to compute and track. }
% 
{Considering $\Lbtina$, defined in Sec.~\ref{sec:general geometries}, as a close proxy of the optimal solution of \ref{eq:ufm-svm}, we provide a connection between the support sets and embeddings geometry. Suppose $\Lbmm\approx\Lbtina$. Then, by Thm.~\ref{thm:reg path},}

% \citet{seli} verifies Claim \ref{claim:conj} in the special case of one-hot case with STEP-imbalanced training distribution. In other words, in this special case, $\Lbmm = (\Id_V - \ones_V\ones_V^\top)\smat$. Thus, 
\begin{align}
     \Wmm{\Wmm}^\top &= (\Lbmm{\Lbmm}^\top)^{\frac{1}{2}} \approx \Big((\Id_V-\frac1V\ones_V\ones_V^\top)\smat\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\Big)^{\frac{1}{2}},\\
    {\Hmm}^\top\Hmm &= ({\Lbmm}^\top\Lbmm)^{\frac{1}{2}} \approx \Big(\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\smat\Big)^{\frac{1}{2}}.
\end{align}
% 
% \tina{what is the interpretation of $\Wmm{\Wmm}^\top\Wmm{\Wmm}^\top$?}
% In other words,
% \begin{align*}
%      \Wmm{\Wmm}^\top\Wmm{\Wmm}^\top &=  (\Id_V-\ones_V\ones_V^\top)\smat\smat^\top(\Id_V-\ones_V\ones_V^\top)\\
%     {\Hmm}^\top\Hmm{\Hmm}^\top\Hmm &= \smat^\top(\Id_V-\ones_V\ones_V^\top)\smat
% \end{align*}
% 
In other words, the Gram matrix of $\Wmm$ (resp. $\Hmm$) is close to the square root of $\smat\smat^\top$ (resp. $\smat^\top\smat$) after some projection to the subspace orthogonal to $\ones_V$. 
This suggests a heuristic justification for why we observe the high correlations between the embeddings geometry and the sparsity pattern of language in our experiments in Figs.\ref{}.
% \new{Since taking the square root of a matrix, equivalently copmuting its SVD decomposition, is computationally expensive for large matrices, inspired by \eqref{eq:proxy1}, }


% \begin{enumerate}
%     \item This might be the reason behind the high correlation between the Gram matrices of $\Wmm$ and $\Hmm$ with $\smat\smat^\top$ and $\smat^\top\smat$. However, it also shows that it is unreasonable to expect an exact pattern matching between the Gram matrix of $\smat$ and optimal UFM parameters. 

%     \item The conjecture does not hold in general! Figure \ref{fig:L_counterEx} shows one counter-example. The approximate values of the optimal solution is as follows (only shown for the first column:
%     \begin{align*}
%        \begin{bmatrix}
%     0.8618 &
%     0.8618 &
%     -0.1382 &
%     -0.7562 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 
% \end{bmatrix}^\top
%     \end{align*}
% \textbf{Note:} cvxpy solution has lower rank!
% \end{enumerate}





==> Arxiv_NewTempl/sections/Lmm_conj_app.tex <==
\new{In Sec\ref{}, we used $\smat^\top\smat$ and $\smat\smat^\top$ as proxies for the geometric patterns of the optimal context and word embeddings, respectively. We found a high correlation between the Gram matrix of $\smat^\top$ (resp. $\smat$) with that of $\W$ (resp. $\Hb$) empirically in the synthetic setup \ref{}. We then used these heuristic metrics as a reference for the optimal word and context embeddings in our larger-scale experiments of \ref{??}. We relied on this approach because, in our large-scale experiment, calculating the optimal $\Lbmm$ is not feasible, and even if it were, performing the SVD on the optimal logit for recovering the optimal $\W$ and $\Hb$ would be computationally expensive. In contrast, the heuristic metrics $\smat\smat^\top$ and $\smat^\top\smat$ are easier to compute and track. }
% 
{Considering $\Lbtina$, defined in Sec.~\ref{sec:general geometries}, as a close proxy of the optimal solution of \ref{eq:ufm-svm}, we provide a connection between the support sets and embeddings geometry. Suppose $\Lbmm\approx\Lbtina$. Then, by Thm.~\ref{thm:reg path},}

% \citet{seli} verifies Claim \ref{claim:conj} in the special case of one-hot case with STEP-imbalanced training distribution. In other words, in this special case, $\Lbmm = (\Id_V - \ones_V\ones_V^\top)\smat$. Thus, 
\begin{align}
     \Wmm{\Wmm}^\top &= (\Lbmm{\Lbmm}^\top)^{\frac{1}{2}} \approx \Big((\Id_V-\frac1V\ones_V\ones_V^\top)\smat\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\Big)^{\frac{1}{2}},\\
    {\Hmm}^\top\Hmm &= ({\Lbmm}^\top\Lbmm)^{\frac{1}{2}} \approx \Big(\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\smat\Big)^{\frac{1}{2}}.
\end{align}
% 
% \tina{what is the interpretation of $\Wmm{\Wmm}^\top\Wmm{\Wmm}^\top$?}
% In other words,
% \begin{align*}
%      \Wmm{\Wmm}^\top\Wmm{\Wmm}^\top &=  (\Id_V-\ones_V\ones_V^\top)\smat\smat^\top(\Id_V-\ones_V\ones_V^\top)\\
%     {\Hmm}^\top\Hmm{\Hmm}^\top\Hmm &= \smat^\top(\Id_V-\ones_V\ones_V^\top)\smat
% \end{align*}
% 
In other words, the Gram matrix of $\Wmm$ (resp. $\Hmm$) is close to the square root of $\smat\smat^\top$ (resp. $\smat^\top\smat$) after some projection to the subspace orthogonal to $\ones_V$. 
This suggests a heuristic justification for why we observe the high correlations between the embeddings geometry and the sparsity pattern of language in our experiments in Figs.\ref{}.
% \new{Since taking the square root of a matrix, equivalently copmuting its SVD decomposition, is computationally expensive for large matrices, inspired by \eqref{eq:proxy1}, }


% \begin{enumerate}
%     \item This might be the reason behind the high correlation between the Gram matrices of $\Wmm$ and $\Hmm$ with $\smat\smat^\top$ and $\smat^\top\smat$. However, it also shows that it is unreasonable to expect an exact pattern matching between the Gram matrix of $\smat$ and optimal UFM parameters. 

%     \item The conjecture does not hold in general! Figure \ref{fig:L_counterEx} shows one counter-example. The approximate values of the optimal solution is as follows (only shown for the first column:
%     \begin{align*}
%        \begin{bmatrix}
%     0.8618 &
%     0.8618 &
%     -0.1382 &
%     -0.7562 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 &
%     -0.1382 
% \end{bmatrix}^\top
%     \end{align*}
% \textbf{Note:} cvxpy solution has lower rank!
% \end{enumerate}





==> Arxiv_NewTempl/sections/Lmmprops.tex <==
% \subsection{On the solution of \texorpdfstring{\ref{eq:ufm-svm}}{NTP-SVM*}}
% \ct{change framing and call it something like: on the structure of $\Lbmm$}
% \vspace{-0.05in}
% 
\tina{edit this if decided to keep some parts in the main body} To better understand how the SVD factorization informs the geometry, we investigate further how the structure of $\Lbmm$ (solution to \ref{eq:ufm-svm}) depends on the support matrix $\Sb$.
% \vspace{-0.1in}

\subsection{Special case: support sets of equal sizes}
% \vspace{-0.05in}
\begin{proposition}\label{prop:all symmetric geometry}
    Fix $k\in[V-1]$ and suppose $\smat$ contains all $m={V\choose k}$ support sets of size $k$.  Then,
    \begin{enumerate}[noitemsep,leftmargin=*]
       % \setlength{\itemindent}{-2em}
       % \vspace{-0.15in}
        \item[(i)] The logit matrix takes the form $\Lbmm=(\Id_V-\frac{1}{V}\ones\ones^\top)\Sb$.
        %
        \item[(ii)] Word embeddings form equiangular tight frame (ETF) being equinorm and maximally separated. 
        %
        \item[(iii)] Context embeddings are equinorm and the embedding $\hb_j$ of context $j$ is co-linear to $\sum_{z\in\Sc_j}\w_z$.
    \end{enumerate}
\end{proposition}

In the symmetric setting of the proposition, we can analytically solve \ref{eq:ufm-svm} giving $\Lbmm$ as expressed in the statement (i). In fact, it is possible to obtain an explicit characterization of the SVD of $\Lbmm$, which enables the precise definition of embeddings' geometries in statements (ii) and (iii). This explicit characterization leads to closed-form formulas for the angles and norms of embeddings, detailed in Prop.~\ref{prop:sym geo app}. 

\begin{proposition}\label{prop:sym geo app}
       Assume the setting of Proposition \ref{prop:all symmetric geometry}. The geometry of context and word embeddings  is described by the following relations:
    \begin{subequations}
    \begin{align}
        \forall v\neq v'\in[V]\,&:\,\cosa{\w_v}{\w_{v'}} = \frac{-1}{V-1} \quad\text{and}\quad \|\w_v\|=\|\w_{v'}\|
        \\
        \forall j\neq j'\in[m]\,&:\,\cosa{\hb_j}{\hb_{j'}}=\frac{|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}}{k-\frac{k^2}{V}}\quad\text{and}\quad \|\hb_j\|=\|\hb_{j'}\|
        \\
        \forall j\in[m], v\in[V]\,&:\
        \cosa{\w_v}{\hb_j} = \begin{cases}
    \sqrt{\frac{V-1}{k(V-k)}} & v\in\Sc_j\\
     \frac{-1}{\sqrt{k(V-k)(V-1)}} & v\notin\Sc_j
    \end{cases}\,
    \\
    \forall j\in[m], v\in[V]\,&:\ \frac{\|\w_v\|^2}{\|\hb_j\|^2} = \frac{(V-1)\,\binom{V-2}{k-1}}{k(V-k)}\,.
    \end{align}
    \end{subequations}
\end{proposition}


\begin{figure}[t]
    \centering 
    \includegraphics[width=0.7\linewidth]{figures/symmetric_geo_w_h.eps}  
\captionsetup{width=\textwidth}
    \caption{Geometry properties illustration for Proposition \ref{prop:all symmetric geometry}. Shown two values of $V$ for varying values of $k\in[V-1]$. (Left) angles between context and word embeddings. (Right) normalized norm ratio of word to context embeddings.}
    \label{fig:symmetric_geo}
\end{figure}


For $k=1$ these formulas recover the ETF geometry that has been previously shown for the setting of one-hot classification \citep{NC}. For general $k>1$, word embeddings continue forming an ETF, but the geometry of context embeddings changes although they remain equinorm. Embedding $\hb_j$ forms the same \emph{acute} angle with all in-support word vectors $\w_v, v\in\Sc_j$ and  the same \emph{obtuse} angle with all out-of-support word vectors $\w_v, v\notin\Sc_j$.  Additionally, for $k>1$, norms of word embedddings become larger than norms of context embeddings. See also Fig.~\ref{fig:symmetric_geo} for a visualization of these properties. \new{We defer the proof of these two propositions to Sec.~\ref{sec:props_proof}.}




% \vspace{-0.05in}
\subsection{A simple candidate solution}\label{sec:general geometries}
 Generally, achieving an analytic expression for $\Lbmm$, as was possible in Prop. \ref{prop:all symmetric geometry}, might not always be feasible. This challenge primarily arises from the combinatorial complexity of the constraints that adhere to the sparsity pattern of $\Sb$. To mitigate this issue and potentially circumvent the need to solve the semidefinite program in \ref{eq:ufm-svm}—which becomes computationally intensive for large $V$ and $m$—we introduce a strategy that allows for a numerical verification of whether a given simple matrix solves \ref{eq:ufm-svm}.
The matrix we propose, inspired by Prop. \ref{prop:all symmetric geometry}, is defined as follows: %$\Lbtina[z,j]=1-|\Sc_j|/V$ if $z\in\Sc_j$, and $\Lbtina[z,j]=-|\Sc_j|/V$ if $z\notin\Sc_j$.
% $
%         \Lbmm = \big(\Id_V-\frac{1}{V}\ones\ones^\top\big)\smat\,.
%     $
% Consequently, the logits are determined by 
\begin{align}\label{eq:Lmm explicit}
    \Lbtina[z,j] = \begin{cases}
        1-|\Sc_j|/V, & z\in\Sc_j\,\\
            -{|\Sc_j|}/{V}, & z\not\in\Sc_j\,
        \end{cases}
        \,.
    \end{align}
 $\Lbtina$ readily satisfies the feasibility conditions for \ref{eq:ufm-svm}, meeting all inequality constraints with equality. %\tina{-}Our empirical evaluations indicate that it successfully solves \ref{eq:ufm-svm} in numerous  realizations of $\Sb$ we have examined. 
 Below, we further introduce a dual-certificate condition that, when fulfilled by $\Lbtina$, ensures optimality. \looseness=-1 %The details of this condition are articulated in Proposition \ref{propo:svm sufficient condition}.
\begin{proposition}\label{propo:svm sufficient condition}
    Let $\Lbtina=\Ub\Sigmab\Vb^\top$ denote the SVD of $\Lbtina=(\Id_V-\frac{1}{V}\ones\ones^\top)\smat$. Define, $\Ab:=\Ub\Vb^\top$. If $\forall j \in [m]$ and all $v\not\in\Sc_j$, it holds that  $\Ab[v,j]< 0$, then $\Lbtina$ solves \eqref{eq:ufm-svm}.
\end{proposition}
%The proposed certificate is applicable to any potential solution matrix. However, we particularly recommend the specific form in \eqref{eq:Lmm explicit} as a straightforward and frequently effective option. Additionally, 
Verifying the certificate's conditions only requires an SVD of $\Lbtina$. In situations where these SVD factors can be analytically determined, the certificate also enables a formal proof of optimality. For example, this approach is used in the proof of Prop. \ref{prop:all symmetric geometry} in Sec.~\ref{sec:props_proof}. 

\new{Whether $\Lbtina$ satisfies the dual certificate in Prop.~\ref{propo:svm sufficient condition} or not, and thus its optimality, depends on the language conditional distribution as encoded in the sparsity pattern of $\Sb$. Our empirical evaluations show that $\Lbtina$ successfully solves \ref{eq:ufm-svm} in numerous  realizations of $\Sb$ we have examined. However, this solution is not guaranteed to be optimal in all cases. In Fig.~\ref{fig:L_counterEx}, we present an example of two realizations of $\Sb$, where the condition in Prop.~\ref{propo:svm sufficient condition} is met in one instance but not in the other. The second and third column of the figure display the heatmap of $\Lbtina$ and the optimal solution of \ref{eq:ufm-svm} as determined by CVXPY \citep{cvx} for the support sets $\Sb$ shown in the first column. Notably, although $\Lbtina$ is not optimal in the second row, it provides a close and simple approximation of the optimal $\Lbmm$. Additionally, in Fig.~\ref{fig:L_conj_synthetic}, we show similar heatmaps of the optimal logits for the synthetic setup of Sec.~\ref{}. Once again, while $\Lbtina$ is not necessarily optimal, it serves as a close proxy for the optimal solution.} \tina{Note that in the case of one-hot classification under STEP imbalanced data, \citet{seli} had previously proved that $\Lbtina$ is the unique minimizer of \ref{eq:ufm-svm}.}

% \tina{worth mentioning that cvxpy solution has lower rank?}
% \ct{motivate the conjecture based on the prop above for the symmetric case}
% \begin{conjecture}\label{conj:Lmm}
%     The optimal solution of \eqref{eq:ufm-svm} is given as follows in terms of the support matrix $\smat\in\{0,1\}^{V\times m}$:
%     \begin{align}\label{eq:Lmm explicit}
%     \Lbmm [j,z] = \begin{cases}
%         1-|\Sc_j|/V, & z\in\Sc_j\,\\
%             -{|\Sc_j|}/{V}, & z\not\in\Sc_j\,
%         \end{cases}
%         \,.
%     \end{align}
%     That is, in matrix form: $
%         \Lbmm = \left(\Id_V-\frac{1}{V}\ones\ones^\top\right)\smat\,.
%     $
% \end{conjecture}
% \tina{check the counter example}




% 1. The diagonal element contributes \( k \) to the sum.

% 2. Each off-diagonal element corresponds to the inner product of two different columns of $\smat$, which equals the size $r$ of the intersections of the support sets that they represent and ranges from $1$ to $k-1$. Now, for each \( r \), the number of support sets that share exactly \( r \) elements with a given set is \( \binom{k}{r} \binom{V-k}{k-r} \).

% Thus, the sum of the entries of a column in \( S'S \) can be expressed as:
% \[
%  k + \sum_{r=1}^{k-1} r \binom{k}{r} \binom{V-k}{k-r} = \frac{k \,(V-1)!}{(k-1)! \,(V - k)!}\,.
% \]





\begin{figure*}[t]
	\vspace{-0pt}
	\centering
	\hspace{-7pt} 
 \begin{subfigure}{0.9\textwidth}
		\centering
		\begin{tikzpicture}
		% \node at (-0,-0) {\includegraphics[scale=0.35]{figures/Lconjecture.png}};
  \node at (-0,0){\includegraphics[scale=0.35]{figures/Lmmconj_Ex5.pdf}};
  \node at (-5.3,1.3) [scale=0.7]{$\Sb$};
    \node at (-0,1.3) [scale=0.7]{$\Lbtina$};
        \node at (4.8,1.3) [scale=0.7]{$\Lb_\text{CVXPY}$};
		\end{tikzpicture}
    \end{subfigure}

 \vspace{-10pt}
 \begin{subfigure}{0.9\textwidth}
		\centering
		\begin{tikzpicture}
		% \node at (-0,-0) {\includegraphics[scale=0.35]{figures/Lconjecture.png}};
  \node at (-0,0){\includegraphics[scale=0.35]{figures/Lmmconj_counterEx2.pdf}};
		\end{tikzpicture}
    \end{subfigure}
 \captionsetup{width=\linewidth}
 \vspace{-5pt}
    \caption{Comparison between the solution found by CVXPY for \ref{eq:ufm-svm} and $\Lbtina$ defined in Sec.~\ref{sec:general geometries} for two realizations of the support set matrix $\Sb$. See text for details.
     }\label{fig:L_counterEx}
	\vspace{-15pt}
\end{figure*}




\begin{figure*}[t]
	\vspace{-0pt}
	\centering
	\hspace{-180pt} 
 \begin{subfigure}{0.9\textwidth}
		\centering
		\begin{tikzpicture}
		% \node at (-0,-0) {\includegraphics[scale=0.35]{figures/Lconjecture.png}};
  \node at (-0,0){\includegraphics[scale=0.45]{figures/S_L_mm_cvxpy_thm_tiny_extract_m404.pdf}};
  \node at (-5.8,.7) [scale=0.7]{$\Sb$};
    \node at (-0.3,0.7) [scale=0.7]{$\Lbtina$};
        \node at (5.3,0.7) [scale=0.7]{$\Lb_\text{CVXPY}$};
		\end{tikzpicture}
    \end{subfigure}
 \captionsetup{width=\linewidth}
 \vspace{-5pt}
    \caption{Same as Fig.~\ref{fig:L_counterEx} for the support set configuration in synthetic experiment of Sec.~\ref{}.
     }\label{fig:L_conj_synthetic}
	\vspace{-15pt}
\end{figure*}


\subsection{{Relationship between word/context embeddings geometry and support set}}
\tina{section or paragraph?}
\input{Arxiv/sections/Lmm_conj}



\subsection{Proof of Proposition \ref{propo:svm sufficient condition}}
% \tina{we haven't defined the non-convex svm anywhere else ig}
% 

To prove the proposition, we first derive the dual of \ref{eq:ufm-svm}. 

We begin with a more convenient, but equivalent, formulation of \ref{eq:ufm-svm}. One way to do this is by recalling that \ref{eq:ufm-svm} is a convex relaxation to 
\begin{align*}
    \min_{\W,\Hb} \frac{1}{2}\norm{\W}_F^2 + \frac{1}{2}\norm{\Hb}_F^2, \quad \text{s.t.} \quad \forall j\in[m], z_j\neq z\in\Sc_j~&:~~(\eb_{z_j}-\eb_{z'})^\top\W \hb_j =0\,
        \\
        \forall j\in[m], v\notin\Sc_j~&:~~(\eb_{z_j}-\eb_{v})^\top\W \hb_j \geq 1\,.
\end{align*}
where, for each sample $j$, we choose an anchor label $z_j\in\Sc_j$. We can now relax this in terms of the matrix $\Xb = \begin{bmatrix}
    \W\\
    \Hb^\top
\end{bmatrix}\begin{bmatrix}
    \W^\top & \Hb
\end{bmatrix}$. (Note that $\Lb$ essentially corresponds to the off-diagonal blocks of $\X$.).
This gives us the following reformulation of \ref{eq:ufm-svm} (Formally, it is easy to show that \eqref{eq:svm X formulation} is the dual of the dual of \ref{eq:ufm-svm}. This result about nuclear minimization is classic (e.g., \cite{RechtFazel}) and we omit the details.):
\begin{align}\label{eq:svm X formulation}
    \min_{\Xb\succcurlyeq0}\,\, \frac{1}{2}\tr(\Xb)\quad \text{s.t.}\quad \forall j\in[m], z_j\neq z\in\Sc_j~&:~~\Xb[z_j,V+j] - \Xb[z',V+j] =0\,
        \\
        \forall j\in[m], v\notin\Sc_j~&:~~\Xb[z_j,V+j] - \Xb[v,V+j] \geq 1\,. \nn
\end{align}

Define $\Ab_{V\times m}$ such that $\Ab[z,j] = -\lambdab_{j,z},\,z\neq z_j$ and $\Ab[z_j,j] = \sum_{z\neq z_j}\lambdab_{j,z}$. ($\oneb_V^\top\Ab=0$).

The dual problem is 
\begin{align*}
&
\max_{\Ab} \,\min_{\Xb\succcurlyeq0} \,\sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} + \frac12\tr\bigg(\begin{bmatrix}
    \Id & -\Ab\\
    -\Ab^\top & \Id 
\end{bmatrix}\Xb\bigg)\,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad \Ab[v,j]\leq0,\,v\not\in\Sc_j\\
=&\max_{\Ab} \,\sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} \,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad {\Ab[v,j]\leq0,\,v\not\in\Sc_j},\quad \norm{\Ab}_2\leq 1\\
=&\max_{\Ab} \,\,\tr(\Ab^\top\Lbtina) \,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad {\Ab[v,j]\leq0,\,v\not\in\Sc_j},\quad \norm{\Ab}_2\leq 1
\end{align*}
%\tina{for $|\Sc_j|=1$ boils down to $\Ab \odot \Lbmm \geq 0$ similar to what we had before.}
% 
where here $\Lbtina=(\Id_V-\frac{1}{V}\ones_V\ones_V^\top)\smat$ is the matrix we defined in Sec.~\ref{sec:general geometries}. The last line above holds since,
\begin{align*}
    \sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} &= \sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v} - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
    &= \sum_{j\in[m]}\sum_{v\neq z_j}\lambdab_{j,v} - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
    &= \sum_{j\in[m]} (\frac{1-|\Sc_j|}{V} + \frac{|\Sc_j|}{V}) \sum_{v\neq z_j}\lambdab_{j,v}  - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
    &= \sum_{j\in[m]} \frac{1-|\Sc_j|}{V} \Ab[z_j,j] - \sum_{j\in[m]} \frac{|\Sc_j|}{V} \sum_{v\neq z_j} \Ab[v,j] + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\Ab[v,j]\\
    &= \sum_{j\in[m]} \Lbtina[z_j,j] \Ab[z_j,j] + \sum_{j\in[m]} \sum_{v\not\in\Sc_j} \Lbtina[v,j]  \Ab[v,j] + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\Lbtina[v,j] \Ab[v,j]\\
    &=\sum_{j\in[m]} \sum_{v\in[V]}\Lbtina[v,j] \Ab[v,j]\,.
\end{align*}

We remark the following about the dual problem derived above. First, because $\Lbtina$ is feasible in \eqref{eq:ufm-svm} and constraints are linear, Slater's conditions hold, thus, we have strong duality. Second, by complementary slackness, if the nonegativity conditions $\Ab[v,j]\leq0, v\notin\Sc_j$ are strict, then, at optimality, $\Lb$ satisfies the inequality constraints \eqref{eq:svm inequalities} with equality. 

Now, regarding solving the dual, observe that if we remove the constraint $\Ab[v,j]\leq0, v\notin\Sc_j$, then the solution to the dual is simply $\Ab=\Ub\Vb^\top$ where $\Ub\Sigmab\Vb^\top$ is the SVD of $\Lbtina$. In fact, it is not hard to show that this is the unique solution of the relaxed dual; see for example \cite[Lemma C.1]{seli} for an analogous result. Therefore, if $\Ub\Vb^\top$ satisfies the condition of the proposition, then it is clearly the unique optimal solution to the dual problem. 

From this and complementary slackness discussed above, it must be that any minimizer of \eqref{eq:ufm-svm} must satisfy the inequality constraints with equalities. Formally, the optimal solution $\hat\Lb$ satisfies simultaneously:
\[
\hat\Lb^\top\ones_V=0_m\quad\text{and}\quad \forall j\in[m]: \Ebin{j}\hat\ellbb_j=\ones_{S_j},\,\, ~\Ebout{j}\hat\ellbb_j=0_{V-1-S_J}.
\]
Note that this is a system of $m+\sum_{j\in[m]}(S_j+V-1-S_j)=Vm$ linear equations. It can also be easily verified that these equations are linearly independent. Thus, their unique solution is $\Lbtina$. This completes the proof of the proposition.

% \ct{proof needs to be completed}
% \begin{proposition}\label{propo:svm sufficient condition}
%     Let $\Lbmm=\Ub\Sigmab\Vb^\top$ be the SVD of $\Lbmm$ and define $\bar{\Ab}:=\Ub\Vb^\top$. If $\forall j \in [m]$, $v\not\in\Sc_j$,  we have  $\Ab[v,j]\leq0,\,$, Then, 
% \end{proposition}




%-----------------------------
% To prove Prop.~\ref{propo:svm sufficient condition}, we focus on the non-convex counter-part of the \ref{eq:ufm-svm} below: 
% \begin{align*}
%     \min_{\W,\Hb} \frac{1}{2}\norm{\W}_F^2 + \frac{1}{2}\norm{\Hb}_F^2, \quad \text{s.t.} \quad \forall j\in[m], z\neq z'\in\Sc_j~&:~~(\eb_z-\eb_{z'})^\top\W \hb_j =0\,
%         \\
%         \forall j\in[m], v\notin\Sc_j~&:~~(\eb_z-\eb_{v})^\top\W \hb_j \geq 1\,.
% \end{align*}
% % 
% For each sample $j$, choose an anchor label $z_j\in\Sc_j$. We can then re-write the above program as, 
% \begin{align*}
%     \min_{\W,\Hb} \frac{1}{2}\norm{\W}_F^2 + \frac{1}{2}\norm{\Hb}_F^2, \quad \text{s.t.} \quad \forall j\in[m], z_j\neq z\in\Sc_j~&:~~(\eb_{z_j}-\eb_{z'})^\top\W \hb_j =0\,
%         \\
%         \forall j\in[m], v\notin\Sc_j~&:~~(\eb_{z_j}-\eb_{v})^\top\W \hb_j \geq 1\,.
% \end{align*}
% % 
% Let $\Xb = \begin{bmatrix}
%     \W\\
%     \Hb^\top
% \end{bmatrix}\begin{bmatrix}
%     \W^\top & \Hb
% \end{bmatrix}$ and consider the following convex relaxation of the above program,
% \begin{align*}
%     \min_{\Xb\succcurlyeq0}\,\, \frac{1}{2}\tr(\Xb)\quad \text{s.t.}\quad \forall j\in[m], z_j\neq z\in\Sc_j~&:~~\Xb[z_j,V+j] - \Xb[z',V+j] =0\,
%         \\
%         \forall j\in[m], v\notin\Sc_j~&:~~\Xb[z_j,V+j] - \Xb[v,V+j] \geq 1\,. 
% \end{align*}
% % 
% Define $\Ab_{V\times m}$ such that $\Ab[z,j] = -\lambdab_{j,z},\,z\neq z_j$ and $\Ab[z_j,j] = \sum_{z\neq z_j}\lambdab_{j,z}$. Note that $\oneb_V^\top\Ab=0$. Then, we can express the dual problem as follows,
% \begin{align*}
% &
% \max_{\Ab} \,\min_{\Xb\succcurlyeq0} \,\sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} + \frac12\tr\bigg(\begin{bmatrix}
%     \Id & -\Ab\\
%     -\Ab^\top & \Id 
% \end{bmatrix}\Xb\bigg)\,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad \Ab_{j,v}\leq0,\,v\not\in\Sc_j\\
% =&\max_{\Ab} \,\sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} \,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad {\Ab_{j,v}\leq0,\,v\not\in\Sc_j},\quad \norm{\Ab}_2\leq 1\\
% =&\max_{\Ab} \,\,\tr(\Ab^\top\Lbmm) \,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad {\Ab_{j,v}\leq0,\,v\not\in\Sc_j},\quad \norm{\Ab}_2\leq 1
% \end{align*}
% % \tina{for $|\Sc_j|=1$ boils down to $\Ab \odot \Lbmm \geq 0$ similar to what we had before.}
% % 
% The last equality holds since,
% \begin{align*}
%     \sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} &= \sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v} - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
%     &= \sum_{j\in[m]}\sum_{v\neq z_j}\lambdab_{j,v} - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
%     &= \sum_{j\in[m]} (\frac{1-|\Sc_j|}{V} + \frac{|\Sc_j|}{V}) \sum_{v\neq z_j}\lambdab_{j,v}  - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
%     &= \sum_{j\in[m]} \frac{1-|\Sc_j|}{V} \Ab[z_j,j] - \sum_{j\in[m]} \frac{|\Sc_j|}{V} \sum_{v\neq z_j} \Ab[v,j] + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\Ab[v,j]\\
%     &= \sum_{j\in[m]} \Lbmm[z_j,j] \Ab[z_j,j] + \sum_{j\in[m]} \sum_{v\not\in\Sc_j} \Lbmm[v,j]  \Ab[v,j] + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\Lbmm[v,j] \Ab[v,j]\\
%     &=\sum_{j\in[m]} \sum_{v\in[V]}\Lbmm[v,j] \Ab[v,j]
% \end{align*}

% \tina{comp slackness: explain}

% \begin{proposition}\label{propo:svm sufficient condition}
%     Let $\Lbmm=\Ub\Sigmab\Vb^\top$ be the SVD of $\Lbmm$ and define $\bar{\Ab}:=\Ub\Vb^\top$. If $\forall j \in [m]$, $v\not\in\Sc_j$,  we have  $\Ab_{j,v}\leq0,\,$, Then, 
% \end{proposition}
%--------------------------



\subsection{Proof of Propositions \ref{prop:all symmetric geometry} and \ref{prop:sym geo app}} \label{sec:props_proof}
At the heart of proving both Propositions \ref{prop:all symmetric geometry} and \ref{prop:sym geo app} is the following result, which determines the SVD factors $\Ub$, $\Sigmab$, and $\Vb$ of $\Lbtina=(\Id_V-\frac{1}{V}\ones\ones^\top)\Sb$. This shows immediately that word embeddings form an ETF. It also forms the basis for computing the geometry of context embeddings. We show this after proving the lemma.
\begin{lemma}
Fix any $k\in[V]$ and suppose $\smat$ contains all $V\choose k$ support sets of size $k$, i.e. $m={V\choose k}$. Let $\Pbb\in\R^{V\times (V-1)}$ be orthonormal basis of the subspace orthogonal to $\ones_V$. Then, the $\Ub,\Sigmab$ factors of the SVD of $\Lbtina$ are:
$\Ub=\Pbb$ and $\Sigmab=\sqrt{\binom{V-2}{k-1}}\,\Id_{V-1}$. Thus,
\[
\Ub\Sigmab\Ub^\top \propto \Big(\Id_V-\frac{1}{V}\ones\ones^\top\Big)\,.
\]
Moreover, the matrix $\Vb\in\R^{m\times(V-1)}$ of right-singular vectors is such that its rows $\vb_j, j\in[m]$ can be expressed as follows with respect to the rows $\ub_z, z\in[V]$ of $\Ub$:
\[
\vb_j = \frac{1}{\sqrt{\binom{V-2}{k-1}}}\sum_{z\in\Sc_j}\ub_z\,~~j\in[m].
\]
\end{lemma}
\begin{proof}
    We will compute explicitly $\Lbtina{\Lbtina}^\top$. Start with computing $\smat\smat^\top$.  For diagonal elements,  the dot product is between a row of $\smat$ and itself, counts the number of $1$s in that row. Since each element is included in $\binom{V-1}{k-1}$ support sets (choosing the remaining $k-1$ elements from the other $V-1$ elements), each diagonal entry of $\smat\smat^\top$ is $\binom{V-1}{k-1}$. For off-diagonal elements, the dot product counts the number of support sets in which both elements of the corresponding rows appear. This requires choosing the remaining $k-2$ elements from  $V-2$ elements, giving $\binom{V-2}{k-2}$ for each off-diagonal entry of $\smat\smat'$. Overall, after algebraic simplification, we find that
    \[
    \smat\smat^\top = \binom{V-2}{k-1}\left(\Id_V+\frac{k-1}{V-k}\ones\ones^\top\right)\,.
    \]
    We may now use the closed form of $\Lbtina$ and few more algebra simplifications to find that
    \[
    \Lbtina{\Lbtina}^\top=\binom{V-2}{k-1}\left(\Id_V-\frac{1}{V}\ones\ones^\top\right)\,.
    \]
    Let $\Pbb\in\R^{V\times (V-1)}$ denote an orthonormal basis of the subspace orthogonal to $\ones_V$. Since $ \Lbtina{\Lbtina}^\top=\binom{V-2}{k-1}\Pbb\Pbb^\top$ and $\Lbtina{\Lbtina}^\top=\Ub\Sigmab^2\Ub^\top$, we have shown that $\Ub=\Pbb$ and $\Sigmab=\sqrt{\binom{V-2}{k-1}}\,\Id_V$.
\end{proof}

Using $\ones^\top\smat=k$, we can compute
\[
\Lbtina{\Lbtina}^\top=\smat^\top\smat-\frac{1}{V}(\smat^\top\ones_V)(\smat^\top\ones_V)^\top = \smat^\top\smat-\frac{k^2}{V}\ones_m\ones_m^\top\,.
\]
From this and the fact that $\diag{\smat^\top\smat}=k\Id_m$, and recalling that $\Lbtina{\Lbtina}^\top=\Vb\Sigmab^2\Vb^\top$,  we find that all context embeddings are equinorm with squared norm (i.e. diagonal entries of $\Vb\Sigmab\Vb^\top$) equal to 
\[
\|\hb_j\|^2= \frac{k-\frac{k^2}{V}}{\sqrt{\binom{V-2}{k-1}}},\,\,\forall j\in[m].
\]
Recall also that the diagonal entries of $\Ub\Sigmab\Ub^\top$ are
\[
\|\w_v\|^2= \left(1-\frac{1}{V}\right)\sqrt{\binom{V-2}{k-1}},\,\,\forall v\in[V].
\]

From the off-diagonal entries of $\Lbtina{\Lbtina}^\top$, we can infer the angles between different context embeddings. Let $j\neq j'\in[m]$, then the $(j,j')$ of $\Lbtina{\Lbtina}^\top$ is $|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}$. Thus, the  $(j,j')$ off-diagonal entries of $\Vb\Sigmab\Vb^\top$ are \[ \hb_j^\top\hb_{j'}=\frac{|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}}{\sqrt{\binom{V-2}{k-1}}}\implies \cosa{\hb_j}{\hb_{j'}}=\frac{|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}}{k-\frac{k^2}{V}}\,\,\,j\neq j'\in[m]\,.
\]


Recalling that $\W\Hb^\top=\Lbmm$, we may now compute the angle between word and context embeddings as follows:
\begin{align}
    \cosa{\w_v}{\hb_j} = \begin{cases}
    \sqrt{\frac{V-1}{k(V-k)}} & v\in\Sc_j\\
     \frac{-1}{\sqrt{k(V-k)(V-1)}} & v\notin\Sc_j
    \end{cases}\,.
\end{align}
This completes the proof of Proposition \ref{prop:sym geo app} and the proof of statements (ii) and (iii) of Proposition \ref{prop:all symmetric geometry}.

It remains to prove statement (i) of Proposition \ref{prop:all symmetric geometry}, i.e. proving that $\Lbtina=(\Id_V-\frac{1}{V}\ones\ones^\top)\Sb$ is the unique minimizer of \eqref{eq:ufm-svm}.

To prove this, we appeal to Proposition \ref{propo:svm sufficient condition}. First, it is straightforward checking that $\Lbmm$ satisfies the SVM constraints (in fact, with equality). Thus, from Proposition \ref{propo:svm sufficient condition}, it suffices that the matrix $\A:=\Ub\Vb^\top$ satisfies $\A[v,j]<0$ for all $v\notin\Sc_j$ and all $j\in[m]$. But, in our case $\Ab=\Ub\Vb^\top=\binom{V-2}{k-1}^{-\frac{1}{2}}\Lbtina$ because $\Sigmab=\Id_{V-1}$. Thus, the desired condition holds for $\A$ since $\Lbtina[v,j]=-k/V<0$ for all $j\notin\Sc_j$ and $j\in[m]$.

% \tina{where dual certificate is discussed? proof should comeafter that}





==> Arxiv_NewTempl/sections/ToDo.tex <==
\section{To-do}
\begin{enumerate}
    \item \textbf{UFM analysis:}~
    \begin{enumerate}
        \item UFM experiments. 
        \begin{enumerate}
            \item \textbf{@Tina} Check whether the conjecture holds (esp. the subspace part)
        \end{enumerate}
        \item UFM theory.~
        \begin{enumerate}
            \item Proof of conjecture \tina{probably boils down to general imbalance setup which is sad} \ct{or super exciting! :) before we were saying solving that problem is not worth it. now you have a new strong motivation for it! But let's also think of ways to possibly avoid going there, e.g. by normalization/relu. In either case, let's leave proof to later. For now a conjecture/claim that we can strongly support with experiments is already excellent}
            \item What about adding activation (ReLU)/normalization to the model (What do LLMs have in the final layer)? Does it make the analysis easier?
            \item UFM for AR: possible? how should it change?
        \end{enumerate}
    \end{enumerate}
    \item \textbf{Experiments:}
    \begin{enumerate}
        \item (Of lower importance but nice if it works): convergence of soft-label image classification to theory?
        \item (More important since we need to eventually make clear connections to language): Language Experiments -- emphasis on \textbf{last}-token training/prediction for now
        \begin{enumerate}
            \item \textit{Dataset:}~Experimental setup on 1) synthetic (like what Yize has right now), 2) small language datasets (like the ones on the blog post).
            \begin{enumerate}
                \item Can we make the synthetic dataset more diverse? For example: the last-token having various type of grammatical roles (or whatever makes sense). Hope: can we see a kind of grammatical grouping in the embedding space?
                \item In the theory, we need at least $d \text{ (embedding dim) } \geq V\text{ (vocab size) }$. Need to either adjust the tokenizer or use large (impractical) $d$.
            \end{enumerate}
            \item \textit{Stuff to check:}
            \begin{enumerate}
                \item empirical entropy: is it large enough? (If too close to zero, then we are not diverging from the hard-label setup significantly.) Has anyone computed \textbf{token-level} entropy of language? (the ones on the blog post are word-level and character-level)\\
                We should probably go with \textbf{small context window} so that entropy is not very small...
                \item loss converging to empirical entropy 
                \item W norm increasing
                \item convergence to whatever UFM says
                \item what is collapse here?
                \item Is there anything we can check on pre-trained LLMs? (note: they are probably still not in the regime where loss is close to language entropy)
            \end{enumerate}
        \end{enumerate}
    \end{enumerate}

    \item \textbf{Connections to AR/Beyond soft-labels:}
    \begin{enumerate}
        \item How should we think of AR? What is specific to language/sequential data in all this story? 
        \item To check empirically. Take a pre-trained LLM with their corresponding training set: Do the final embeddings of the over-lapping subsequences have high correlation (irrespective of their next token)? Or do we see high correlation only for subsequences which have similar next tokens (class-wise collapse)? 
        \item 
    \end{enumerate}
    
\end{enumerate}


==> Arxiv_NewTempl/sections/additional_exps.tex <==
\pagebreak
\section{Additional Experiments for camera ready}
\tina{@Yize: get rid of this section when figures moved}
\subsection{Experiments}
\subsubsection{Sim(H,H) with context labels(appendix)}
To demonstrate the connection between geometries of context embeddings and semantic meanings, we include the labeled pairwise similarity matrix for smaller-scale datasets. (Figure \ref{fig:sim_H_lable_404}, \ref{fig:sim_H_label_verysmall})
For example, in our synthetic setting(Figure \ref{fig:sim_H_label_verysmall}), we show higher similarities between the embedding of "Lily was playing with her" and "lily spent time with her". \yz{should I include S heatmap with labels as well}

\subsubsection{MLP (main body experimental section)}
To verify the geometry properties in other architectures, we trained a Multi-layer Perceptron model(MLP) on Extracted TinyStories dataset. As MLP models are less expressive than Transformers, we use a MLP contained eight times more number of parameters comparing to transformers. 
\yz{say something about the result}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/Sim_SHWFixedLMLP_d128.pdf}
%     \caption{\yz{fix:remove title, fix colorbar. }Embedding geometries trained by MLP. \\First row: Geometry Comparison between $S$ and $\Hb$; second row: Geometry comparison between $S^T$ and $W^T$ }
%     \label{fig:Sim_SHWFixedLMLP_d128}
% \end{figure}
\subsubsection{Auto-regressive Loss curve(Auto-regressive section in the appendix)+explain in the set-up}
Note that the length of context does not have impact on our theory, therefore we expect similar behavior in Auto-regressive(AR) setting, where we vary the context length. 
For this experiment, we train a 8-layer transformer auto-regressively on 200 stories from TinyStories with character-level tokenizer. We measure the loss convergence to entropy 
at each position from t=2 to t=17, i.e. for context length from 1 to 16. 
We also compare the pairwise-similarity of different length context embeddings and their pairwise similarity of support sets. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/losses_8 layer Transformer pos off_d256.pdf}
%     \caption{Loss convergence to entropy for at each position from t=2 to t=17. The convergence shows different curves across different positions. \yz{not sure if i should say the following} The convergence decreases as t increases when t is less than half the maximum length. However, for t greater than this threshold, better convergence is observed for larger t, with certain exceptions, such as t=3. }
%     \label{fig:positional_losses}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/H_S_sim_label_ar.pdf}
%     \captionsetup{width=\textwidth}
% \caption{Comparison of geometric cosines between $Cos(H,H)$ and $Cos(S,S)$ in auto-regressive experiments. The heatmaps display pairwise similarities for contexts ending with identical tokens (top-left and bottom-right) and cross-similarities for contexts ending with different tokens (top-right and bottom-left), selecting 5 contexts per length from 2 to 16 for endings "y\_" and "\_t".}

%     \label{fig:H_S_sim_label_ar}
% \end{figure}
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
%         % Node for the first image
%         \node[anchor=south west,inner sep=0] (image1) at (0,0) {\includegraphics[width=0.5\textwidth]{exp_results_yize/S_sim_label_ar.pdf}};
%         % Node for the second image, right next to the first
%         \node[anchor=south west,inner sep=0] (image2) at (image1.south east) {\includegraphics[width=0.5\textwidth]{exp_results_yize/H_sim_label_ar.pdf}};
%     \end{tikzpicture}
%     \caption{AR S and H comparison}
% \end{figure}

\subsubsection{Additional Linear Layer Experiment}
This section examines the network's performance when the decoder dimension $d_{\text{decode}}$ is less than $V$, contrary to the requirement of $d>V$ specified in Equation \ref{eq:ufm relax}. By fixing the context embeddings' expressibility, we investigate the impact of varying $d_{\text{decode}}$ on the geometry embeddings. To maintain adequate expressivity, we configure the network with ten transformer layers, each with a dimensionality of $d=64$. Additionally, we introduce an extra linear layer to adjust $d_{\text{decode}}$, and subsequently, we analyze the effects on loss convergence and geometric properties.

\begin{figure}[ht]
\centering
\vspace{-10pt}
\begin{subfigure}{0.6\textwidth}
		\centering
  \hspace{-55pt}
		\begin{tikzpicture}
			\node at (-0,-0) 
			{\includegraphics[scale=0.3]{exp_results_yize/Hsim_6 layer Transformer pos off_d64.pdf}};
   \node at (0.0,-1.7) [scale=0.9]{(a) cosine similarity heatmaps};
		\end{tikzpicture}
    \end{subfigure}
    % 
    \hspace{35pt}
    \begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (-0,-0) 
			{\includegraphics[scale=0.33]{exp_results_yize/CEloss_6layerTFM_tiny_extract_m404_128_64.pdf}};
   \node at (0.0,-1.7) [scale=0.9]{(b) loss convergence};
		\end{tikzpicture}
    \end{subfigure}
    \caption{\textbf{(a)} Left: Column-wise similarities of support sets.  Middle and Right: Column-wise similarities of context embeddings $H$ trained with Transformer model with $d=128>V$ and $d=64<V$, respectively. The vocabulary size is set to $V=104$, and number of unique contexts $m=403$, \textbf{(b)} Loss converges to lower bound $H=1.2179$ for both transformer models with $d=128>V$ and $d=64<V$.}

    \label{fig:d<V}
    \end{figure}
% \subsubsection{$WW^T$ VS $\sqrt{SS^T}$(no normalization) informal discussion on $SS^T$. remain as empirical in main body}
% \subsubsection{$d<v$ + future section + appendix section(preliminary empirical result on $d<V$)}

% To better motivate future work on $d<V$, we present preliminary experiments in this section. We preform similar experiments to Sec. 4.2 and Fig. 1 in the initial manuscript, this time for $d < V$. 
% For moderate values of $d$, the loss reaches the empirical entropy lower bound. We also note the high overlap between the similarity patterns of contexts and support sets, similar to the case of $d>V$ presented in the paper.

% \begin{figure}[ht]
% \centering
% \vspace{-10pt}
% \begin{subfigure}{0.6\textwidth}
% 		\centering
%   \hspace{-55pt}
% 		\begin{tikzpicture}
% 			\node at (-0,-0) 
% 			{\includegraphics[scale=0.3]{exp_results_yize/Hsim_4 layer Transformer pos off_d64.pdf}};
%    \node at (0.0,-1.7) [scale=0.9]{(a) cosine similarity heatmaps};
% 		\end{tikzpicture}
%     \end{subfigure}
%     % 
%     \hspace{35pt}
%     \begin{subfigure}{0.3\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0,-0) 
% 			{\includegraphics[scale=0.33]{exp_results_yize/CEloss_TFM_tiny_extract_m404_128_64.pdf}};
%    \node at (0.0,-1.7) [scale=0.9]{(b) loss convergence};
% 		\end{tikzpicture}
%     \end{subfigure}
    
% \caption{\textbf{(a)} Left: Column-wise similarities of support sets.  Middle and Right: Column-wise similarities of context embeddings $H$ trained with Transformer model with $d=128>V$ and $d=64<V$, respectively. The vocabulary size is set to $V=104$, and number of unique contexts $m=403$, \textbf{(b)} Loss converges to lower bound $H=1.2179$ for both transformer models with $d=128>V$ and $d=64<V$.}

% \label{fig:structual_corr}
% \end{figure}
\subsubsection{SSIM curves \yz{(Include!!) for W as well, in the main body}}
% \subsubsection{SSIM Curves}
We quantitatively measure the structural similarity index (SSIM), as defined in \eqref{eq:ssim}, between the cosine similarities of $Cos(H, H)$, $Cos(S, S)$, $Cos(W^T, W^T)$, and $Cos(S^T, S^T)$ throughout the training process. This analysis complements the patterns observed in the heatmaps regarding the embedding geometry.

% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
%         % Node for the first image
%         \node[anchor=south west,inner sep=0] (image1) at (0,0) {\includegraphics[width=0.5\textwidth]{exp_results_yize/H_S_sim_structural_corr_bothdatasets.pdf}};
%         % Node for the second image, right next to the first
%         \node[anchor=south west,inner sep=0] (image2) at (image1.south east) {\includegraphics[width=0.5\textwidth]{exp_results_yize/W_S_sim_structural_corr_bothdatasets.pdf}};
%     \end{tikzpicture}
%     \caption{Increasing structural correlation between $Cos(H, H)$ and $Cos(S, S)$, as well as $Cos(W^T, W^T)$ and $Cos(S^T, S^T)$, during training. \tina{@Yize: fix title/labels + For the experiments we include in the main body, I prefer to have their ssim in the main body. or is Appendix better?} \tina{$SS^\top$ or the centered one?}}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/H_S_sim_structural_corr_bothdatasets.pdf}
%     \caption{Increasing structural correlation between $Cos(H, H)$ and $Cos(S, S)$ during training.}
%     \label{fig:H_S_sim_ssim}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/W_S_sim_structural_corr_bothdatasets.pdf}
%     \caption{Increasing structural correlation between $Cos(W^T, W^T)$, and $Cos(S^T, S^T)$ during training.}
%     \label{fig:W_S_sim_ssim}
% \end{figure}

\subsubsection{SSIM for conjecture \yz{?}}
% \subsubsection{$WW^T$ VS $(I-1/V11^T)SS^T(I-1/V11^T)$(no normalization)}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/gh_sqrtlmm_structural_corr_bothdatasets.pdf}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{exp_results_yize/gw_sqrtlmm_structural_corr_bothdatasets.pdf}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% % \end{figure}
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
%         % Node for the first image
%         \node[anchor=south west,inner sep=0] (image1) at (0,0) {\includegraphics[width=0.5\textwidth]{exp_results_yize/gh_sqrtlmm_structural_corr_bothdatasets.pdf}};
%         % Node for the second image, right next to the first
%         \node[anchor=south west,inner sep=0] (image2) at (image1.south east) {\includegraphics[width=0.5\textwidth]{exp_results_yize/gw_sqrtlmm_structural_corr_bothdatasets.pdf}};
%     \end{tikzpicture}
%     \caption{Increasing structural correlation between $H^TH$ and $(\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\smat)^{\frac{1}{2}}$, as well as between $WW^T$ and $((\Id_V-\frac1V\ones_V\ones_V^\top)\smat\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top))^{\frac{1}{2}}$, during training.}
% \end{figure}
% % \begin{align*}
%      \Wmm{\Wmm}^\top &= (\Lbmm{\Lbmm}^\top)^{\frac{1}{2}} \approx \Big((\Id_V-\frac1V\ones_V\ones_V^\top)\smat\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\Big)^{\frac{1}{2}},\\
%     {\Hmm}^\top\Hmm &= ({\Lbmm}^\top\Lbmm)^{\frac{1}{2}} \approx \Big(\smat^\top(\Id_V-\frac1V\ones_V\ones_V^\top)\smat\Big)^{\frac{1}{2}}.
% \end{align*}
% \subsubsection{Rank of $L_{in}$ and $L_{mm}$ and $L_{in} + C L_{mm}$ try this and see how rank changes}

 \pagebreak

==> Arxiv_NewTempl/sections/autoregressive.tex <==
\section{Autoregressive}


\begin{definition}
    The unconstrained features model for \textbf{autoregressive} NTP training over training set $\Tc = \{\{\pih_{t,j},\ph_{t,j,z\in\Vc}\}_{j\in[m_t]}\}_{t\in[T-1]}$ refers to the following problem:
    \begin{align}\label{eq:ufm}
        \min_{\W,\hd_{t,j}} ~~\left\{ - \sum_{t\in[T-1]}\sum_{j\in[m_t]}\pih_{t,j}\sum_{z\in\Sc_j}\ph_{t,j,z}\log\left(\sfti{z}{\W \hd_{t,j}}\right)\right\}+\la\|\W\|^2 + \la\sum_{t\in[T-1]}\|\Hb_t\|^2,\tag{NTP-UFM}
    \end{align}
    where the minimization is over $\W\in\R^{V\times d}$ and $\Hb_t:=[\hd_{t,1},\ldots,\hd_{t,m_t}]\in\R^{V\times m_t}$. Here, $m_t, t\in[T-1]$ is the number of distinct contexts of size $t$. Note that $m_1\geq m_2 \geq \cdots \geq  m_{T-1}.$ Accordingly, $\hd_{t,j}, t\in[T-1],j\in[m_t]$ is the $j$-th distinct embedding of $t$-long context $\xd_{t}:=(z_1,\ldots,z_t)$.
\end{definition}

\begin{definition}[AR-\NTPH-compatible]\label{def:NTP-comp}
    We say that training data $\Tc$ are AR-\NTP-entropy-compatible   if there exists $V\times d$ matrix $\Wf$ and embeddings $\hd_{t,j}, t\in[T-1],j\in[m_t]$ satisfying the following:
    %For all $j\in[m]$ and all $z\neq z'\in\Sc_j$,
        \begin{align}\label{eq:Wf condition}
\forall t\in[T-1],j\in[m_t], z\neq z'\in\Sc_{t,j}~:~~        (\eb_z-\eb_{z'})^\top\Wf \hd_{t,j}=\log\left({\ph_{t,j,z}}\big/{\ph_{t,j,z'}}\right)\,.
        \end{align}
\end{definition}

\begin{definition}[AR-\NTP-separable]\label{def:NTP-sep}
    We say that training data $\Tc$ are AR-\NTP-separable if there exists $V\times d$ matrix $\Ws$ and  embeddings $\hd_{t,j}, t\in[T-1],j\in[m_t]$ satisfying the following:
        \begin{subequations}\label{eq:Wmm condition}
        \begin{align}
        \forall t\in[T-1], j\in[m_t], z\neq z'\in\Sc_j~&:~~(\eb_z-\eb_{z'})^\top\Ws \hd_{t,j} =0\,\label{eq:Wmm condition equal}
        \\
        \forall t\in[T-1], j\in[m_t], v\notin\Sc_j~&:~~(\eb_z-\eb_{v})^\top\Ws \hd_{t,j} \geq 1\,.\label{eq:Wmm condition larger}
        \end{align}
        \end{subequations}
\end{definition}

\subsection{Simple architectures}
The models below were first explored  at least as early as \cite{bengio1999modeling}, and applied to language modeling in \cite{bengio2000neural}. The modern version of this idea
is called the Neural Autoregressive Distribution Estimator (NADE) \cite{larochelle2011neural}.


\paragraph{Simple(st) embedding architecture: One-hiddne ReLU layer with parameter sharing.} Let $\eb_z\in\{0,1\}^{V}$ be one-hot encoding of token $z\in\Vc$. Then, sequence $\z_{\leqt}=(z_1,\ldots,z_t)$ has one-hot encoding representation $\eb(\z_{\leqt}):=[\eb_{z_1}^\top,\ldots,\eb_{z_t}^\top]\in\{0,1\}^{tV}$. 

Now, let $\A\in\R^{d\times (T-1)V}$ be weight-matrix of hidden layer. Denote $\A_\leqt:=\A_{:,1:tV}\in\R^{d\times tV}$ the submatrix consisting of the first $tV$ columns of $\A$. 

The embedding $\hb_{t}$ of input sequence $\z_\leqt$ is given as:
\begin{align}
    \hb_t = \relu\left(\A_\leqt\eb\left(\z_\leqt\right)\right)
\end{align}

% Thus, the $V$ output logits of the model are 
% \[
% \ellbb_t:=\W\hd_t\,.
% \]

\paragraph{MLP with parameter sharing and input encoder} A slightly more realistic variation of this is one that uses real-valued encoding of tokens before passing through MLP. Specifically, let $\Win\in\R^{V\times \din}$ an input encoder. Then every token $z$ gets encoded to $\Win^\top\eb_{\z}$ and a sequence $\z_\leqt$ gets encoded to
\[
\eb(\z_\leqt;\Win)=[\eb_{z_1}^\top\Win,\ldots,\eb_{z_t}^\top\Win]\in\R^{t\din}
\]
Now, let $\A\in\R^{d\times (T-1)\din}$ be weight matrix of hidden layer. Denote $\A_\leqt$ the submatrix of the first $t\din$ columns (or $t$ column blocks). 

Then, the embedding $\hb_t$ of input sequence $\z_\leqt$ is given as
\begin{align}
    \hb_t=\relu\left(\A_\leqt \eb(\z_\leqt;\Win)  \right)\in\R^d
\end{align}

Overall, the $V$ output logits of the model are
\[
\ellbb_t:=\W\relu\left(\A_\leqt \eb(\z_\leqt;\Win)\right) \,.
\]

Of particular interest might be the (commonly used in practice) setting of encoder-decoder parameter-sharing in which $\Win=\W$.


\paragraph{Deep.} Let $\A_{k}, k=1,\ldots,D\in\R^{d_k\times (T-1)d_{k-1}}$ be  weight matrices of $D$ hidden layers with $d_0:=\din$ and $d_D:=d$. Then, with notations above, the embedding $\hb_t$ of input sequence $\z_\leqt$ is:
\begin{subequations}
\begin{align}
\hb_t&:=\hb_{D,t} 
\\
\hb_{k,t}&=\relu\left(\A_{k,\leqt} \hb_{k-1,t}\right),\quad k=1,\ldots,D\\ \hb_{0,t}&=\eb(\z_\leqt;\Win)      
\end{align}
\end{subequations}


==> Arxiv_NewTempl/sections/collapse_app.tex <==
\begin{proposition}[Subspace collapse]\label{propo:collapse}
 Assume \ref{eq:ufm-svm} is feasible. There exists minimizer $\Hb=[\hb_1,\ldots,\hb_m]$  of \ref{eq:ufm} such that for all contexts $j,j'\in[m]$ with same support set $\Sc_j=\Sc_{j'}$, their embeddings are same in direction in the limit of vanishing regularization, i.e., $\lim_{\laz}\left\|\overline{\hb_j}-\overline{\hb_{j'}}\right\|=0$. 
\end{proposition}
% 

This is consistent with our empirical observations in Figs.~\ref{fig:simplified_intro} and \ref{fig:intro_TinyStories}: As the loss approaches its lower bound, context embeddings with the same support set converge in the same direction and exhibit maximum correlation. This is indicated by the bright diagonal blocks in $\corr{\Hb}$ heatmaps.


% As specified by Thm.~\ref{thm:reg path finite}, the on-support entries of the logit $\Lb_{\la\to0}$ satisfy the log-odds constraints on a subspace orthogonal to the subspace where the limiting direction of $\Lb_\laz$ resides. See Secs.~\ref{sec:ufmexp} and \ref{sec:exp_main} for more numerical results.

The proposition can be proved by inspecting \ref{eq:ufm-svm}: Since the affine constraints \eqref{eq:svm equalities} for each sample $j\in[m]$ depend solely on the support set $\Sc_j$, it can be shown that there exists a minimizer $\Lbmm=[\ellbb_1^\text{mm},\cdots,\ellbb_m^\text{mm}]$ such that $\ellbb_j^\text{mm}=\ellbb_{j'}^\text{mm}$ whenever $\Sc_j=\Sc_{j'}$. This implies that the corresponding columns $j,j'$ of $\Vb^\top$ are identical. As a result, by Cor.~\ref{cor:WH}, $\lim_{\laz}\left\|\overline{\hb_j}-\overline{\hb_{j'}}\right\|=0$. \looseness=-1

It is important to reiterate that Prop.~\ref{propo:collapse} does not prevent the minimizer $\Lb_\la=\W_\la\Hb_\la$ from accurately recovering the distinct soft-label values $\pbh_j,\pbh_{j'}$ and achieving the empirical entropy lower-bound $\Hc$ as $\laz$: The collapse occurs on subspace $\Ts_\perp$, orthogonal to the data subspace $\Ts$ on which the logit matrix satisfies the log-odds constraints indicated in Thm.~\ref{thm:reg path finite}; See Secs.~\ref{sec:ufmexp} and \ref{sec:exp_main} for numerical verifications. \looseness=-1


==> Arxiv_NewTempl/sections/discussion.tex <==
\vspace{-0.1in}
\section{Future Work}
\vspace{-0.1in}
We foresee several promising avenues for future research. Even within the current linear setting and GD, a particularly interesting direction involves extending our analyses to the autoregressive training objective Eq. \eqref{eq:intro CE} covering all subsequences. Additionally, it is intriguing to identify exact thresholds for \NTP linear-separability under distributional assumptions, akin to previous work on one-hot separability (see Remark \ref{rem:sep thresholds}).
 Finally, we envision using our results to facilitate the study of generalization in \NTP settings by examining the statistical properties of the \NTP-SVM solution. As discussed in Sec. \ref{sec:rel work}, past research has successfully undertaken similar investigations for one-hot classification. While we acknowledge the importance of addressing specific challenges inherent to the \NTP setting—such as determining an appropriate measure of generalization that may differ from the winner-takes-all approach, or establishing suitable statistical models for embeddings that respect the discrete nature of the underlying token subsequences defining the context—we believe this direction holds promise for further exploration. In addition to these aspects, essential extensions include relaxing the linearity assumption, thereby studying architecture-specific embeddings. Exploring the \NTP implicit bias of adaptive algorithms, such as normalized GD and Adam, is another avenue for future research. The overall goal is to contribute to a deeper understanding of the intricacies and yield potential improvements in \NTP training and its applications. 

 


% \paragraph{Beyond linear.}


% \paragraph{Beyond last-token.}


% \paragraph{Other algorithms.}

% \paragraph{Generalization.}

==> Arxiv_NewTempl/sections/experiments.tex <==
%\section{Experiments}

\section{Experiments}\label{sec:exp}
We examine the implicit bias of GD on NTP training over synthetic data generated as follows. We construct dataset with $n=5000$ sequences involving $m=50$ distinct contexts. Each distinct context gets mapped to a randomly generated embedding of dimension   $d=60>m$. We set vocabulary size $V=10$ and each context $j\in[m]$ is followed by $S_j=6, \forall j\in[m]$ possible next-tokens. The support sets $\Sc_j\subset\Vc$ and the probabilities $\ph_{j,z}, z\in\Sc_j$ are chosen randomly; see Fig. \ref{fig:probs} for representative examples from the training dataset. For a fixed realization of the dataset (for which $\Hc\approx1.445$nats), we run GD, normalized GD (NGD), and Adam from random LeCun initialization. For GD, we use learning rate $\eta=0.5$ and for NGD and Adam $\eta=0.01$. For Adam, we also set $\beta_1=0.9, \beta_2=0.99$. We run all algorithms for $1e4$ iterations. For each case, we plot the following as a function of iterations:
\begin{enumerate}
    \item Upper Left: CE loss versus entropy lower bound
    \item Upper Right: parameter norm growth
    \item Lower Left: correlation of $\Wmm$ with iterates $\W_k$ and of ``corrected'' iterates $\W_k-\Wstar$ after substracting the component on $\Hc$ 
    \item Lower Right: convergence of the subspace component $\W_{k,\perp}$
\end{enumerate}
Fig. \ref{fig:implicit bias} shows an instance of these. As predicted by our analysis, in this overparameterized setting: CE loss converges to its lower-bound, parameter norm increases, iterates align in direction with $\Wmm$, and the subspace component converges to $\Wstar$.

  

%A toy example of \NTP training and its implicit bias in $d=2$. \emph{Left:} Visualization of the  $m=3$ embeddings $\hd_j$ (blue markers) and of their associated support sets $\Sc_j$ (colored text below each marker).
 %   Also, shown the hyperplanes defined by rows of $\Wmm$ for the vocabulary of size $V=5$. \emph{Right:} CE loss, parameter norm growth and correlation with $\Wmm$ over $1e5$ GD iterations. Correlation is shown for $\W_k-\Wf$ for two different choices of $\Wf$ (green,blue) and directly for $\W_k$ (red).

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{probs2.eps} 
% \includegraphics[width=\linewidth]{figure2d.pdf}  
\captionsetup{width=\textwidth}
    \caption{Eight randomly picked contexts with their associated  next-token empirical conditional probabilities $\pbh_j$. The indices shown on the x-axis define the support set $\Sc_j$ of each context.
    }
    \label{fig:probs}
\end{figure}


Figure \ref{fig:both} illustrates the same plots, but this time for training over the same dataset with NGD and Adam. We observe same implicit bias, but faster convergence. For NGD, this is consistent with analogous findings (rigorous in that case) for one-hot classification \cite{nacson2019convergence,ji2021characterizing}.
%\ct{briefly talk about experiment. Appendix for high-dimensional example}

Finally, Figure \ref{fig:2d} illustrates a toy 2d example where the embeddings and the hyperplanes defined by each row of $\Wmm$ can be visualized. We used $d=2, m=3, V=5$ and $S_1=S_2=S_3=3$. The support sets of each embedding are shown in the figure color-coded to match the respective decoder hyperplane. Probabilities are assigned randomly. For the instance shown therein, the empirical conditional entropy evaluates to $\Hc=0.8811$.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{ngd.eps}  
% % \includegraphics[width=\linewidth]{figure2d.pdf}  
% \captionsetup{width=\textwidth}
%     \caption{Implicit bias of \emph{normalized} GD in \NTP over synthetic data with overparameterization. Observe that NGD exhibits the same implicit bias, but converges faster than GD.
%     }
%     \label{fig:ngd}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{adam.eps}  
% % \includegraphics[width=\linewidth]{figure2d.pdf}  
% \captionsetup{width=\textwidth}
%     \caption{Implicit bias of \emph{normalized} GD in \NTP over synthetic data with overparameterization. Observe that Adam exhibits the same implicit bias, but converges even faster than NGD.
%     }
%     \label{fig:adam}
% \end{figure}



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{main}  
% \includegraphics[width=\linewidth]{figure2d.pdf}  
\captionsetup{width=\textwidth}
    \caption{Experimental illustration of the implicit bias of GD in \NTP over synthetic data with overparameterization. See App. \ref{sec:exp} for detailed description of the experimental setting. The upper two graphs confirm the predictions of Lemma \ref{lem:norm growth}, while the lower two graphs adhere to the predictions of Theorem \ref{thm:GD main}.
    }
    \label{fig:implicit bias}
\end{figure}


\begin{figure}[h!]
    \centering
    \begin{minipage}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ngd.eps}  
        \vspace{-0.3in}
        \caption*{NGD}
        % \label{fig:ngd}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.47\textwidth}
        \centering
        \includegraphics[width=\linewidth]{adam.eps}  
        \vspace{-0.3in}
        \caption*{Adam}
        % \label{fig:adam}
    \end{minipage}
    \captionsetup{width=\textwidth}
    \vspace{-0.15in}
    \caption{Implicit bias of \emph{normalized} GD (Left) and of Adam (Right) in \NTP over synthetic data with overparameterization. Both exhibits the same implicit bias, but converge faster than GD, with Adam being slightly faster than NGD.}
    \label{fig:both}
\end{figure}

==> Arxiv_NewTempl/sections/exps.tex <==
% In this section, we empirically validate our theoretical findings. We start  by tracking the GD path when training UFM and confirming its convergence to the theoretical claims outlined in Thms.~\ref{thm:reg path}, \ref{thm:reg path finite} and Cor.~\ref{cor:WH}. We then validate our predictions using transformers (TFs) trained on our synthetic data and on a subset of Tiny Stories \citep{eldan2023tinystories}. 
% \vspace{-0.1in}
% 
% In this section, we empirically validate our theoretical findings. We start by UFM, confirming that the solution found by GD converges to the claims outlined in Thms.~\ref{thm:reg path} and \ref{thm:reg path finite}. We then move on to experiments on deep-nets. We start by a synthetic setup where it is computationally feasible to find the optimal solution predicted by our theoretical analysis for $\W$ and $\Hb$. In these two setups, we empirically find a close proxy for the geometrical structure of the embeddings that does not rely on SVD calculations. We then use this proxy in a larger-scale experiment, where we train transformer (TF) based model on a portion of the TinyStories dataset.


In this section, we empirically validate our theoretical findings on text data. 
% We begin with UFM, confirming that the solution found by gradient descent aligns with the regularization path characterized in Thms.~\ref{thm:reg path} and \ref{thm:reg path finite}. Next, 
Unlike Sec.~\ref{sec:ufmexp}, the probability and sparsity matrices $\Pbb$ and $\smat$ abide by the structure of underlying language data. Also, embeddings are generated by training deep networks. 
We start with two small-scale synthetic test-data setups for which we examine Claims \ref{P logits}-\ref{P soft-labels}. We then experiment with a larger-scale dataset. For this, SVD calculation are expensive. Thus, we only compare the implicit geomtry of the deep network to the Proxy \ref{P proxy}. \looseness=-1
% where it is computationally feasible to find the optimal solution predicted by our theoretical analysis for \(\W\) and \(\Hb\). In the synthetic setup, we empirically verify how close our proxies in \Eqref{eq:proxy2} is to the geometric structure of the embeddings. We then examine this proxy in a larger-scale experiment, training a transformer-based model on a portion of the \TS~dataset \citep{eldan2023tinystories}, where SVD calculations turn out to be expensive.


% % \vspace{-5pt}
% \subsection{UFM}\label{sec:ufmexp}
% We train UFM with vocabulary size $V=10$, embedding dimension $d=10$, and $m=95$ training samples whose support matrix $\smat$ is shown in Fig.~\ref{fig:UFM_heatmap} (c). We set $\pih_j = {1}/{m}$ and for this fixed support matrix $\smat$, we generate random soft labels $\pbh_{j}\in\Delta^{V-1}$ such that $\ph_{j,v}\neq0, v\not\in\Sc_j$.
% % 
% % $\pbh_{j,z}, z\in\Sc_j$. 
% We train \ref{eq:ufm} with SGD and small weight decay $\lambda=10^{-5}$. 
% % \new{In this section, we measure the directional distance of two matrices $\mathbf{A}$ and $\hat{\mathbf{A}}$ as $\|\frac{\mathbf{A}}{\|\mathbf{A}\|_*}- \frac{\hat{\mathbf{A}}}{\|\hat{\mathbf{A}}\|_*}\|$}.

% % Defining $\Lb_k, \Hb_k, \W_k$ to be the logits, embeddings and classifiers at iteration $k$, we verify the predictions of Thms.~\ref{thm:reg path} and \ref{thm:reg path finite} in Fig.~\ref{fig:UFM_conv}:  1) The loss converges to its lower-bound, $\Hc$, which we compute using the true soft labels. 2) The norms $\norm{\Lb_k}_*$, $\norm{\W_k}$, and $\norm{\Hb_k}$ keep growing as training progresses. 3) While $\Lb_k$ grows in norm, it converges in direction to $\Lbmm$ that only depends on the support matrix. However, its projection to the subspace $\Ts$ will align with $\Lbin$ that ensures the soft-labels are learned by the model. 4) As specified in Cor.~\ref{cor:WH}, since the relaxation in \eqref{eq:ufm relax} is tight, $\W_k\W_k^\top$ and $\Hb_k\Hb^\top_k$ converge in direction to $\GWmm:=\Ub\Sigmab\Ub^\top$ and $\GHmm:=\Vb\Sigmab\Vb^\top$. \new{Here, we note that, the convergence is slow which is consistent with the implicit bias results that generally exhibit a convergence rate of $\mathcal{O}(1/\log(k))$ \citep{soudry2018implicit}.}

% \new{The results are shown in Fig.~\ref{fig:UFM_heatmap}. 
% % Let $\Lb_k, \Hb_k, \W_k$ be the logits, context and word embeddings at epoch $k$. 
% We train the model long enough to get close to the empirical entropy lower-bound $\Hc$: As illustrated in the Fig.~\ref{fig:UFM_heatmap} (d), towards the end of the training, the loss $\CE(\Lb_k)$ converges to $\Hc\approx1$ within an order of $10^{-4}$. }

% \new{In panel (a), we show the evolution of the UFM parameters, logits $\Lb_k=\W_k\Hb_k$, word embeddings $\corr{\W_k^\top}$ and context embeddings $\corr{\Hb_k}$. We first note that at the end of the training the parameters converge to the theoretical prediction by Thm.~\ref{thm:reg path} and Cor.~\ref{cor:WH} specified by $\Lbmm$ and its SVD factors as shown in column (b).  Next, we empirically observe that the correlation patterns between the word/context embeddings follow closely the structural patterns of the support sets and their pairwise similarity as displayed in column (c).}
% % \new{% We track the evolution of the embeddings' geometry throughout training. The first three columns in Fig.~\ref{fig:UFM_heatmap} display the logit matrix \(\Lb_k\), the geometry of the % word embeddings $\cosa{\W^\top}{\W^\top}$ % \tina{ do we want to change the notations? like $.$ (for l2 normalization over cols) and another notation for row wise normalization , and the context embeddings $.$, at initialization, at an intermediate step, and at the final iteration.}\ct{I don't like this notation much. What would be cleaner is to define  a metric (you can call it corr for correlation or anything else you think is better, e.g. simply $\corr{\A}$) $\operatorname{corr}{A}$ for $\cos(\A,\A)$ and then use $\operatorname{corr}{A}$ or $\operatorname{corr}{A^\top}$}% }% \new{We first note that the structural patterns appearing in the geometry of the embeddings closely follows the theoretical prediction in Cor.~\ref{cor:WH}, i.e., $\Wmm$ and $\Hmm$ illustrated in the fourth column. Next, we empirically observe that the similarity patterns between the embeddings are well-correlated with the similarity between the support sets (fifth column).} 
% Specifically, for a given sample $j\in[m]$, the corresponding embedding has higher correlation with samples $j'$ whose support set intersection $|\Sc_j\cap \Sc_{j'}|$ is larger. {In the special case where the support sets of two contexts are identical, the figure also verifies property \ref{P collapse}: Along the diagonal blocks of $\corr{\Hb}$, where the contexts with similar support sets lie, the samples have maximum correlation and are aligned.} Similarly, word embeddings of two tokens are closer if they appear together in more support sets: \new{word embedding $\w_z$ is more similar to $\w_{z'}$ when $|\{j| \w_z, \w_{z'}\in\Sc_j,\,j\in[m]\}|$ is larger}. 
% \new{To verify the close relationship between the embeddings and the support sets more quantitatively, we measure $\ssim{\corr{\Hb}}{\corr{\Sb}}$ and $\ssim{\corr{\W^\top}}{\corr{\Sb^\top}}$ \tina{bad notation}, where $\ssim{\Xb}{\Yb}$ measures the structural correlation between the two matrices as follows,\footnote{This is the structure component in the Structural Similarity Index Measure (SSIM) which is used to measure the similarity between two images \citep{wang2004image}.}
% % the structural similarity of $\corr{\Hb}$ (resp. $\corr{\W^\top}$) with $\corr{\Sb}$ (resp. $\corr{\Sb^\top}$), using the following correlation metric between two matrices $\Xb$ and $\Yb$:\footnote{This is the structure component in the Structural Similarity Index Measure (SSIM) which used to measure the similarity between two images \citep{wang2004image}.} 
% }
% % 
% \begin{align}\label{eq:ssim}
%     \ssim{\Xb}{\Yb} = \frac{\sigma_{\Xb\Yb} + \epsilon}{\sigma_\Xb \sigma_\Yb + \epsilon}, 
% \end{align}
% \new{where \(\sigma_{\Xb\Yb}\) is the covariance, and \(\sigma_\Xb\) and \(\sigma_\Yb\) are the standard deviations of \(\Xb\) and \(\Yb\), respectively, and $\epsilon$ is a small constant for stable division. A value of \(\ssim{\Xb}{\Yb} = 1\) indicates perfect correlation. We show the evolution of this metric for context embeddings (blue) and word embeddings (red) in plot (e). }


% These observations are consistent with the intuition of the distributional assumption that the meaning of a word/context is determined by the ``company it keeps'' \citep{harris1954distributional}.
% This behavior, which is reflected on embeddings, emerges from our model and analysis as a consequence of the implicit bias of the NTP training to promote low-rank logits subject to equality/inequality margin constraints for in/out-support tokens. 
% % 
% {We provide more detailed quantitive verifications of Thms.~\ref{thm:reg path} and \ref{thm:reg path finite} in Sec.~\ref{sec:ufm_app} in the App.}

% % We first  illustrates their evolution throughout training. The figure shows their geometry is well correlated with the structural properties of the training distribution. Specifically, observe that, for a given sample $j\in[m]$, the corresponding embedding has higher correlation with samples $j'$ whose support set intersection $|\Sc_j\cap \Sc_{j'}|$ is large. In fact, for those contexts that share the same support set $\Sc_j=\Sc$, the learned context embeddings nearly collapse \tina{need some clarification on collapse at some point}, as observed on the diagonal blocks of $\cosa{\Hb}{\Hb}$. Similarly, word embeddings of two tokens are closer if they appear together in more support sets: \new{word embedding $\w_z$ is more similar to $\w_{z'}$ when $|\{j| \w_z, \w_{z'}\in\Sc_j,\,j\in[m]\}|$ is larger}. {These observations are consistent with the intuition of the distributional assumption that the meaning of a word/context is determined by the ``company it keeps'' \citep{harris1954distributional}. This behavior, which is reflected on embeddings, emerges from our model and analysis as a consequence of the implicit bias of the NTP training to promote low-rank logits subject to equality/inequality margin constraints for in/out-support tokens.}
% % 
% % We also note that the recovered geometry during training converges to the max-margin solution specified by $\Lbmm$ in Thm.~\ref{thm:reg path}. We also confirm numerically that in this case $\Lbmm=\Lbtina$ as defined in Sec.~\ref{sec:general geometries}\tina{check}. 
% % For detailed verification of Thms.~\ref{thm:reg path} and \ref{thm:reg path finite}, see Sec.~\ref{sec:ufm_app}.% in the App.%\tina{move this to synthetic section if moved to appendix} \tina{comparison to mm not discussed}


% % \textbf{Logits.}~To measure the finite component, We track , where $\Lbin$ is ??, and the projection is defined as in ??. For the directional convergence, we compute $\|{\frac{\Lbo_k}{\|\Lbo_\la\|_*} - \frac{\Lbmm}{\norm{\Lbmm}_*}}\|$, where $\Lbmm$ is the \eqref{eq:ufm-svm} solution \tina{found by cvxpy?}. \tina{fix the plots with nuc norm normalization}
% % 
% % \textbf{Classifiers and embeddings.}~To verify Cor.~\ref{cor:WH}, we track $\|\overline{\W_k\W_k^\top}- \Ub\overline{\Sigmab}\Ub^\top\|_F$ and  $\|\overline{\Hb_k\Hb_k^\top}- \Vb\overline{\Sigmab}\Vb^\top\|_F$. \tina{or projections?}
% % 



\subsection{Datasets}
We use a total of three datasets. We first employ two smaller-scale datasets, which are well-suited for verifying our theoretical solutions. Then, we use one larger-scale dataset designed to investigate the geometric properties of text in conditions that approximate real-world text scenarios. \looseness=-1 

% \begin{itemize}
    % \item 
    % \vspace{5pt}
    \noindent\synth.~We generate each context $\xd_j$ as follows: We select $T-1=5$ words (tokens), and manually come up with the $T=6$-th tokens that are consistent with the given context. To model the probabilities $\pih_j$ and $\pbh_j$, we sample each support independently to a number of repeats to emulate the behavior of repeated context in natural language. For instance, the context $\xd_j=$ ``\texttt{Lily wants to try the}'' is followed by $\Sc=\{\texttt{soup}, \texttt{game}, \texttt{movie}\}$ with respective probabilities $ [0.5, 0.25, 0.25]$. {The dataset consists of $n=116$ samples, containing $m=16$ distinct contexts, and a vocabulary size of $V=30$. Each context has a fixed support set length of $|\mathcal{S}_j|=3$.} In Fig.~\ref{fig:verysmalldataset}, we show the $m=16$ unique contexts and the soft labels on their next token. In this dataset, the tokenization is done at the word level and the empirical entropy lower-bound is $\Hc= 1.6597$.\looseness=-1% In Fig.~\ref{fig:verysmall_heatmaps}, we provide analogous plots to Fig.~\ref{fig:syn_heatmaps_w} for this setting.
    
    %\item 
    % \vspace{5pt}
    \noindent\simTS.~Advancing towards a more realistic but still controlled dataset, we use contexts and support sets from the \TS~corpus. 
    We derive contexts $\xd_j$ and support sets $\Sc_j$ from the \TS~dataset and we create the training data from the most frequent word-level contexts with length 5, such as $\xd_j = [\texttt{``once'', ``upon'', ``a'', ``time'', ``,''}]$. For the support sets $\Sc_j$, we record all next tokens of $\xd_j$ in the original dataset. Then, we replace the words in the contexts with their synonymous to generate new contexts with identical support sets. This allows us to have multiple contexts sharing common support sets, while controlling the vocabulary size, which is set to $V=104$. {The final dataset consists of $n\approx3050$ samples with $m\approx400$ unique contexts.} The frequencies $\pbh_j$ are determined by  independently sampling each next token from $\Sc_j$ several times. Here, $\Hc= 1.0166$.
    
    %\item 
    % \vspace{5pt}
    \noindent\TS.~To experiment with more standard data, we use 100 stories sampled from \TS. Here, we do not make any sample selections for contexts and support sets, unlike the other two datasets. We use a tokenizer with vocabulary size $V=128$, and fixed context length $T=6$. We choose a small context window and vocabulary size to make tracking the distinct contexts and their support sets computationally manageable. In this setup, the number of distinct contexts $m\sim 10^5$ and $\Hc=0.3112$. \looseness=-1
% \end{itemize}

\subsection{Models}
To test our theoretical framework, we train decoder-only transformer (TF) models on the three datasets described above. For \synth~and \simTS, we use a TF model with 4 layers, 6 attention heads and embedding dimension $d=128$. For \TS, we use a 12-layer TF with $d=256$. 

We inspect the context and word embeddings $\Hb$ and $\W$ at several checkpoints for each model to verify the following two claims made in Sec.~\ref{sec:analysis}: 1) We assess whether numerically optimizing both the TF model and \ref{eq:ufm} in each data setup yields the same geometrical structure. 2) We evaluate the global solution of \ref{eq:ufm}, as specified by Thm.~\ref{thm:reg path} and Cor.~\ref{cor:WH}, and check whether it respects the same implicit geometry as the TF and the \ref{eq:ufm}. For the first claim, we train the log-bilinear model in \ref{eq:ufm} directly on the label distribution of each dataset. This is computationally feasible only for the first two datasets. For the second claim, we find the global solution $\Lbmm$ of \ref{eq:ufm-svm} on each dataset using CVXPY \citep{diamond2016cvxpy}, and find $\Hmm$ and $\Wmm$ as in Cor.~\ref{cor:WH}. If not computationally possible, we only compare the implicit geometry with the proxy terms \ref{P proxy}.\looseness=-1
 
% We detail the models used to test our theoretical framework under varying configurations:
% \tina{no MLP here?}
% \yz{log-bilinear model}
% \begin{itemize}
    % \item \textbf{UFM on Text Data:} Operating under the assumption of over-parametrization, our goal was to test the theoretical analysis in a fully unconstrained setting. The Unconstrained Feature Model (UFM) was chosen to ensure that context embeddings remain free from model architectures. The learning targets, represented by next-token probability labels, were derived as soft labels from the text data. 
    % \item \textbf{Transformer:}
    % To validate our hypotheses, we conducted experiments using transformer models, known for their robust representational abilities and strong performance on textual data. For experiments on the Synthetic and Simplified TinyStories datasets, we employ a decoder-only transformer consisting of 4 layers and 6 attention heads. 
    % For the TinyStories dataset, we use a 12-layer transformer to ensure an appropriate level of over-parametrization and entropy convergence. 
  
% \end{itemize}


\subsection{Metrics}\label{sec:metric}
% To verify our theoretical analysis, We highlight the following key metrics:
In all our experiments, we track the CE loss convergence to the empirical entropy lower-bound $\Hc$ and verify the norm growth of the parameters as specified by Thm.~\ref{thm:reg path}. We also define the following metrics:

\vspace{2pt}
\noindent\textbf{Visualization of embeddings' geometry.}~To visualize the geometry of the word and context embeddings, we plot the heatmap of the normalized Gram matrix $\corr{\W^\top}$ and $\corr{\Hb}$, where for matrix $\Xb$,  $\corr{\Xb}$ is a matrix whose $(i,j)$-th entry is the cosine similarity between the respective columns of $\Xb$, i.e., \looseness=-1
$\big[\corr{\Xb}\big]_{i,j}=\frac{\x_i^\top\x_j}{\|\x_i\|\|\x_j\|}.$
To check Proxy \ref{P proxy}, we compare the context and word embeddings with $\corr{\smatbar}$ and $\corr{\smatbar^\top}$. \looseness=-1

\vspace{2pt}
\noindent\textbf{Quantifying geometric similarity.}~To measure the structural similarity between $\W$, $\Hb$ and $\smatbar^\top$, $\smatbar$ as in the proxy \ref{P proxy}, we use the following correlation metric between two matrices,\footnote{This is the Structural Similarity Index Measure (SSIM) used to measure the similarity between two images \citep{wang2004image}.}
%\begin{align}\label{eq:ssim}
 $   \ssim{\Xb}{\Yb} = \frac{\sigma_{\Xb\Yb} + \epsilon}{\sigma_\Xb \sigma_\Yb + \epsilon},$ 
%\end{align}
where \(\sigma_{\Xb\Yb}\) is the covariance, and \(\sigma_\Xb\) and \(\sigma_\Yb\) are the standard deviations of \(\Xb\) and \(\Yb\), respectively, and $\epsilon$ is a small constant for stable division. A value of \(\ssim{\Xb}{\Yb} = 1\) indicates perfect structural correlation. 
To simplify the presentation, and with some abuse of notation, we denote the similarity metric for context and word embeddings as follows,
% \footnote{To achieve \eqref{eq:proxy2}, we approximated the optimal solution and reduced computational complexity by omitting the square root. Therefore, we do not expect \eqref{eq:proxy2} to exactly match the Gram matrix of the embeddings. However, we want to determine if this proxy accurately predicts the structural properties of the embeddings. Thus, instead of directly computing the correlation between the embeddings and the centered support sets, we use the SSIM. \tina{keep or remove??}} 
\begin{align*}
    \ssimstar{\Hb}{\smatbar}:=\ssim{\corr{\Hb}}{\corr{\smat}}, \quad \ssimstar{\W^\top}{\smatbar^\top}:=\ssim{\corr{\W^\top}}{\corr{\smat^\top}}.
\end{align*}


% \vspace{5pt}
\noindent\textbf{Recovery of soft-labels.}~To verify   Thm.~\ref{thm:reg path finite}, we measure the distance $\|\Qcs(\Lb_k) - \Lbin\|$ of $\Lbin$ from the projection of $\Lb_k$ onto the subspace $\Fc$. 
% \begin{align*}
%     \distF{\Lb_k}{\Lbin} = \|\Qcs(\Lb_k) - \Lbin\|
% \end{align*}

% \begin{itemize}
    % \item \textbf{Loss Convergence to Entropy:} We measure how closely the loss values converge to the theoretical entropy limits, indicating the efficiency of the model in capturing the underlying data distribution.

    % \item \textbf{Similarity between Optimal Embedding Geometry and Support Sets:} We assess the geometric similarity between the calculated optimal embeddings and the actual support sets. This evaluation includes comparisons of heatmap representations and the use of the Structural Similarity Index (SSIM) to measure similarity more quantitatively.

    % \item \textbf{Projected Logits Convergence to $\Lbin$:} \yz{Yize fix}
    
    % \item \textbf{Convergence of Embedding Gram Matrices:} We examine the convergence of the embedding gram matrices to the theoretical constructs described in Corollary \ref{cor:WH}. This metric checks for the structural and mathematical alignment of the embeddings with the theoretical predictions.
% \end{itemize}






\vspace{-5pt}
% \noindent\textbf{Training Data.}~
% \noindent\textbf{Models.}~
\input{Arxiv_NewTempl/sections/expyize}

\vspace{-10pt}
% \subsection{Deep-nets}


==> Arxiv_NewTempl/sections/expvala.tex <==
% \label{sec:expvala}
% \subsubsection{Experimental Setup}

% \tina{old}In order to validate our hypothesis in a more practical environment, we conduct deepnet experiments on a subset of TinyStories \cite{?}, a simple synthetic dataset generated using GPT-4 with a simpler vocabulary, similar to that of a 3-4 year old child. We sample the first 2000 stories from the dataset and train a 4 layer transformer using AdamW \cite{?} for next token prediction (not auto-regressive). We tokens the stories with 512 unique tokens trained on the 2000 stories and use a sequence length of 6 for the training. This provides us 500K contexts with 400K of the contexts being unique. We use a exponentially decaying learning rate (starting from 5e-4) and train on the entire corpus for 300 epochs, saving the model in the process. In order to confirm our hypothesis, we compare the gram matrix of the support set for the gram matrix of features for the final model. For the comparison, we only consider 100 samples from the entire contexts encountered in the training dataset with the largest support set sizes. 

==> Arxiv_NewTempl/sections/expyize.tex <==
% \tina{@Yize, check if any details are missing} 
% \vspace{-5pt}
\subsection{Results} 
% We conduct experiments with both UFM and transformer models across different datasets. The UFM and transformer models are trained on two controlled datasets: the Synthetic dataset and the Simplified TinyStories dataset. Additionally, the transformer model is applied to a larger-scale dataset, TinyStories, to verify the geometry properties in a more complex and realistic environment.

% \yz{Yize fix, reorganize }
% \yz{Experiments on Synthetic and Simplified Tinystories datasets}
\subsubsection{Synthetic and Simplified Tinystories datasets}\label{sec:synth_res}
% \yz{I merged the synthetic dataset and simplified TinyStories because the 1. settings/metrics/figures are almost the same except for datasets and 2. I merged the loss/ssim/norm curves together. plz let me know if we have better ideas} \tina{i like merging them.}
% 
% \input{Arxiv_NewTempl/sections/figure_verysmall_heatmaps}
% {We train a 4-layer TF, with embedding dimension $d=128$ on both Synthetic and Simplified TinyStories datasets. To compare training dynamics of TFs to \ref{eq:ufm}, we also train \ref{eq:ufm} on the probability matrix $\Pbb$ of each dataset.} In all experiments, we use AdamW optimizer with a weight decay parameter of \(\lambda=10^{-6}\). The learning rate is initially set to \(10^{-4}\), with a step-decay schedule. We train the models long enough to ensure that each model approach the empirical entropy lower-bound ($\Hc= 1.6597$ for Synthetic and $\Hc= 1.0166$ for Simplified TinyStories) 
% % \tina{Yize: add the values please} 
% within an order of $10^{-4}$.

We train the models long enough to ensure approaching the empirical entropy lower-bound $\Hc$ within an order of $10^{-4}$. In all experiments, we use AdamW optimizer with a weight decay \(\lambda=10^{-6}\). The learning rate is initially set to \(10^{-4}\), with a step-decay schedule. \looseness=-1

% \subsubsection{Experiments on Simplified TinyStories Dataset}
% \subsection{Experiments on simplified TinyStories}\label{sec:synth}

% {We create an artificial setup where we have control over the structure of the training data and where it is numerically feasible to compute the optimal word and context embeddings as specified by Cor.~\ref{cor:WH}. We focus on the $T=6$-th token prediction task in this section, and we use word-level tokenization. We generate the synthetic data in two ways: 1) by manually curating a small dataset of simple sentences% {(see App. \ref{sec:synthetic_app} for details)}
% , 2) by choosing and adjusting a subset of most frequent contexts from the TinyStories \citep{eldan2023tinystories} dataset.}
% \new{We leave the details and results of the first case to the App.~\ref{sec:synthetic_app} and here we focus on the second case.}
% 
% 
% \noindent\textbf{Subset of Tiny Stories.}~
% For the second case, 
% We derive contexts $\xd_j$ and support sets $\Sc_j$ from the TinyStories dataset and we create the training data from the most frequent word-level contexts with length 5, such as $\xd_j = [\texttt{``once'', ``upon'', ``a'', ``time'', ``,''}]$. For the support sets $\Sc_j$, we record all next tokens of $\xd_j$ in the original dataset. Then, we replace the words in the contexts with their synonymous to generate new contexts with identical support sets. This allows us to have multiple contexts sharing common support sets, while controlling the vocabulary size, which is set to $V=104$. {The final dataset consists of $n\approx3050$ samples with $m\approx400$ unique contexts.} The frequencies $\pbh_j$ are determined by  independently sampling each next token from $\Sc_j$ several times.
%

In Figs.~\ref{fig:simplified_intro} and \ref{fig:synthetic_heatmap_small}, we illustrate the logits $\Lb$ and the pairwise cosine-similarity of word embeddings $\corr{\W^\top}$ and context embeddings $\corr{\Hb}$ learned by TF (column (a)) and by \ref{eq:ufm} (column (b)) at the end of training, for \simTS~and \synth~datasets respectively.
We also inspect the theoretical prediction of Thm.~\ref{thm:reg path} in Panel (c).
% so that $\Wmm{\Wmm}^\top=\GWmm$ and ${\Hmm}^\top\Hmm=\GHmm$. 
Observe that \ref{eq:ufm}, despite being a simplified abstraction of over-parameterized models, learns the same geometrical structure for both word and context embedding as that of the TF. This geometry also aligns well with that of the \ref{eq:ufm-svm} solution of Thm.~\ref{thm:reg path}. Further note the subspace collapse property in the heatmaps: The diagonal blocks on the first row, which correspond to the contexts with the same support set, consistently show the highest values, indicating full correlation of their respective embeddings. Figs.~\ref{fig:sim_H_label_verysmall} and \ref{fig:sim_H_lable_404} in the appendix visualize the text values of contexts that exhibit supspace collapse, e.g., \tina{@yize, add an example please}
Finally, column (d) shows that our proxy \ref{P proxy}, which is based on the support set similarities, is a close but less expensive alternative to the theory for capturing the overall geometry of the embeddings.\looseness=-1

% Comparing the geometric structure of the context embeddings $\corr{\Hb}$ and word embeddings $\corr{\W}$ with the correlation structures of the support sets $\corr{\smat}$ and $\corr{\smat^\top}$, we verify the observations made in the UFM experiments of Sec.~\ref{sec:ufmexp}: 1) Contexts with a larger intersection in the support set of their next-tokens roughly exhibit larger correlation in the embeddings space. 2) Words that appear as the next token of similar contexts have closer word embeddings. 

In Fig.~\ref{fig:synthetic_curves}, we display analogous plots to those in Fig.~\ref{fig:UFM_curves}. Specifically, Fig.~\ref{fig:synthetic_curves}-(a) confirms that the loss is close to the entropy lower bound. Next, Fig.~\ref{fig:synthetic_curves}-(b) confirms the norm growth of the parameters. Note the slower growth of the context embeddings $\Hb$ in the TF model, which we suspect is due to the layer normalization implemented at the final layer of the network. We also confirm the recovery of the soft labels per Thm.~\ref{thm:reg path finite} in Fig.~\ref{fig:synthetic_curves}-(c). Finally Fig.~\ref{fig:synthetic_curves}-(d) and (e) track the correlation of the learned geometries with the proxy \ref{P proxy} and with the theoretical predictions $(\Hmm,\Wmm)$. Note that all similarity metrics increase towards $1$ as training progresses. In Figs.~\ref{fig:m404steps} and \ref{fig:verysmallsteps} in the appendix, we display the evolution of the embeddings by capturing their heatmaps at various training checkpoints. Interestingly, the final patterns emerge early in the training process. 

% \new{Fig. \ref{fig:synth_ssim}also confirms that as the training continues, the similarity between the learned embeddings and the support set structures increases by measuring the similarity metric \eqref{eq:ssim}.} 
% We note that these observations are made in a regime where the loss is close to the entropy lower bound, as illustrated in Fig.~\ref{fig:syn_losses}  
% \yz{i don want to give the impression that this only happens near iteration 30k, maybe say something about "the geometry converged faster(around 3k) iterations but we trained very long to verify the loss goes to entropy", something like -- } 
% We observed that these properties begin to emerge around 3,000 iterations; however, we extended training to ensure that the losses converge towards entropy with an order of 1e-4. 

\hspace{-50pt}
% \include{Arxiv/sections/figure_synthetic_curves}
\begin{figure*}[t]% [htbp]
    \vspace{-10pt}
    \centering
    \begin{tikzpicture}
        % First row
        \node (img1) at (0,0) {\includegraphics[width=0.33\textwidth]{exp_results_yize/CElosses_all_4 layer Transformer pos off_tiny_extract_m404_d128.pdf}};
        \node (img2) at (5,0) {\includegraphics[width=0.33\textwidth]{exp_results_yize/WHnormgrowth_all_tiny_extract_m404_4 layer Transformer pos off_d128.pdf}};
        \node (img3) at (10,0) {\includegraphics[width=0.33\textwidth]{exp_results_yize/L_proj_L_fin_diff_all_4 layer Transformer pos off_tiny_extract_m404_d128.pdf}};
        
        % Second row
        \node (img4) at (2.5,-4.1)
        {\includegraphics[width=0.33\textwidth]{exp_results_yize/HW_Lmmthm_sim_structural_corr_tiny_extract_m404_4 layer Transformer pos off_d128.pdf}};
        \node (img5) at (7.5,-4.1) 
        {\includegraphics[width=0.33\textwidth]{exp_results_yize/HW_HWmm_sim_structural_corr_tiny_extract_m404_4 layer Transformer pos off_d128.pdf}};
        
        % Center-top aligned text for each figure
        \node[anchor=south, text width=0.3\textwidth, align=center, fill=white, fill opacity=1] at (0,-1.85) {\tiny Epoch$(k)$};
        \node[anchor=south, text width=3cm, align=center, fill=white, fill opacity=1] at (5,-1.85) {\tiny Epoch$(k)$};;
        \node[anchor=south, text width=3cm, align=center, fill=white, fill opacity=1] at (10,-1.85) {\tiny Epoch$(k)$};;
        \node[anchor=south, text width=0.5\textwidth, align=center, fill=white, fill opacity=1] at (2.5,-6) {\tiny Epoch$(k)$};;
        \node[anchor=south, text width=0.5\textwidth, align=center, fill=white, fill opacity=1] at (7.5,-6) {\tiny Epoch$(k)$};

        \node[anchor=south, text width=0.3\textwidth, align=center] at (0,1.4) {\textbf{(a)} Loss convergence};
        \node[anchor=south, text width=3cm, align=center] at (5,1.4) {\textbf{(b)} Norm growth};
        \node[anchor=south, text width=3cm, align=center] at (10,1.4) {\textbf{(c)} $\norm{\Qcs(\Lb_k) - \Lbin}$};
        \node[anchor=south, text width=0.5\textwidth, align=center] at (2.5,-2.8) {\textbf{(d)} Correlation with proxies};
        \node[anchor=south, text width=0.5\textwidth, align=center] at (7.5,-2.8) {\textbf{(e)} Correlation with theory};

        % Y-axis labels, rotated and centered vertically
        \node[anchor=east, rotate=90] at (-2.1,0.8) {\tiny $\text{CE}(\Lb_k)-\Hc$};
        % \node[anchor=east, rotate=90] at (3.2,0.8) {\tiny Euclidean norm};
        % \node[anchor=east, rotate=90] at (8.2,0.8) {\tiny Y-axis Label 3};
        % \node[anchor=east, rotate=90] at (1.7,-4) {\tinyY-axis Label 4};
        % \node[anchor=east, rotate=90] at (6.7,-4) {\tinyY-axis Label 5};
    \end{tikzpicture}
    % 
    \vspace{-10pt}
    \captionsetup{width=\textwidth}
    % \caption{\yz{whats wrong with this figure}}
    \caption{Numerical experiments on \synth~and \simTS~datasets. 
    \textbf{(a):} CE approaches to $\Hc$, \textbf{(b):} Norms of the parameters grow during training. \textbf{(c):} The projection of $\Lb_k$ on the data subspace $\Fc$ converges to the finite component $\Lbin$ specified by the soft-labels $\pbh_j$. \textbf{(d):} $\ssimstar{\Hb}{\smatbar}$ (solid) and $\ssimstar{\W^\top}{\smatbar^\top}$ (dashed) throughout training. At the final stage the learned embeddings exhibit high similarity with proxy. \textbf{(e):} Same as (d), this time comparing with theory, i.e., $\ssimstar{\Hb}{\Hmm}$ and $\ssimstar{\W^\top}{{\Wmm}^\top}$. See Sec.~\ref{sec:synth_res} for details.
    % \tina{@ Yize: xlabel's are not in latex so i can't change them: change xlabel to ``Epoch $k$''. } 
    }
    \label{fig:synthetic_curves}
\end{figure*} 
% 
\vspace{-5pt}
\subsubsection{TinyStories dataset}\label{sec:exp_tiny}
% To experiment on more realistic data, we train on $100$ stories sampled from TinyStories. We use a 12-layer TF with embeddings dimension $d=256$, a tokenizer with vocabulary size $V=128$, and fixed context length $T=6$. We choose a small context window and vocabulary size to make tracking the unique contexts and their support sets computationally manageable. In this setup, the number of unique contexts $m\sim 10^5$ . The model is trained with Adam optimizer for $600$ epochs. We use warm-up over the first 5 epochs to increase the learning rate to $5 \times 10^{-4}$ and use a cosine learning rate scheduler to decay its values over the course of the training. We use a weight decay of $10^{-5}$ throughout the training. \looseness=-1
% To experiment on more realistic data, we train on $100$ stories sampled from TinyStories. We use a 12-layer TF with embeddings dimension $d=256$, a tokenizer with vocabulary size $V=128$, and fixed context length $T=6$. We choose a small context window and vocabulary size to make tracking the unique contexts and their support sets computationally manageable. In this setup, the number of unique contexts $m\sim 10^5$. 
We train TF with Adam optimizer until it reaches the empirical entropy lower-bound within an order $10^{-3}$. We use warm-up over the first 5 epochs to increase the learning rate to $5 \times 10^{-4}$ and use a cosine learning rate scheduler to decay its values over the course of the training. We set the weight decay to $10^{-5}$. \looseness=-1

For visualization, we choose $10$ unique support sets in the dataset with $|\Sc_j|>2$. For each of the chosen support sets $\Sc$, we choose $10$ distinct contexts $j$ such that $\Sc_j=\Sc$ (a total of $100$ samples), and illustrate the Gram matrix of the centered support matrix $\smatbar$ and context embeddings $\Hb$ for this subset of the contexts. Given that the support sets are sparse, we choose to use those with the largest support set size which would result in a more pronounced pattern on the correlation matrices. We visualize the heatmaps in Fig.~\ref{fig:intro_TinyStories}. We skip visualizing the word embeddings $\W$, as the heatmaps did not display any noticeable visual structures. \looseness=-1

Finally, in Fig.~\ref{fig:TinyStories_curves}, we track the metrics discussed in Sec.~\ref{sec:metric}, similar to Figs.~\ref{fig:UFM_curves} and \ref{fig:synthetic_curves}. Due to the larger number of context embeddings, we only compute metrics such as $\norm{\Qcs(\Lb_k) - \Lbin}$, norm growth and correlation with proxies using a sample of $1000$ token/context pairs chosen randomly from the training set. We observe qualitatively similar behavior, with the exception of the norm growth of $\Hb$, which we conjecture to be a consequence of layer normalization in the final embedding layer. \looseness=-1








% \new{Finally, we note that the results in Thms.~\ref{thm:reg path} and \ref{thm:reg path finite} hold as long as the model is expressive enough to generate (approximately) unconstrained embeddings and the loss is minimized close to the lower-bound. To 
%  verify this, we repeat the above experiment by replacing the TF model with an MLP network. We use an MLP with \tina{XX} number of layers and width \tina{XX} with \tina{ReLU} activations. This leads to a network with \tina{$\sim10$} times more number of parameters than the TF model. We choose a larger MLP network since TF is more expressive than plain MLP. The final embeddings geometry is depicted in Fig.~\ref{fig:Sim_SHWFixedLMLP_d128}. We observe that the geometrical patterns appearing in $\corr{\Hb}$ and $\corr{\W^\top}$ are similar to those of the TF model. We conjecture that with even larger MLP, we will see better convergence to our theoretical analysis. 
%  }
%  \begin{figure}[t]
%     \centering
%     \hspace{-10mm}
%     \includegraphics[width=1.\linewidth]{exp_results_yize/Sim_SHWFixedLMLP_d128.pdf}
%     \captionsetup{width=\linewidth}
%     \caption{\yz{fix:remove title, fix colorbar. }Embedding geometries trained by MLP. \\Left: Geometry Comparison between $S$ and $\Hb$; right: Geometry comparison between $S^T$ and $W^T$.
%     % \tina{Why are we comparing the mlp embeddings with S here? what's our message? mlp if large enough finds similar embeddings to TF? or it minimizes the loss and finds the theoretical prediction? Then, we should either compare with TF or theory heatmaps here. Or is there some other point we can make by directly comparing with S?}  \yz{I kinda wanted to state that MLP does not work as well as transformer, but you are right. I'm not sure what the messages here. do you have a preference?}
%     }
%     \label{fig:Sim_SHWFixedLMLP_d128}
% \end{figure}
%on the smaller synthetic dataset.
% For similar plots on the small synthetic data see Sec.~\ref{sec:synthetic_app} in the App.
% \new{We compare $\W_k$, $\Hb_k$ and $\Lb_k$ learned by TF with those learned by UFM. We also inspect the theoretical prediction of Thm.~\ref{thm:reg path}: we find the optimal solution $\Lbmm$ of \ref{eq:ufm-svm} using CVXPY \citep{diamond2016cvxpy}, and find $\Wmm$ and $\Hmm$ as in Cor.~\ref{cor:WH} so that $\Wmm{\Wmm}^\top=\GWmm$ and ${\Hmm}^\top\Hmm=\GHmm$. 
% We show the evolution of $\Lb_k$ and the pairwise similarity of $\W_k$ and $\Hb_k$ as training progresses in Fig.~\ref{}. 
% 
% In Fig.~\ref{fig:syn_heatmaps_w}, for the dataset curated from Tiny Stories, we illustarte the pairwise cosine-similarity of the word and context embeddings for TF and UFM at the final training iteration, as well as the pairwise similarity of the max-margin solutions $\Wmm$ and $\Hmm$. We observe that, despite UFM being an abstarct model of over-parameterized models, both UFM and TF learn the same geometrical structure for both word and context embedding. This geometry aligns well with that of the max-margin solution of Thm.~\ref{thm:reg path}. Comparing the geometric structure of $\Hb$ (resp. $\W$) with the column-wise (resp. row-wise) pairwise similarity of the support matrix $\smat$, we have a similar observation to the UFM experiments of Sec.~\ref{sec:ufmexp}: 1) Two contexts that have a larger intersection in the support set of their next tokens exhibit larger correlation in the embeddings space. 2) Two words that appear as the next token of similar contexts have closer word embeddings. We note that this observation is made in a regime where the loss is close to the entropy lower bound, as illustrated in Fig.~\ref{fig:syn_losses} in App. For similar plots on the small synthetic data see Sec.~\ref{sec:synthetic_app} App.
% 
% As predicted by Thm.~\ref{thm:reg path} \tina{this is on reg path...}, the optimal direction of UFM parameters is characterized by the SVD factors of $\Lbmm$. Furthermore, despite UFM being an abstarct model of over-parameterized models, we observe that TF recovers the same geometry for the word and context embeddings. We also observe high correlation between the pairwise similarity of embeddings with that of support sets: At a high level, for a given sample $j\in[m]$, the corresponding embedding has higher correlation with those samples $j'$ whose support set intersection $|\Sc_j\cap \Sc_{j'}|$ is larger \tina{this might not be always true}. Specifically, for those contexts that share the same support set $\Sc_j=\Sc$, the learned context embeddings collapse, as observed on the diagonal blocks of $\Hb_k^\top\Hb_k$. Similarly, the word embeddings of two tokens are closer if they appear together in more support sets.\tina{copied from UFM section} 
% For the loss and norm plots, see App. \tina{shall we have loss and norm plots in the App?}
% }
% \subsubsection{Result}
% We present the following result on UFM and the transformer model: 
% \begin{enumerate}[label=\arabic*., font=\bfseries,leftmargin=*]
% \item \textbf{The convergence of loss to empirical entropy. (Figure \ref{fig:syn_losses})}
% To verify the loss convergence to the lower bound, as stated in \ref{sec:ce_h}, \ref{thm:reg path app}, we evaluate the difference between the Cross Entropy loss and the empirical entropy, ie. $(\CE({\thetab_t}) - \ent)$ and plot it along training epochs. We observed that the Cross Entropy loss converged towards the empirical entropy in the order of $10^{-4}$.
% % \subsubsection{Convergence to Max-Margin Solution}
% % The second metric, illustrated in Figure Y, involved evaluating the trained embeddings' convergence towards the max-margin solution. This solution was derived by addressing the minimum nuclear norm problem [min nuclear norm] and employing SVD factorization [SVD eqn]. The y-axis in this plot measured GH-GHmm, representing the difference between the normalized embedding trained by the model and the normalized Hmm value.  
% % % Additionally, we noted that the logits, gram matrix of weights, converged towards max-margin solution L and the gram of Wmm
% \item \textbf{The norm increase of both $W$ and $H$ during training. (Figure \ref{fig:syn_normincrease})}
% We verify the norm of $W$ and $H$ increase for both UFM and transformer models. 
% \item  \textbf{Similarity between trained logits and Max-Margin solution.(Figure \ref{fig:syn_logits})}
% We visualize the logits, $L$, trained by both models on two synthetic datasets, and compare them with the max-margin solution obtained by solving the nuclear norm minimization problem described in Corollary \ref{eq:ufm-svm}. The max-margin solution is computed using CVXPY. We show that the logits trained by both UFM and transformer have a similar pattern to the max-margin solution, particularly considering the on-support entries. 
% \item  \textbf{Embedding Geometry. (Figure \ref{fig:syn_heatmaps_h})}
% We visualize the pairwise similarities of the embeddings in a heat map, ie. $ \cosa{\hb_j}{\hb_{j'}}$, for $ j, j'\in[m]$ and comparing them to  1.the pairwise similarity of the supports,$ \cosa{\smat_j}{\smat_{j'}}$, where $\smat\in\{0,1\}^{V\times m}$, and 2. the pairwise similarities of the basis of max-margin solution of H, $\Hb_{mm}$, solved by SVD of $L_{mm}$, described in \ref{cor:WH}. 
% This visualization illustrated that for both the transformer and UFM models, the embedding geometry of the context was closely aligned with the max-margin solution, and their respective support sets. Specifically,  a higher overlap in support sets corresponded to greater similarity within their embedding space.
% \end{enumerate}
% \input{Arxiv/sections/figure_synthetic_heatmaps_h}
% \input{Arxiv/sections/figure_synthetic_heatmaps_w}
% \input{Arxiv/sections/figure_syn_losses}
% \input{Arxiv/sections/figure_logits}
% \input{Arxiv/sections/figure_m404_heatmaps}
% % \subsubsection{Result}
% % We present the following result on UFM and 2-layer transformer model: 
% % \begin{enumerate}
% %     \item The Cross Entropy loss converges to the lower bound of the entropy. (Figure \ref{fig:loss_ufm_tfm})
% %     % \item 
% %     \item The logits, gram matrix of Embeddings and Weights, converge to $L_mm$ and the gram of $W_{mm}$ and $H_{mm}$. (Figure \ref{fig:ufm_matrix}, \ref{fig:tfm_matrix}) 
% %     \item The embedding geometry of the context is closely related to their support set for both transformer and UFM. More specifically, the higher overlap between the support sets indicates a higher similarity in their embedding space. (Figure \ref{fig:ufm_support}, \ref{fig:tfm_support})
% % % \end{enumerate}
% % \begin{figure}[h!]
% %     \centering 
% %     \includegraphics[width=\linewidth]{exp_results_yize/CE losses ufm tfm.png}  
% % \captionsetup{width=\textwidth}
% %     \caption{The plots show the difference between Cross Entropy loss and empirical entropy decreases during training. Note that the y-axis evaluates the $(\CE({\thetab_t}) - \ent)$ and the x axis is the iteration steps. }
% %     \label{fig:loss_ufm_tfm}
% % \end{figure}
% % \begin{figure}[h!]
% %     \centering 
% %     \includegraphics[width=\linewidth]{exp_results_yize/Matrices_UFM.png}  
% % \captionsetup{width=\textwidth}
% %     \caption{The Convergence of UFM model to Max-Margin solutions. Left: The comparison between model logits and $L_{mm}$; Middle: The comparison between the gram matrix of trained Embeddings and $GH_{mm}$; Right: The comparison between the gram matrix of trained Classifier and $GW_{mm}$}
% %     \label{fig:ufm_matrix}
% % \end{figure}
% % \begin{figure}[h!]
% %     \centering 
% %     \includegraphics[width=\linewidth]{exp_results_yize/Matrices_2 layer Transformer.png}  
% % \captionsetup{width=\textwidth}
% %     \caption{The Convergence of 2-layer transformer to Max-Margin Solutions. Left: The comparison between model logits and $L_{mm}$; Middle: The comparison between the gram matrix of trained Embeddings and $GH_{mm}$; Right: The comparison between the gram matrix of trained Classifier and $GW_{mm}$}
% %     \label{fig:tfm_matrix}
% % \end{figure}
% % \begin{figure}[h!]
% %     \centering 
% %     \includegraphics[width=\linewidth]{exp_results_yize/Suppot_sim_UFM.png}  
% % \captionsetup{width=\textwidth}
% %     \caption{The positive correlation between the overlap in support set and similarity between pairs of logits and embeddings, in trained UFM model. Left: The cosine similarities between logits. Middle: The cosine similarities between embeddings. Right: The number of overlaps between support sets. Note that both vertical and horizontal indexes indicate m unique contexts in synthetic dataset. }
% %     \label{fig:ufm_support}
% % \end{figure}
% % \begin{figure}[h!]
% %     \centering 
% %     \includegraphics[width=\linewidth]{exp_results_yize/Suppot_sim_2 layer Transformer.png}  
% % \captionsetup{width=\textwidth}
% %     \caption{The positive correlation between the overlap in support set and similarity between pairs of logits and embeddings, in trained 2 layer Transformer model. Left: The cosine similarities between logits. Middle: The cosine similarities between embeddings. Right: The number of overlaps between support sets. Note that both vertical and horizontal indexes indicate the m unique contexts in synthetic dataset.}
% %     \label{fig:tfm_support}
% % \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \subsubsection{Dataset}\label{sec:expyz}
% % \textbf{Synthetic Text dataset}
% % To demonstrate the theory on text data, a toy language dataset is constructed as follows: we manually select five word-level tokens, referred to as one context, and we come up with some corresponding 6th tokens that align with the given context, referred to as the support sets. The dataset comprises 16 distinct contexts $(m=16)$, with a fixed support set length of 3 $(\Sc_{j}=3$ for $j\in[m])$. Each support is then sampled independently to a number of repeats to emulate the behavior of repeated context in natural language.
% % %[These support sets were independently sampled and repeated to mimic common occurrences of context in natural language.]
% % The primary task involved predicting the sixth token based on the preceding five-token context. For instance, given the context "Lily wants to try the", the model might predict words such as ["soup", "game", "movie"], based on the frequencies and probabilities [8, 4, 4] and [0.5, 0.25, 0.25] respectively. The distribution of these support sets is detailed in Figure \ref{fig:verysmalldataset}.
% % \textbf{Context Extracted from TinyStories}
% % The second dataset was derived from a subset of "TinyStories" dataset, aiming to test the theory in a larger and more realistic setting. This dataset was selected from the most frequent word-level contexts with length 5, such as "once", "upon", "a", "time" ",". We recorded all subsequent tokens as the support set for each context. To increase the number of contexts without increasing the vocabulary size, we replace the words in the contexts with their synonymous to generate new contexts with similar or identical support sets. This approach allowed us to observe collapse of contexts, wherein different contexts share common support sets. The sampling of repeats and next token probabilities was conducted in a manner similar to the smaller synthetic text dataset. We posit that this TinyStories-based dataset offers a more accurate representation of real-world data due to its derivation from genuine text sources and the inclusion of naturally occurring contexts and support sets.
% % \subsubsection{Model}
% % \textbf{UFM}
% % We first focused on the Unconstrained Feature Model (UFM). The primary goal was to examine the embedding behavior in conjunction with real text supports. Specifically, when training the UFM, we keep the embeddings unconstrained, and use real supports as the training labels. The model's embedding dimension was configured at d=128.
% % \textbf{Transformer}
% % We then extended our experiment to an over-parameterized 4-layer transformer model, with a dimension of d=128. This exploration was guided by the hypothesis that the over-parameterized language model would exhibit behavior analogous to the UFM, thus aligning with our analytical findings.
% % % \subsubsection{Training}
% % The AdamW optimizer was employed for gradient descent, coupled with a step-decay learning rate for the training process. The models are trained for 30k iterations. 
% % \subsubsection{Result}
% % We present the following result on UFM and the transformer model: 
% % \begin{enumerate}[label=\arabic*., font=\bfseries,leftmargin=*]
% % \item \textbf{The convergence of loss to empirical entropy. (Figure \ref{fig:syn_losses})}
% % To verify the loss convergence to the lower bound, as stated in \ref{sec:ce_h}, \ref{thm:reg path app}, we evaluate the difference between the Cross Entropy loss and the empirical entropy, ie. $(\CE({\thetab_t}) - \ent)$ and plot it along training epochs. We observed that the Cross Entropy loss converged towards the empirical entropy in the order of $10^{-4}$.
% % % \subsubsection{Convergence to Max-Margin Solution}
% % % The second metric, illustrated in Figure Y, involved evaluating the trained embeddings' convergence towards the max-margin solution. This solution was derived by addressing the minimum nuclear norm problem [min nuclear norm] and employing SVD factorization [SVD eqn]. The y-axis in this plot measured GH-GHmm, representing the difference between the normalized embedding trained by the model and the normalized Hmm value.  
% % % % Additionally, we noted that the logits, gram matrix of weights, converged towards max-margin solution L and the gram of Wmm
% % \item \textbf{The norm increase of both $W$ and $H$ during training. (Figure \ref{fig:syn_normincrease})}
% % We verify the norm of $W$ and $H$ increase for both UFM and transformer models. 
% % \item  \textbf{Similarity between trained logits and Max-Margin solution.(Figure \ref{fig:syn_logits})}
% % We visualize the logits, $L$, trained by both models on two synthetic datasets, and compare them with the max-margin solution obtained by solving the nuclear norm minimization problem described in Corollary \ref{eq:ufm-svm}. The max-margin solution is computed using CVXPY. We show that the logits trained by both UFM and transformer have a similar pattern to the max-margin solution, particularly considering the on-support entries. 
% % \item  \textbf{Embedding Geometry. (Figure \ref{fig:syn_heatmaps})}
% % We visualize the pairwise similarities of the embeddings in a heat map, ie. $ \cosa{\hb_j}{\hb_{j'}}$, for $ j, j'\in[m]$ and comparing them to  1.the pairwise similarity of the supports,$ \cosa{\smat_j}{\smat_{j'}}$, where $\smat\in\{0,1\}^{V\times m}$, and 2. the pairwise similarities of the basis of max-margin solution of H, $\Hb_{mm}$, solved by SVD of $L_{mm}$, described in \ref{cor:WH}. 
% % This visualization illustrated that for both the transformer and UFM models, the embedding geometry of the context was closely aligned with the max-margin solution, and their respective support sets. Specifically,  a higher overlap in support sets corresponded to greater similarity within their embedding space.
% % \end{enumerate}
% % \input{Arxiv/sections/figure_synthetic_heatmaps}
% % \input{Arxiv/sections/figure_syn_losses}
% % \input{Arxiv/sections/figure_logits}
% % % \subsubsection{Result}
% % % We present the following result on UFM and 2-layer transformer model: 
% % % \begin{enumerate}
% % %     \item The Cross Entropy loss converges to the lower bound of the entropy. (Figure \ref{fig:loss_ufm_tfm})
% % %     % \item 
% % %     \item The logits, gram matrix of Embeddings and Weights, converge to $L_mm$ and the gram of $W_{mm}$ and $H_{mm}$. (Figure \ref{fig:ufm_matrix}, \ref{fig:tfm_matrix}) 
% % %     \item The embedding geometry of the context is closely related to their support set for both transformer and UFM. More specifically, the higher overlap between the support sets indicates a higher similarity in their embedding space. (Figure \ref{fig:ufm_support}, \ref{fig:tfm_support})
% % % % \end{enumerate}
% % % \begin{figure}[h!]
% % %     \centering 
% % %     \includegraphics[width=\linewidth]{exp_results_yize/CE losses ufm tfm.png}  
% % % \captionsetup{width=\textwidth}
% % %     \caption{The plots show the difference between Cross Entropy loss and empirical entropy decreases during training. Note that the y-axis evaluates the $(\CE({\thetab_t}) - \ent)$ and the x axis is the iteration steps. }
% % %     \label{fig:loss_ufm_tfm}
% % % \end{figure}

% % % \begin{figure}[h!]
% % %     \centering 
% % %     \includegraphics[width=\linewidth]{exp_results_yize/Matrices_UFM.png}  
% % % \captionsetup{width=\textwidth}
% % %     \caption{The Convergence of UFM model to Max-Margin solutions. Left: The comparison between model logits and $L_{mm}$; Middle: The comparison between the gram matrix of trained Embeddings and $GH_{mm}$; Right: The comparison between the gram matrix of trained Classifier and $GW_{mm}$}
% % %     \label{fig:ufm_matrix}
% % % \end{figure}
% % % \begin{figure}[h!]
% % %     \centering 
% % %     \includegraphics[width=\linewidth]{exp_results_yize/Matrices_2 layer Transformer.png}  
% % % \captionsetup{width=\textwidth}
% % %     \caption{The Convergence of 2-layer transformer to Max-Margin Solutions. Left: The comparison between model logits and $L_{mm}$; Middle: The comparison between the gram matrix of trained Embeddings and $GH_{mm}$; Right: The comparison between the gram matrix of trained Classifier and $GW_{mm}$}
% % %     \label{fig:tfm_matrix}
% % % \end{figure}
% % % \begin{figure}[h!]
% % %     \centering 
% % %     \includegraphics[width=\linewidth]{exp_results_yize/Suppot_sim_UFM.png}  
% % % \captionsetup{width=\textwidth}
% % %     \caption{The positive correlation between the overlap in support set and similarity between pairs of logits and embeddings, in trained UFM model. Left: The cosine similarities between logits. Middle: The cosine similarities between embeddings. Right: The number of overlaps between support sets. Note that both vertical and horizontal indexes indicate m unique contexts in synthetic dataset. }
% % %     \label{fig:ufm_support}
% % % \end{figure}
% % % \begin{figure}[h!]
% % %     \centering 
% % %     \includegraphics[width=\linewidth]{exp_results_yize/Suppot_sim_2 layer Transformer.png}  
% % % \captionsetup{width=\textwidth}
% % %     \caption{The positive correlation between the overlap in support set and similarity between pairs of logits and embeddings, in trained 2 layer Transformer model. Left: The cosine similarities between logits. Middle: The cosine similarities between embeddings. Right: The number of overlaps between support sets. Note that both vertical and horizontal indexes indicate the m unique contexts in synthetic dataset.}
% % %     \label{fig:tfm_support}
% % % \end{figure}

% \begin{figure*}[t]%[htbp]
% % \vspace{-30pt}
%     \hspace{0pt} \begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0,-1.4) 
% 			{\includegraphics[scale=0.2]{New_Figures_TinyStories/FinalCameraReady/Paper_LossMinusEntropy_plots_numSam_1000e_470_V7_ctxLen6_voc64_dim512_numStories100_Test.jpg}};
%             \node at (0.1,-0.0) [scale=0.8]{\textbf{(a)} Loss convergence};
%             \node at (-2.1,-1.5) [scale=0.8, rotate=90]{$\text{CE}(\Lb_k)-\Hc$};
%             \node at (0.2,-2.7) [scale=0.6]{Epoch ($k$)};
% 		\end{tikzpicture}
%     \end{subfigure}
%     \hspace{-0pt} \begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0,-1.4) 
% 			{\includegraphics[scale=0.2]{New_Figures_TinyStories/FinalCameraReady/Paper_NormGrowth_plots_numSam_1000e_598_V7_ctxLen6_voc64_dim512_numStories100_Test.jpg}};
%             \node at (0.2,-2.7) [scale=0.6]{Epoch ($k$)};
%             \node at (0.1,0.0) [scale=0.75]{\textbf{(b)} Norm growth};
% 		\end{tikzpicture}
%     \end{subfigure}
%     \hspace{-0pt} \begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0,-1.4) 
% 			{\includegraphics[scale=0.2]{New_Figures_TinyStories/FinalCameraReady/Paper_L_proj_to_L_in_plots_numSam_1000e_598_V7_ctxLen6_voc64_dim512_numStories100_Test.jpg}};
%             \node at (0.1,0.0) [scale=0.75]{\textbf{(c)} $\norm{\Qcs(\Lb_k) - \Lbin}$};
%             \node at (0.2,-2.7) [scale=0.6]{Epoch ($k$)};
% 		\end{tikzpicture}
%     \end{subfigure}
%     \hspace{-0pt} \begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0,-1.4) 
% 			{\includegraphics[scale=0.2]{New_Figures_TinyStories/FinalCameraReady/Paper_SSIM_H_W_FullS_Conject_plots_numSam_1000e_598_V7_ctxLen6_voc64_dim512_numStories100_Test.jpg}};
%             \node at (0.1,0.0) [scale=0.75]{\textbf{(d)} Correlation with proxies};
%              \node at (0.2,-2.7) [scale=0.6]{Epoch ($k$)};
% 		\end{tikzpicture}
%     \end{subfigure}
% 	% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \vspace{-10pt}
%     \captionsetup{width=\textwidth}
%     \caption{
%     Similar to Fig.~\ref{fig:UFM_heatmap}, this time on a 12-layer TF trained on a subset of $100$ stories from the \TS~dataset. \looseness=-1 %Here, computing the theoretical prediction $\Hmm$ is computationally expensive. Thus, we compare the embeddings geometry with the proxy. See Sec.~\ref{sec:exp_tiny} for details.  
%     % 
%     % 
%      % Embeddings' geometry correlates with the structural properties of text data as captured by the sparsity pattern of the support set of distinct contexts within the dataset: $12$-layer transformer (TF) trained on a subset of $1000$ stories from the Tiny Stories \citep{eldan2023tinystories}. \textbf{(Left)} Loss approaches the empirical entropy $\Hc$ of the dataset. \textbf{(Middle)} The intersection between the support sets of $100$ contexts in the dataset. Entry $(i,j)$ equals $|\Sc_j\cap\Sc_i|$, where $\Sc_i$ is the set of possible next tokens for the $i$-th context. \textbf{(Right)} Gram matrix of the corresponding $100$ context embeddings $\Hb$ learned by the TF. Contexts that share a larger common set of next tokens, are arranged closer to each other in the embedding space. Contexts that share the exact same support set, i.e., $\Sc_j=\Sc_i$, approximately align with each other (observed on the diagonal blocks). See text for details. \tina{@Vala: Christos: ``in app, do you think is good idea to add a visualization of $\smat$ (or at least part of it) to give sense of the sparsity patterns?''}
%     }
% 	\label{fig:TinyStories_curves} 
% 	% \vspace{-15pt}
% \end{figure*}









==> Arxiv_NewTempl/sections/figure_UFM_conv.tex <==

% \begin{figure*}[t]
% 	\vspace{-10pt}
% 	\centering
% 	\hspace{-0pt} \begin{subfigure}{0.45\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0,-1.4) 
% 			{\includegraphics[scale=0.3]{figures/UFM_P.pdf}};
% 			\node at (-0,-.3) [scale=0.9]{$\mathbf{P}$};
% 		\end{tikzpicture}
%     \end{subfigure}
%     \hspace{-3pt}\begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (0,-1.4) {\includegraphics[scale=0.3]{figures/UFM_loss.pdf}};
% 			\node at (0,-.3) [scale=0.9]{$\mathbf{\Lc(\W_k,\Hb_k) - \Hc}$};
% 			\node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
% 	\end{subfigure}\hspace{13pt}\begin{subfigure}{0.24\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (0,-1.4) {\includegraphics[scale=0.3]{figures/UFM_norm.pdf}};
% 			\node at (0,-.3) [scale=0.9]{\textbf{Norms}};
% 			\node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
% 	\end{subfigure}\vspace{-10pt}
% 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
% 	\vspace{15pt}
% 	\centering
% 	\hspace{-0pt} \begin{subfigure}{0.22\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-1.4,-1.4)
% 			{\includegraphics[scale=0.3]{figures/UFM_Lconv.pdf}};
% 			\node at (-1.4,-.3) [scale=0.9]{$\|{\frac{\Lbo_k}{\|\Lbo_k\|_*} - \frac{\Lbmm}{\norm{\Lbmm}_*}}$};
% 			\node at (-1.4,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
% 	\end{subfigure}\hspace{13pt}\begin{subfigure}{0.22\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (0,-1.4) {\includegraphics[scale=0.3]{figures/UFM_Linconv.pdf}};
% 			\node at (0,-0.3) [scale=0.9]{$\norm{\Qcs(\Lb_k) - \Lbin}_F$};
% 			\node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
% 	\end{subfigure}\hspace{13pt}\begin{subfigure}{0.22\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (0,-1.4) {\includegraphics[scale=0.3]{figures/UFM_Wconv.pdf}};
% 			\node at (0,-0.3) [scale=0.9]{$\|\frac{\W_k\W_k^\top}{\|\W_k\W_k^\top\|_F}\| - \frac{\GW^*}{\|\GW^*\|}$};
% 			\node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
% 	\end{subfigure}\hspace{13pt}
% 	 \begin{subfigure}{0.22\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (0,-1.4)
% 			{\includegraphics[scale=0.3]{figures/UFM_Hconv.pdf}};
% 			\node at (0,-0.3) [scale=0.9]{$\|\frac{\Hb_k\Hb_k^\top}{\|\Hb_k\Hb_k^\top\|_F}\| - \frac{\GH^*}{\|\GH^*\|}$};
% 			\node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}%\vspace{-0.2cm}
% 	\end{subfigure}
%     \vspace{-5pt}
%     \caption{UFM convergence plots for random P \tina{if we're to keep this: fix label font size, log-scale, titles, legends, train for longer, colors} \tina{need to explain Lmm by cvxpy or closed form?} \tina{fix normalization of L convergenec} \tina{keep convergence of projection? or original ones? or both?}\tina{swap P and S in the two figures}}
% 	\label{fig:UFM_conv}
% %	\vspace{-5pt}
% \end{figure*}




\begin{figure*}[t]
	\vspace{-10pt}
	\centering
	\hspace{-0pt} \begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (-0,-1.4) 
			{\includegraphics[scale=0.3]{figures/UFM_P.pdf}};
			\node at (-0.5,-.3) [scale=0.9]{$\mathbf{P}$};
			\node at (-3.1,-1.3) [scale=0.7]{${V}$};
			\node at (-0.5,-2.6) [scale=0.7]{${m}$};
   
			\node at (-0.5,-3.) [scale=0.9]{\textbf{\textcolor{white}{(a)}}};
		\end{tikzpicture}
    \end{subfigure}
    \hspace{-0pt}
    \begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.3]{figures/UFM_Lmm.pdf}};
			\node at (0,-.3) [scale=0.9]{$\Lbmm$};
			% \node at (-3.1,-1.3) [scale=0.7]{${V}$};
			\node at (-0.5,-2.6) [scale=0.7]{${m}$};
   
			\node at (-0.5,-3.) [scale=0.9]{\textbf{(a)}};
		\end{tikzpicture}
	\end{subfigure}
    \hspace{-0pt}
    \begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.3]{figures/UFM_Lin.pdf}};
			\node at (0,-.3) [scale=0.9]{$\Lbin$};
			% \node at (-3.1,-1.3) [scale=0.7]{${V}$};
			\node at (-0.5,-2.6) [scale=0.7]{${m}$};
			\node at (-0.5,-3.) [scale=0.9]{\textbf{\textcolor{white}{(a)}}};
		\end{tikzpicture}
	\end{subfigure}\vspace{-0pt}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
	\vspace{12pt}
    \begin{subfigure}{0.33\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.33]{figures/UFM_norm.pdf}};
			\node at (0,-0.1) [scale=0.7]{\textbf{Norms}};
			\node at (0,-2.6) [scale=0.7]{Epoch ($k$)};
			\node at (-0.,-3.) [scale=0.9]{\textbf{\textcolor{black}{(b)}}};
		\end{tikzpicture}
	\end{subfigure}\hspace{-10pt}
	\centering
	\hspace{-10pt} \begin{subfigure}{0.33\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (-1.4,-1.4)
			{\includegraphics[scale=0.33]{figures/UFM_HWLconv.pdf}};
			\node at (-1.2,-.1) [scale=0.7]{\textbf{Directional distance to optimal }};
			\node at (-1.4,-2.6) [scale=0.7]{Epoch ($k$)};
			\node at (-1.4,-3.) [scale=0.9]{\textbf{\textcolor{black}{(c)}}};
		\end{tikzpicture}
	\end{subfigure}\hspace{-10pt}
    \begin{subfigure}{0.33\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.33]{figures/UFM_Linconv.pdf}};
			\node at (0,-.1) [scale=0.7]{$\norm{\Qcs(\Lb_k) - \Lbin}$};
			\node at (0,-2.6) [scale=0.7]{Epoch ($k$)};
   
			\node at (-0.,-3.) [scale=0.9]{\textbf{\textcolor{black}{(d)}}};
		\end{tikzpicture}
	\end{subfigure}
    \vspace{-5pt}
    \captionsetup{width=\linewidth}
    \caption{
    UFM trained on randomly-generated soft-probability labels matrix: \textbf{(a)} A realization of the soft-labels $\Pbb$, \ref{eq:ufm-svm} solution $\Lbmm$ that depends on the support matrix $\Sb$, and the unique finite component of the optimal solution $\Lbin\in\Ts$ that satisfies \NTPH-compatibility  constraints. \textbf{(b)} The parameters grow in norm as training continues, \textbf{(c)} While growing in norm, the logits $\Lb_k$ converge asymptotically in direction to $\Lbmm$ and $\W_k\W_k^\top$, $\Hb_k^\top\Hb_k$ converge to $\GWmm$ and $\GHmm$ that are specified by the SVD factors of $\Lbmm$, \textbf{(d)} the projection of $\Lb_k$ on subspace $\Ts$ \eqref{eq:subspace} converges to the unique solution $\Lbin$ in $\Ts$. See text, Thms.~\ref{thm:reg path},\ref{thm:reg path finite} and Cor.~\ref{cor:WH} for details. 
    % 
    % UFM trained on randomly-generated soft-probability labels matrix $\mathbf{P}$: \textbf{(Top row)} The loss converges to the entropy $\Hc$. \textbf{(Bottom row)} 1) As predicted by Thm.~\ref{thm:reg path finite}, the projection of the optimal solution on subspace $\Ts$ \eqref{eq:subspace} converges to the unique solution $\Lbin$ in $\Ts$ that satisfies the \NTPH-compatibility  constraints (see Defn. \ref{def:NTP-comp}), 2) While the norm of the parameters grows during training, $\mathbf{G}_\mathbf{W_k}$, $\mathbf{G}_\mathbf{H_k}$ and $\Lb_k$ asymptotically converge in direction to the prediction of Thm.~\ref{thm:reg path}. The direction only depends on the sparsity pattern of the support matrix $\smat$. See text for details. 
    % % \tina{if we're to keep this: fix label font size, log-scale, titles, legends, train for longer, colors} \tina{need to explain Lmm by cvxpy or closed form?} \tina{fix normalization of L convergenec} \tina{keep convergence of projection? or original ones? or both?}\tina{swap P and S in the two figures}
    }
	\label{fig:UFM_conv}
%	\vspace{-5pt}
\end{figure*}

==> Arxiv_NewTempl/sections/figure_UFM_heatmaps.tex <==

\begin{figure*}[t]
	\vspace{-5pt}
	\centering
	\hspace{-0pt} \begin{subfigure}{0.9\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
   {\includegraphics[scale=0.152]{figures/UFM_Lheatmap.pdf}};
			\node at (-5.8,0.8) [scale=0.6]{Epoch 0};
			\node at (-3.3,0.8) [scale=0.6]{Epoch 40};
   
			\node at (-3.3,1.4) [scale=0.8]{\textbf{(a) Training checkpoints}};
			\node at (2.4,1.4) [scale=0.8]{\textbf{(b) Theory}};
			\node at (5.5,1.4) [scale=0.8]{\textbf{(c) Proxy}};
   
			\node at (-0.8,0.8) [scale=0.6]{Epoch 10000};
			\node at (2.4,0.8) [scale=0.6]{$\Lbmm$};
			\node at (5.5,0.8) [scale=0.6]{$\smat$};
			\node at (-7.5,0.0) [scale=0.6, rotate=90]{$\Lb$};
   % \draw[black, dashed, line width=1pt] (1.5,1.2) -- (1.5,0);
		\end{tikzpicture}
    \end{subfigure}\vspace{-10pt}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
	\vspace{7pt}
	\centering
	\hspace{5pt} \begin{subfigure}{0.9\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.16]{figures/UFM_Wheatmap.png}};
			% {\includegraphics[scale=0.16]{figures/UFM_Wheatmap_norm.png}};
   {\includegraphics[scale=0.15]{figures/UFM_Wheatmap2.pdf}};
			% \node at (-0,-.3) [scale=0.8]{$\mathbf{P}$};
   \node at (-5.8,1.4) [scale=0.6]{Epoch 0};
			\node at (-3.3,1.4) [scale=0.6]{Epoch 40};
			\node at (-0.8,1.4) [scale=0.6]{Epoch 10000};
			\node at (2.4,1.4) [scale=0.6]{$\corr{{\Wmm}^\top}$};
			\node at (5.6,1.4) [scale=0.6]{$\corr{\smat^\top}$};
			\node at (-7.45,0.0) [scale=0.6, rotate=90]{$\corr{\W^\top}$};
		\end{tikzpicture}
    \end{subfigure}\vspace{-10pt}

    \vspace{7pt}
	\centering
	\hspace{15pt} \begin{subfigure}{0.9\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.16]{figures/UFM_Hheatmap.png}};
			% {\includegraphics[scale=0.16]{figures/UFM_Hheatmap_norm.png}};
   {\includegraphics[scale=0.15]{figures/UFM_Hheatmap2.pdf}};
			% \node at (-0,-.3) [scale=0.8]{$\mathbf{P}$};
      \node at (-5.8,1.4) [scale=0.6]{Epoch 0};
			\node at (-3.3,1.4) [scale=0.6]{Epoch 40};
			\node at (-0.8,1.4) [scale=0.6]{Epoch 10000};
			\node at (2.4,1.4) [scale=0.6]{$\corr{{\Hmm}}$};
			\node at (5.6,1.4) [scale=0.6]{$\corr{{\smat}}$};
			\node at (-7.4,0.0) [scale=0.6, rotate=90]{$\corr{\Hb}$};
            % \node at (-3.3,-1.6) [scale=0.8]{\textbf{(a)}};
            % \node at (2.4,-1.6) [scale=0.8]{\textbf{(b)}};
            % \node at (5.6,-1.6) [scale=0.8]{\textbf{(c)}};
		\end{tikzpicture}
    \end{subfigure}
    \begin{tikzpicture}[remember picture,overlay]
        % \draw[red, thick] (current page.north) -- (current page.south);
        
   \draw[black, line width=2pt] (-6.25,8.8) -- (-6.25,0.15);
      \draw[black, line width=2pt] (-2.85,8.8) -- (-2.85,0.15);
   
    \end{tikzpicture}

  %   \vspace{15pt}
  %   \hspace{45pt}
  %   \begin{subfigure}{0.45\textwidth}
		% \centering
		% \begin{tikzpicture}[remember picture]
		% 	\node at (-0,-0) 
		% 	% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
  %           {\includegraphics[scale=0.45]{figures/UFM_loss.pdf}};
			
		% 	\node at (0.2,1.6) [scale=0.8]{Loss convergence};
  %          \node at (-2.8,0.2) [scale=0.8, rotate=90]{$\text{CE}(\Lb_k)-\Hc$};
  %            \node at (0.2,-1.6) [scale=0.6]{epoch $(k)$};
  %           \node at (0.2,-2.1) [scale=0.8]{\textbf{(d)}};
		% \end{tikzpicture}
  %   \end{subfigure}
  %   % 
  %   \hspace{-20pt}
  %   \begin{subfigure}{0.45\textwidth}
		% \centering
		% \begin{tikzpicture}[remember picture]
		% 	\node at (-0,-0) 
		% 	% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
  %           {\includegraphics[scale=0.45]{figures/UFM_SSIM.pdf}};
			
		% 	\node at (0.3,1.6) [scale=0.75]{Structural correlation with $\Sb$};
  %            \node at (0.2,-1.6) [scale=0.6]{epoch ($k$)};
  %           \node at (0.2,-2.1) [scale=0.8]{\textbf{(e)}};
		% \end{tikzpicture}
  %   \end{subfigure}
    \vspace{-0pt}
	\vspace{-0pt}
 \captionsetup{width=\linewidth}
 \vspace{-5pt}
    \caption{Evolution of UFM parameters $\Lb_k$, $\corr{\W_k^\top}$ and $\corr{\Hb_k}$ when training close to convergence to the empirical entropy $\Hc$ (See Fig.~\ref{fig:UFM_curves}). At the end of the training, the parameters align with the prediction of Thm.~\ref{thm:reg path} ((a) vs (b)). Additionally, the correlation patterns between the embeddings closely follows the similarities between the support sets ((a) vs (c)). \tina{replace with centered S?} %We verify the similarity between the optimal embedding geometry and the support sets by measuring $\ssim{\corr{\Hb_k}}{\corr{\Sb}}$ (red) and $\ssim{\corr{\W_k^\top}}{\corr{\Sb^\top}}$ (blue) in plot (e).
    %Evolution of UFM parameters $\Lb_k$, $\corr{\W_k^\top}$ and $\corr{\Hb_k}$ when training close to convergence to the empirical entropy $\Hc$ (plot (d)). At the end of the training, the parameters align with the prediction of Thm.~\ref{thm:reg path} ((a) vs (b)). Additionally, the correlation patterns between the embeddings closely follows the similarities between the support sets ((a) vs (c)). We verify the similarity between the optimal embedding geometry and the support sets by measuring $\ssim{\corr{\Hb_k}}{\corr{\Sb}}$ (red) and $\ssim{\corr{\W_k^\top}}{\corr{\Sb^\top}}$ (blue) in plot (e).
    % Evolution of heatmaps of logits $\Lb$, cosine similarity of word embeddings $\W$ and context embeddings $\Hb$ of UFM during training: 1) at the end of training, heatmaps align with the prediction of Thm.~\ref{thm:reg path}, 2) word/context embeddings have higher correlations when their support set structures are more similar. See text for details. 
    % Heatmaps of $\Lb$, $\W\W^\top$ and $\Hb^\top\Hb$ of UFM during training (Sec.~\ref{sec:ufmexp}): 1) UFM parameters align with the prediction of Thm.~\ref{thm:reg path}, 2) The word and context embeddings have higher correlations when they have more similar support set structures.\tina{replace cosine similarity if time+bit vague}
    }
	\label{fig:UFM_heatmap}
	\vspace{20pt}
% \end{figure*}
% \begin{figure*}[h]
	% \vspace{-35pt}
	\centering
    \hspace{-10pt}
    \begin{subfigure}{0.22\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
            {\includegraphics[scale=0.3]{figures/UFM_loss.pdf}};
			
			\node at (0.1,1.2) [scale=0.8]{\textbf{(a)} Loss convergence};
           \node at (-2.1,0.2) [scale=0.8, rotate=90]{$\text{CE}(\Lb_k)-\Hc$};
             \node at (0.2,-1.2) [scale=0.6]{epoch $(k)$};
            % \node at (0.2,-1.7) [scale=0.8]{\textbf{(a)}};
		\end{tikzpicture}
    \end{subfigure}
    %
    \hspace{10pt}
    \begin{subfigure}{0.22\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
            {\includegraphics[scale=0.3]{figures/UFM_norm.pdf}};
			
			\node at (0.1,1.2) [scale=0.75]{\textbf{(b)} Norm growth};
             \node at (0.2,-1.2) [scale=0.6]{epoch ($k$)};
            % \node at (0.2,-1.7) [scale=0.8]{\textbf{(b)}};
		\end{tikzpicture}
    \end{subfigure}
    % 
    \hspace{0pt}
    \begin{subfigure}{0.22\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
            {\includegraphics[scale=0.3]{figures/UFM_Linconv.pdf}};
			
			\node at (0.1,1.2) [scale=0.75]{\textbf{(c)} $\norm{\Qcs(\Lb_k) - \Lbin}$};
             \node at (0.2,-1.2) [scale=0.6]{epoch ($k$)};
            % \node at (0.2,-1.7) [scale=0.8]{\textbf{(c)}};
		\end{tikzpicture}
    \end{subfigure}
    %
    \hspace{10pt}
    \begin{subfigure}{0.22\textwidth}
		\centering
		\begin{tikzpicture}[remember picture]
			\node at (-0,-0) 
			% {\includegraphics[scale=0.13]{figures/UFM_Lheatmap.png}};
            % {\includegraphics[scale=0.3]{figures/UFM_SSIM.pdf}};
            {\includegraphics[scale=0.3]{figures/UFM_SSIM_MM.pdf}};
			
			\node at (0.1,1.2) [scale=0.75]{\textbf{(d)} Correlation with proxies};
             \node at (0.2,-1.2) [scale=0.6]{epoch ($k$)};
            % \node at (0.2,-1.7) [scale=0.8]{\textbf{(d)}};
		\end{tikzpicture}
    \end{subfigure}
    % 
    \captionsetup{width=\linewidth}
    \vspace{-5pt}
    \caption{Numerical expermients on UFM. \textbf{(a):} CE converges closely to its empirical entropy lower-bound $\Hc$, \textbf{(b):} The norms of the parameters keep growing to derive the loss to its lower-bound, \textbf{(c):} While the parameters converge directionally to $\Lbmm$ (Fig.~\ref{fig:UFM_heatmap}), the projection of $\Lb_k$ on $\Fc$ converges to the finite component $\Lbin$ specified by the soft-labels $\pbh_j$, \textbf{(d):} Correlation between the Gram matrix of $\Hb$ (resp. $\W^\top$) with $\Sb$ (resp. $\Sb^\top$). At the final stage of training the correlation between the parameters and support set proxies is high. See Sec.~\ref{sec:metrics} for the correlation metric. \tina{no convergence plot to Lmm included..., + better to have these figs on the previous page}
    }
	\label{fig:UFM_curves}
	\vspace{0pt}
\end{figure*}


==> Arxiv_NewTempl/sections/figure_syn_losses.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \node[inner sep=0pt] (fig) at (0,0) {
            \begin{subfigure}[b]{0.45\linewidth}
                \includegraphics[width=\linewidth]{exp_results_yize/CElosses_all_4 layer Transformer pos off_tiny_extract_m404_d128.pdf}
                \caption{Loss convergence plot}
                \label{fig:losses}
            \end{subfigure}
            \hfill
            \begin{subfigure}[b]{0.45\linewidth}
                \includegraphics[width=\linewidth]{exp_results_yize/WHnormgrowth_all_tiny_extract_m404_4 layer Transformer pos off_d128.pdf}
                \caption{Norm growth plot}
                \label{fig:norms}
            \end{subfigure}
        };
        % \node[anchor=north west, align=center, opacity=1, text opacity=1, text width=3cm, scale=0.8] at (2.2, 9.5) {$\Lc(\W_k\Hb_k)-\Hc$};
        \node at (-3.8,2.8) [scale=1, align=center, fill=white, fill opacity=1, rounded corners=2pt] {$\Lc(\W_k\Hb_k)-\Hc$}; 
        \node at (3.8,2.8) [scale=1, align=center, fill=white, fill opacity=1, rounded corners=2pt] {Embedding norm}; 
        % Adjust position and styling
        % \draw[red, thick, ->] (label) -- (fig);
    \end{tikzpicture}
    \caption{a) Loss convergence to the lower-bound $\Hc$: Experiments on syntheic setup of Sec.~\ref{sec:synth}.  $\Hc=1.10$ nats for synthetic dataset, $\Hc=1.65$ nats for extracted TinyStories dataset. b) Embeddings grow in norm: Experiments on  the synthetic setup of Sec.~\ref{sec:synth}.
    % \tina{@Yize: fix the legends: UFM for blue and TF for orange. remove titles and axis labels.} 
    \yz{how about this? i merged all loss plots into one and same for norms. FIX LEGENDS}}
	% \label{fig:syn_losses}
\end{figure}

% \begin{figure*}[t]
% 	\vspace{-10pt}
%         \begin{subfigure}{0.5\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (-0.5,-2.1) {\includegraphics[scale=0.43]{yize_paper_figures_tempall/CEloss_UFM_TFM_verysmallset.pdf}};
% 			\node at (0,0.3) [scale=0.8]{$\Lc(\W_k\Hb_k)-\Hc$};
% 			% \node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
%   \caption{Small synthetic dataset}
% 	\end{subfigure}\hspace{10pt}\begin{subfigure}{0.5\textwidth}
% 		\centering
% 		\begin{tikzpicture}
% 			\node at (0,-2.1) {\includegraphics[scale=0.51]{yize_paper_figures_tempall/CEloss_UFM_TFM_tiny404.pdf}};
% 			\node at (0,0.3) [scale=0.8]{$\Lc(\W_k\Hb_k)-\Hc$};
% 			% \node at (0,-2.6) [scale=0.7]{Epoch};
% 		\end{tikzpicture}
%   \caption{Synthetic data from Tiny Stories}
% 	\end{subfigure}

% 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \caption{Loss convergence to the lower-bound $\Hc$: Experiments on syntheic setup of Sec.~\ref{sec:synth}. a) $\Hc=1.10$ nats, (b) $\Hc=1.65$ nats. \tina{@Yize: fix the legends: UFM for blue and TF for orange. remove titles and axis labels.}}
% 	\label{fig:syn_losses}
% %	\vspace{-5pt}
% \end{figure*}

==> Arxiv_NewTempl/sections/geometry_app.tex <==
\subsection{A collapse property: \new{Subspace Collapse}}
\tina{moved to main body}

% The proposition below suggests that embeddings of contexts whose support sets are identical collapse to the same embedding. The proposition supports theoretically the empirical observations in Figs. \ref{fig:intro_TinyStories} and \ref{fig:larger_TinyStories}. 

% \begin{proposition}\label{propo:collapse}
%  Assume \eqref{eq:ufm-svm} is feasible. There exists minimizer $\Hb_\la=[\hb_1,\ldots,\hb_m]$  of \eqref{eq:ufm} such that the following holds. 
%     For all contexts $j,j'\in[m]$ with same support set $\Sc_j=\Sc_{j'}$, the context embeddings are same in direction in the limit of vanishing regularization, i.e.,
%     $\lim_{\laz}\left\|\overline{\hb_j}-\overline{\hb_{j'}}\right\|=0$. 
% \end{proposition}

% % \ct{not complete. need to think more}  
% \begin{proof}
%     \input{Arxiv/sections/collapse_proof} 
% \end{proof}

\subsection{Proof of Proposition \ref{prop:all symmetric geometry}}
\tina{commented and moved above}

%-----------------------------
% Before proving the proposition, we state here a more refined version that explicitly computes norms/angles of the geometry.

% \begin{proposition}%\label{prop:sym geo app}
%        Assume the setting of Proposition \ref{prop:all symmetric geometry}. The geometry of context and word embeddings  is described by the following relations:
%     \begin{subequations}
%     \begin{align}
%         \forall v\neq v'\in[V]\,&:\,\cosa{\w_v}{\w_{v'}} = \frac{-1}{V-1} \quad\text{and}\quad \|\w_v\|=\|\w_{v'}\|
%         \\
%         \forall j\neq j'\in[m]\,&:\,\cosa{\hb_j}{\hb_{j'}}=\frac{|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}}{k-\frac{k^2}{V}}\quad\text{and}\quad \|\hb_j\|=\|\hb_{j'}\|
%         \\
%         \forall j\in[m], v\in[V]\,&:\
%         \cosa{\w_v}{\hb_j} = \begin{cases}
%     \sqrt{\frac{V-1}{k(V-k)}} & v\in\Sc_j\\
%      \frac{-1}{\sqrt{k(V-k)(V-1)}} & v\notin\Sc_j
%     \end{cases}\,
%     \\
%     \forall j\in[m], v\in[V]\,&:\ \frac{\|\w_v\|^2}{\|\hb_j\|^2} = \frac{(V-1)\,\binom{V-2}{k-1}}{k(V-k)}\,.
%     \end{align}
%     \end{subequations}
% \end{proposition}


% \begin{figure}[t]
%     \centering 
%     \includegraphics[width=0.7\linewidth]{figures/symmetric_geo_w_h.eps}  
% \captionsetup{width=\textwidth}
%     \caption{Geometry properties illustration for Proposition \ref{prop:all symmetric geometry}. Shown two values of $V$ for varying values of $k\in[V-1]$. (Left) angles between context and word embeddings. (Right) normalized norm ratio of word to context embeddings.}
%     %\label{fig:symmetric_geo}
% \end{figure}


% At the heart of proving both Propositions \ref{prop:all symmetric geometry} and \ref{prop:sym geo app} is the following result, which determines the SVD factors $\Ub$, $\Sigmab$, and $\Vb$ of $\Lbtina=(\Id_V-\frac{1}{V}\ones\ones^\top)\Sb$. This shows immediately that word embeddings form an ETF. It also forms the basis for computing the geometry of context embeddings. We show this after proving the lemma.
% \begin{lemma}
% Fix any $k\in[V]$ and suppose $\smat$ contains all $V\choose k$ support sets of size $k$, i.e. $m={V\choose k}$. Let $\Pbb\in\R^{V\times (V-1)}$ be orthonormal basis of the subspace orthogonal to $\ones_V$. Then, the $\Ub,\Sigmab$ factors of the SVD of $\Lbtina$ are:
% $\Ub=\Pbb$ and $\Sigmab=\sqrt{\binom{V-2}{k-1}}\,\Id_{V-1}$. Thus,
% \[
% \Ub\Sigmab\Ub^\top \propto \Big(\Id_V-\frac{1}{V}\ones\ones^\top\Big)\,.
% \]
% Moreover, the matrix $\Vb\in\R^{m\times(V-1)}$ of right-singular vectors is such that its rows $\vb_j, j\in[m]$ can be expressed as follows with respect to the rows $\ub_z, z\in[V]$ of $\Ub$:
% \[
% \vb_j = \frac{1}{\sqrt{\binom{V-2}{k-1}}}\sum_{z\in\Sc_j}\ub_z\,~~j\in[m].
% \]
% \end{lemma}
% \begin{proof}
%     We will compute explicitly $\Lbtina{\Lbtina}^\top$. Start with computing $\smat\smat^\top$.  For diagonal elements,  the dot product is between a row of $\smat$ and itself, counts the number of $1$s in that row. Since each element is included in $\binom{V-1}{k-1}$ support sets (choosing the remaining $k-1$ elements from the other $V-1$ elements), each diagonal entry of $\smat\smat^\top$ is $\binom{V-1}{k-1}$. For off-diagonal elements, the dot product counts the number of support sets in which both elements of the corresponding rows appear. This requires choosing the remaining $k-2$ elements from  $V-2$ elements, giving $\binom{V-2}{k-2}$ for each off-diagonal entry of $\smat\smat'$. Overall, after algebraic simplification, we find that
%     \[
%     \smat\smat^\top = \binom{V-2}{k-1}\left(\Id_V+\frac{k-1}{V-k}\ones\ones^\top\right)\,.
%     \]
%     We may now use the closed form of $\Lbtina$ and few more algebra simplifications to find that
%     \[
%     \Lbtina{\Lbtina}^\top=\binom{V-2}{k-1}\left(\Id_V-\frac{1}{V}\ones\ones^\top\right)\,.
%     \]
%     Let $\Pbb\in\R^{V\times (V-1)}$ denote an orthonormal basis of the subspace orthogonal to $\ones_V$. Since $ \Lbtina{\Lbtina}^\top=\binom{V-2}{k-1}\Pbb\Pbb^\top$ and $\Lbtina{\Lbtina}^\top=\Ub\Sigmab^2\Ub^\top$, we have shown that $\Ub=\Pbb$ and $\Sigmab=\sqrt{\binom{V-2}{k-1}}\,\Id_V$.
% \end{proof}

% Using $\ones^\top\smat=k$, we can compute
% \[
% \Lbtina{\Lbtina}^\top=\smat^\top\smat-\frac{1}{V}(\smat^\top\ones_V)(\smat^\top\ones_V)^\top = \smat^\top\smat-\frac{k^2}{V}\ones_m\ones_m^\top\,.
% \]
% From this and the fact that $\diag{\smat^\top\smat}=k\Id_m$, and recalling that $\Lbtina{\Lbtina}^\top=\Vb\Sigmab^2\Vb^\top$,  we find that all context embeddings are equinorm with squared norm (i.e. diagonal entries of $\Vb\Sigmab\Vb^\top$) equal to 
% \[
% \|\hb_j\|^2= \frac{k-\frac{k^2}{V}}{\sqrt{\binom{V-2}{k-1}}},\,\,\forall j\in[m].
% \]
% Recall also that the diagonal entries of $\Ub\Sigmab\Ub^\top$ are
% \[
% \|\w_v\|^2= \left(1-\frac{1}{V}\right)\sqrt{\binom{V-2}{k-1}},\,\,\forall v\in[V].
% \]

% From the off-diagonal entries of $\Lbtina{\Lbtina}^\top$, we can infer the angles between different context embeddings. Let $j\neq j'\in[m]$, then the $(j,j')$ of $\Lbtina{\Lbtina}^\top$ is $|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}$. Thus, the  $(j,j')$ off-diagonal entries of $\Vb\Sigmab\Vb^\top$ are \[ \hb_j^\top\hb_{j'}=\frac{|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}}{\sqrt{\binom{V-2}{k-1}}}\implies \cosa{\hb_j}{\hb_{j'}}=\frac{|\Sc_j\cap\Sc_{j'}|-\frac{k^2}{V}}{k-\frac{k^2}{V}}\,\,\,j\neq j'\in[m]\,.
% \]


% Recalling that $\W\Hb^\top=\Lbmm$, we may now compute the angle between word and context embeddings as follows:
% \begin{align}
%     \cosa{\w_v}{\hb_j} = \begin{cases}
%     \sqrt{\frac{V-1}{k(V-k)}} & v\in\Sc_j\\
%      \frac{-1}{\sqrt{k(V-k)(V-1)}} & v\notin\Sc_j
%     \end{cases}\,.
% \end{align}
% This completes the proof of Proposition \ref{prop:sym geo app} and the proof of statements (ii) and (iii) of Proposition \ref{prop:all symmetric geometry}.

% It remains to prove statement (i) of Proposition \ref{prop:all symmetric geometry}, i.e. proving that $\Lbtina=(\Id_V-\frac{1}{V}\ones\ones^\top)\Sb$ is the unique minimizer of \eqref{eq:ufm-svm}.

% To prove this, we appeal to Proposition \ref{propo:svm sufficient condition}. First, it is straightforward checking that $\Lbmm$ satisfies the SVM constraints (in fact, with equality). Thus, from Proposition \ref{propo:svm sufficient condition}, it suffices that the matrix $\A:=\Ub\Vb^\top$ satisfies $\A[v,j]<0$ for all $v\notin\Sc_j$ and all $j\in[m]$. But, in our case $\Ab=\Ub\Vb^\top=\binom{V-2}{k-1}^{-\frac{1}{2}}\Lbtina$ because $\Sigmab=\Id_{V-1}$. Thus, the desired condition holds for $\A$ since $\Lbtina[v,j]=-k/V<0$ for all $j\notin\Sc_j$ and $j\in[m]$.
%-----------------------------

==> Arxiv_NewTempl/sections/intro_old.tex <==
\section{Introduction}

\subsection{Motivation}
Next-token prediction (NTP) has emerged as a pivotal paradigm in language modeling tasks, revolutionizing various applications such as machine translation, text-summarization, and language generation \cite{radford2018improving}. In NTP,  models are trained to predict the most probable token given a sequence of preceding tokens, commonly referred to as the \emph{context}. Specifically, the objective is to learn a mapping from the input context to the probability distribution over the (finite) vocabulary of possible tokens, enabling the model to generate a token that is contextually appropriate \cite{bengio2000neural,bengio2000taking}. 
%Commonly employed in  transformers and other deep learning architectures, the \NTP training paradigm is believed to capture intricate semantic and syntactic dependencies within language, making it a fundamental building block for understanding and generating coherent textual sequences \cite{}. 

Over the past couple of years or so, the paradigm has witnessed remarkable progress through its utilization on large-scale transformers trained on vast corpora of data \cite{radford2018improving,radford2019language,chatgpt}. This has resulted in unprecedented advances in the field, and the swift integration of these advanced language models into society  \cite{gpt4,claude,gemini2023}.
Concurrently, researchers have raised critical concerns about robustness, interpretability, and bias issues arising from our limited understanding of the fundamental operational principles of these models \cite{bommasani2021opportunities, belkin2024necessity}. Although these issues have garnered significant research attention, a comprehensive theory elucidating the fundamentals of large language models, including key components such as the \NTP paradigm and the transformer architecture, with respect to their optimization and generalization principles, remains elusive.



 \subsection{Approach}

 This paper initiates an investigation of the optimization principles of the \NTP training paradigm. 
 
 \vspace{3pt}\noindent\textbf{\NTP training.} Formalizing the \NTP paradigm, consider autoregressive model $q_{\thetab}$ parameterized by  $\thetab$  trained  to predict the next-token on sequences of length $T$ using the cross-entropy (CE) loss:
\begin{align}\label{eq:intro CE}
\min_{\thetab} ~\hat\E_{\z\sim_{\Tc_n}}\Big[ \sum_{t\in[T]}-\log\left( q_{\thetab}(z_t\,|\,z_1,\ldots, z_{t-1}) \right) \Big].
\end{align}
Here, sequences $\z=(z_1,\ldots,z_T)$ consist of tokens $z_t$ from a finite vocabulary $\Vc=\{1,\ldots,V\}$ and $\hat\E$ is expectation over training set $\Tc_n$ of $n$ such sequences sampled iid from some underlying true distribution over sequences. Typically, the model $q_{\thetab}$ outputs probability of the next token computed via softmax applied on  output logits, which are  computed by projecting $d$-dimensional embeddings $h_{\thetab'}$ to the $V$-dimensional space with a trainable linear decoder $\W\in\R^{V\times d}$. Mathematically, \footnote{Throughout, $\eb_v$ is the $v$-th standard basis vector in $\R^V$, and $\sfti{z}{\ub}:=\eb_z^\top\sft{\ub}$ is the $z$-th index of the softmax output.}
\begin{align*}
&q_{\thetab}(z_t\,|\,z_1,\ldots, z_{t-1}) = \sfti{z_t}{\W h_{\thetab'}(z_1,\ldots,z_{t-1})}\,
= 
\frac{1}{1+\sum_{\stackrel{z'\in\Vc}{z'\neq z_t}} \exp\left((\eb_{z'}-\eb_{z_t})^\top\W h_{\thetab'}(z_1,\ldots,z_{t-1})\right)}\,.
\end{align*}
The CE loss is then minimized over $\thetab=(\W,\thetab')$ using gradient-based methods, e.g. SGD, Adam.

\vspace{3pt}\noindent\textbf{Implicit-bias question.} We pose the following question: 

\begin{center}
\emph{Given training set $\Tc_n$, what are the structural properties of the weights $\thetab$ found by minimizing the \NTP cross-entropy objective with gradient-based methods?}
\end{center}
Drawing inspiration from a substantial body of research in one-hot supervised classification \footnote{
In \NTP, the ground-truth next token is inherently embedded within the underlying text (i.e., the labels are implicit), thus strictly speaking, it falls under the self-supervised learning paradigm \cite{radford2018improving}. However, the utilization of the cross-entropy (CE) training objective in \eqref{eq:CE} bears striking resemblance to supervised training. In this paper, we leverage this resemblance and essentially regard the \NTP paradigm as an instance of supervised learning. At the same time, we make it clear  that it is distinct from classical one-hot encoding supervision.} (e.g. \cite{zhang2017understanding,belkin2018does,soudry2018implicit,ji2018risk}), we specifically target this question in the \emph{overparameterized setting}, where the autoregressive CE training objective \eqref{eq:intro CE} may have an infinite number of solutions, representing an infinite number of models $\thetab$ that minimize the training loss. The central challenge is to discern the particular solution the optimizer is inherently biased towards. Since this 'bias' is not explicitly introduced through regularization but is instead ingrained in the training objective and algorithmic structure, it is termed `implicit bias' \cite{neyshabur2014search}. 

The exploration of implicit bias has a long history in the traditional supervised classification setting of one-hot predictions (see \emph{Related Work in Sec. \ref{sec:rel work}}). In this conventional scenario, the training set comprises feature-label pairs $(\x, y)$, where $\x\in\R^p$ is a continuous feature, and $y$ represents its unique label. The optimization process minimizes the following training objective (over $\W,\thetab'$):
\begin{align}\label{eq:intro traditional}
\hat\E_{(\x,y)}\left[-\log\left(\sfti{y}{\W h'_{\thetab}(\x)}\right)\right].
\end{align}

%\vspace{3pt}\noindent\textbf{Why is \NTP setting different?}
% \vspace{-0.05in}
\noindent\textbf{\NTP vs one-hot prediction.} Initially, it may seem that the \NTP training setting is indistinguishable from traditional one-hot prediction: both involve minimizing the same cross-entropy (CE) loss over a model that parameterizes probabilities using the softmax of logits. The resemblance becomes more apparent when focusing on a simplified \NTP setting, specifically when the objective involves training solely on the last token. In this scenario, the summation in \eqref{eq:intro CE} considers only the $T$-term:
\begin{align}\label{eq:intro CE2}
\hat\E_{\z}\left[-\log\left(\sfti{z_t}{\W h_{\thetab}(z_1,\ldots,z_{T-1})}\right)\right].
\end{align}
Here, the context serves as the feature, and the next token serves as the label. Despite the apparent similarity in training objectives between \NTP and traditional one-hot classification settings, a crucial distinction lies in the nature of the training data that sets these two scenarios apart.

Specifically, in the traditional setting, each feature (e.g., an image) is assigned a single  label (e.g., an image category). In contrast, in the \NTP setting,  contexts $z_1, \ldots, z_{t-1}$ of finite length sampled from finite vocabularies are expected to be repeated in the (vast) training set, potentially multiple times, each time followed by \emph{different} tokens $z_t$. Consequently, the \NTP objective involves training over $m \leq n$ \emph{distinct} (non-repetitive) contexts, each followed by a multitude of possible next tokens, appearing at varying frequencies. For instance, in a language training corpus, the context "\texttt{She is excellent at her role as a}" may be followed by next tokens such as "\texttt{doctor}," "\texttt{lawyer}," or "\texttt{mother}," each with different frequencies. Importantly, certain tokens in the vocabulary may \emph{not} appear after a given context; e.g., in the aforementioned example, tokens like "\texttt{run}," "\texttt{and}," etc., will not follow.

\vspace{3pt}\noindent\textbf{Model.} We delve into the study of \NTP training over a finite vocabulary employing the following model. Given a large training set of $n$ total contexts, we identify $m\leq n$ \emph{distinct} contexts. Each distinct context $j\in[m]$ is linked to a $V$-dimensional empirical probability vector $\pbh_j$, which encodes the frequency with which each vocabulary token follows the context throughout its occurrences in the training set. Crucially, the probability vectors $\pbh_j$ are \emph{sparse}, indicating that the support set $\Sc_j$ of $\pbh_j$ satisfies $|\Sc_j|\ll |\Vc|=V$. In the extreme case where $|\Sc_j|=1$ for all $j\in[m]$, the probability vector $\pbh_j$ becomes an indicator or one-hot-encoding vector, leading to a scenario reminiscent of the traditional classification setting described earlier. However, we advocate that such an extreme case is essentially improbable in practical language settings. %As a result, the \NTP training setting (objectives \eqref{eq:intro CE} and even \eqref{eq:intro CE2}) differs from the traditional one-hot  classification setting (objective \eqref{eq:intro traditional}). 

\paragraph{Soft-label classification.}~In fact, framing \NTP in this manner reveals a connection between the setting and supervised classification with \emph{soft labels}. Unlike most typical benchmark datasets containing hard labels, a line of research advocates for training models on datasets where each example is associated with a vector of soft labels (rather than a one-hot vector), such as by averaging multiple annotators' hard labels \cite{peterson2019human}. Soft-label classification also arises in knowledge distillation \cite{knowledge-distilation} and label smoothing \cite{label_smoothing}. Here, we assert that soft labels naturally emerge in the \NTP setting (specifically, last-token prediction), with a notable characteristic being the sparsity of the vector $\ph_j$ of soft labels. Given this connection, our analysis can also be interpreted (more broadly) as investigating the implicit bias of soft-label classification.

\subsection{Related work}
\vspace{3pt}\noindent\textbf{Classification with Soft Labels.}
Unlike one-hot classification, soft-label classification associates each example with a probability vector, where each entry represents the likelihood of a corresponding label characterizing the example. Although arguably less prevalent than one-hot (or hard-label) classification, soft-label classification arises in various contexts, including modeling human confusion during crowd-sourcing \cite{peterson2019human,soft1,soft2}, knowledge distillation \cite{knowledge-distilation}, and label smoothing \cite{label_smoothing}. Our model of last-token prediction also falls within this setting. Specifically, our approach is most closely related to soft-labels generated by averaging annotators' hard labels \cite{peterson2019human}, rather than following the winner-takes-all rule. \cite{peterson2019human} and follow-up workhave provided empirical evidence that using probabilistic soft labels generated from crowd annotations for training leads to improved performance in terms of model generalization, calibration, and robustness to out-of-distribution data. To the best of our knowledge, no prior work has investigated the implicit bias of gradient descent in this or other soft-label classification settings; thus, our results are of direct relevance to these contexts as well.


% Although arguably less popular than one-hot (or hard-label) classification, soft-label classification arises in various contexts, including in modeling human confusion during crowdsourcing \cite{}, in knowledge distillation \cite{}, and in the mixup technique \cite{}.

% \vspace{-0.12in}
% \subsection{Contributions}
% % \vspace{-0.12in}
% Recognizing the distinction between \NTP and one-hot classification, we initiate a study of implicit bias questions within the \NTP setting.
% To facilitate this, we introduce simplifying assumptions, detailed below, with plans to relax them in future research. %Our hope is that these results inspire further investigations aimed at lifting some of these assumptions.

% \vspace{3pt}\noindent\textbf{Setting: Last-token, linear model, overparameterization and GD.} We focus on objective \eqref{eq:intro CE2} that trains a model over predicting the last token and we train the objective using gradient descent (GD). 
% %We leave extensions to the full autoregressive objective over all tokens in  \eqref{eq:intro CE} and other optimizers to future work. 
% %
% Throughout our analysis, we adopt a `top-down' approach, assuming that only the decoding matrix $\W\in\R^{V\times d}$ is trained, while embeddings remain fixed. This separation allows us to disentangle the intricacies of the \NTP training objective and the underlying architecture responsible for producing embeddings, enabling a focused examination of the former.  Now, the resulting model for the logits is thus linear and the training objective \eqref{eq:intro CE2} is convex. Our primary goal is to determine the structure of the decoder weights $\W_k$ at the end of training. This question is posed within an overparameterized setting, where the dimensionality $d$ is large, resulting in multiple solutions to minimizing \eqref{eq:intro CE2}. We seek to determine the implicit bias of GD towards one of these solutions.%Standard optimization analysis informs us that the training loss of GD approaches the infimum of the objective at rate $\Oc(1/k)$ after $k$ iterations. Instead here, we aim to understand what is the structure of the decoder weights $\W_k$ at the end of training. We pose this question in an overparameterized setting (for linear models here this means large $d$), where there is multiple solutions to minimzing \eqref{eq:intro CE2} and ask to determine the bias of GD towards one of them. 


% \vspace{3pt}\noindent\textbf{\NTP separability.} Concretely, we show that when the embedding dimension $d$ exceeds the number $m$ of distinct contexts, then almost all datasets satisfy two key conditions: \NTPH-compatibility and \NTP-separability. We show that when these conditions are met, the CE  loss can approach its lower bound, the empirical conditional entropy, by traversing certain possible directions towards infinity. This raises the implicit-bias question:  which direction is favored by different iterative algorithms?

% \vspace{3pt}\noindent\textbf{\NTP-SVM.} To gain insight on the implicit bias in \NTP settings, we  investigate  the direction\footnote{Unless otherwise specified $\|\cdot\|$ denotes Euclidean norm. We also let $\overline\W:=\W/\|\W\|$.} ${\What_\la}/{\|\What_\la\|}$ of the ridge-regularized CE minimizer $\What_\la$  with  weight $\lambda$. In the limit of vanishing regularization $\la\rightarrow0$, we show that the direction approaches the direction of $\Wmm$, which is the minimum Euclidean-norm classifier matrix that satisfies the \NTP-separability. $\Wmm$ generalizes the traditional multiclass max-margin classifier  by incorporating additional subspace constraints $\Wmm\in\Ts^\perp$ arising from the potential presence of multiple next-tokens ($|\Sc_j|>1$) per context.

% \vspace{3pt}\noindent\textbf{Implicit bias of GD.} Finally, we show that under \NTPH-compatibility and \NTP separability, in the limit of iterations $k\rightarrow\infty$, the GD iterates grow undoubtedly in norm and and converge to a finite $\Wstar$ within a data subspace $\Ts$, while simultaneously aligning with $\overline\Wmm$ in the complementary subspace $\Ts^\perp$.
% %in direction to the direction of $\Wmm$. 
% We verify our findings via experiments on synthetic data and discuss future work.  







==> Arxiv_NewTempl/sections/logit_factor_notes_do_not_upload.tex <==
\subsection{Logit matrix factorization}
\ct{this section will be removed. please ignore}
% \begin{lemma}
    Suppose $d>2V$. Let $\Lbin=\Ub_1\Sigmab_1\Vb_1^\top$ be the SVD of $\Lbin$. Denote $r:=\rank{\Lbmm}$ and $r_1:=\rank{\Lbin}$. Let $\Qb\in\R^{d\times r}$ and $\Qb_\perp\in\R^{d\times r_1}$ be partial orthonormal matrices with mutually orthogonal columns, i.e. $\Qb^\top\Qb=\Id_r$, $\Qb_\perp^\top\Qb_\perp=\Id_{r_1}$, and $\Qb^\top\Qb_\perp=0, \Qb_\perp^\top\Qb=0$. (It is always possible to select such $\Qb_1,\Qb_2$ since $d\geq2V\geq r_1+r$.) With these define,
    \begin{align}
    \W&:=\Ub_1\sqrt{\Sigmab_1}\Qb_\perp^\top + \sqrt{R}\cdot\Ub\sqrt{\Sigmab}\Qb^\top
    \\
    \Hb&:=\Qb_\perp\sqrt{\Sigmab_1}\Vb_1^\top + \sqrt{R}\cdot\Qb\sqrt{\Sigmab}\Vb^\top
    \end{align}
% \end{lemma}

Note then that
\[
\W\Hb = \Lbin + R\cdot\Lbmm\,.
\]
Additionally,
\begin{align}
    \GW&:=\Ub_1\Sigmab_1\Ub_1^\top + R\cdot\Ub\Sigmab\Ub^\top
    \\
    \GH&:=\Vb_1\Sigmab_1\Vb_1^\top + R\cdot\Vb\Sigmab\Vb^\top
    \end{align}

Let now $\Pbb_{\Ub}^\perp=\Ub_\perp\Ub_\perp^\top$  denote projection matrix to the orthogonal complement of column space of $\Ub$. Similarly, define projections for $\Vb.$

As $R\rightarrow\infty$, we have the following properties:
\[
\overline\GW\propto \Ub\Sigmab\Ub^\top 
\]
and
\begin{align}
\GW\Pbb_{\Ub}^\perp &= \Ub_1\Sigmab_1\Ub_1^\top\Pbb_{\Ub}^\perp
\\
\Pbb_{\Ub}^\perp\GW &= \Pbb_{\Ub}^\perp\Ub_1\Sigmab_1\Ub_1^\top
\\
\Pbb_{\Ub}^\perp\GW\Pbb_{\Ub}^\perp &= \Pbb_{\Ub}^\perp\Ub_1\Sigmab_1\Ub_1^\top\Pbb_{\Ub}^\perp
\end{align}
Similarly,
\[
\overline\GH\propto \Vb\Sigmab\Vb^\top 
\]
and
\begin{align}
\GW\Pbb_{\Vb}^\perp &= \Vb_1\Sigmab_1\Vb_1^\top\Pbb_{\Vb}^\perp
\\
\Pbb_{\Vb}^\perp\GW &= \Pbb_{\Vb}^\perp\Vb_1\Sigmab_1\Vb_1^\top
\\
\Pbb_{\Vb}^\perp\GW\Pbb_{\Vb}^\perp &= \Pbb_{\Vb}^\perp\Vb_1\Sigmab_1\Vb_1^\top\Pbb_{\Vb}^\perp
\end{align}


\subsubsection{Again}
Let $\Lbmm=\Ub\Sigmab\Vb$. Let $\Pbb_{\Ub}^\perp=\Ub_\perp\Ub_\perp^\top$  denote projection matrix to the orthogonal complement of column space of $\Ub$. Also $\Pbb_U=\Ub\Ub^\top$ the projection to $\Ub$. Thus, $\Pbb_U^\perp=\Id_V-\Pbb_U$ Similarly, define projections for $\Vb.$
Finally, define the orthogonal decomposition 
\[
\R^{V\times m}=\Tc\bigoplus\Tc^\perp
\]
 where $\Tc$ is the set of matrices spanned by $\ub\vb^\top$. The projections to the two spaces are given as
 \[
 \Pbb_{\Tc}(\A)=\Pbb_U\A\Pbb_V\,.
 \]
 and
 \[
 \Pbb_{\Ts^\perp}(\A):=\Pbb_{\perp}(\A)=\Pbb_U^\perp\A+\A\Pbb_V^\perp-\Pbb_U^\perp\A\Pbb_V^\perp\,
 \]

 \noindent\textbf{Claim:} In the limit of vanishing regularization, the logit matrix satisfies
 \[
  \|\Pbb_\Ts(\Lb)\|\rightarrow\infty \qquad\text{and}\qquad\Pbb_\Ts(\Lb)\propto\Lbmm
 \]
 \[
  \Pbb_\perp(\Lb)\rightarrow \Lbstar= \ct{???}.
 \]
 
 Then, defining SVD $\Lbstar=\Ub_1\Sigmab_1\Vb_1^\top$ the $\W,\Hb$ decomposition is as follows:
 \begin{align}
    \GW&:=\Ub_1\Sigmab_1\Ub_1^\top + R\cdot\Ub\Sigmab\Ub^\top
    \\
    \GH&:=\Vb_1\Sigmab_1\Vb_1^\top + R\cdot\Vb\Sigmab\Vb^\top
    \end{align}
 or
 \begin{align}
    \GW^*:=(\Id_V-\Ub\Ub^\top)\GW(\Id_m-\Ub\Ub^\top)&:=\Ub_1\Sigmab_1\Ub_1^\top \quad\text{and}\quad (\GW-\GW^*) \propto \Ub\Sigmab\Ub^\top
    \\
    \GH^*:=(\Id_V-\Vb\Vb^\top)\GH(\Id_m-\Vb\Vb^\top)&:=\Vb_1\Sigmab_1\Vb_1^\top \quad\text{and}\quad (\GH-\GH^*) \propto \Vb\Sigmab\Vb^\top
    \end{align}


\subsubsection{Lessons 03/27}

It seems that what we predict is $\Lb_\la$ on the subspace of $\Lbmm$, i.e. on the subspace $\Tc$. Indeed, the error of $\Pbb_\Tc(\Lb_\la-\Lbin)$ to $\Lbmm$ is small, but the component $\Pbb_\perp(\Lb_\la)$ is non-zero. One would hope that this component is equal to $\Pb_\perp(\Lbin)$ but this is not the case. So there is a component of $\Lb_\la$ that we are missing. I suspect this component is coming because to the finite part $\Lbin$, we can in principle add anything that is arbitrary (but finite) on the off-support, i.e. the finite part is $\Lbin$ plus something that is on;y active on the off-support. Then, the part that we are missing from the description of $\Lb_\la$ is $\Pb_\perp(\Lbin+\text{that something}).$
 

==> Arxiv_NewTempl/sections/proof_regpath.tex <==
\subsection{Regularization Path}
\label{app:proof reg-path}

We provide a detailed proof of Theorem \ref{thm:reg-path} filling in missing details from the proof sketch in the main paper.

\subsubsection{Proof of Theorem \ref{thm:reg-path}}
First, we show that $\What_B$ is on the boundary, i.e. $\|\What_B\|=B$. Suppose not, then $\inp{\nabla\CE(\What_B)}{\Ub}=0$ for all $\Ub\in\R^{V\times d}$. 
Using the CE expression in \eqref{eq:CE2} and a few algebraic manipulations, yields
\begin{align}
    \hspace{-0.1in}\inp{-\nabla\CE(\What_B)}{\Ub}  \label{eq:grad}
=\sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\Big(\sum_{\stackrel{z'\in\Sc_j}{z'\neq z}}s_{j,z'}\,(\eb_z-\eb_{z'})^\top\Ub\hd_j+\sum_{v\notin\Sc_j}s_{j,v}\,(\eb_z-\eb_v)^\top\Ub\hd_j\Big),
\end{align}
where we denote the output probabilities at $\What_B$ as $s_{j,v}:=\sfti{v}{\What_B\hd_j}, v\in\Vc, j\in[m].$
 Choose $\Ub=\Wmm$ in \eqref{eq:grad}. Then, the first term in the parenthesis in \eqref{eq:grad} is zero by \eqref{eq:Wmm condition equal}, while the second term is strictly positive by \eqref{eq:Wmm condition larger} and strict positivity of softmax entries, leading to contradiction. % Thus, $\inp{-\nabla\CE(\What_B)}{\Wmm}>0$, which is a contradiction. Hence $\What_B$ is on the boundary.

Now, consider point $\Wstar_B=\Wstar+R(B)\cdot\Wmm$, where, $\Wstar\in\Tc$ satisfies \eqref{eq:Wf condition}, and $R=R(B)$ is chosen such that $\|\Wstar_B\|=B$. Concretely, for $B>\|\Wstar\|$, set 
\[R=\frac{1}{\|\Wmm\|}\sqrt{B^2-\|\Wstar\|^2}.\] Note also  that $R/B\rightarrow1/\|\Wmm\|$ as  $B\rightarrow\infty$. We will show that $\Wstar_B$ attains a small CE loss as $B$ (hence, $R$) grows. To do this, denote for convenience the logits for all $v\in\Vc, j\in[m]:$ 
\[
\ellstar_{j,v}:=\eb_v^\top\Wstar\hd_j\quad\text{and}\quad\ellmm_{j,v}:=\eb_v^\top\Wmm\hd_j\,,
\]
and note that $\eb_v^\top\Wstar_B\hd_j=\ellstar_{j,v}+R\,\ellmm_{j,v}.$ 
By using \eqref{eq:Wf condition} and \eqref{eq:Wmm condition equal}:
\[
\sum_{z'\in\Sc_j}e^{-(\ellstar_{j,z}+R\ellmm_{j,z}-\ellstar_{j,z'}-R\ellmm_{j,z'})} = \frac{1}{\ph_j}.
\]
Moreover, using \eqref{eq:Wmm condition larger}
\begin{align*}
    \sum_{v\notin\Sc_j}e^{-(\ellstar_{j,z}+R\ellmm_{j,z}-\ellstar_{j,v}-R\ellmm_{j,v})} \leq e^{-R} \sum_{v\notin\Sc_j}e^{-(\ellstar_{j,z}-\ellstar_{j,v})} \leq C\,e^{-R},
\end{align*}
where we define constant (independent of $R$)  $C:=Ve^{\|\Wstar\|M}$, for $M:=\sqrt{2}\cdot\max_{j/\in[m]}\|\hd_j\|$.

Combining the above displays and using in Eq. \eqref{eq:CE2}, yields
\begin{align}
    \CE(\Wstar_B) &\leq \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log\Big(\frac{1}{\ph_{j,z}}+C\,e^{-R}\Big)\,\nn
    \leq\sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\Big(\log\big(\frac{1}{\ph_{j,z}}\big)+\ph_{j,z}C\,e^{-R}\Big)\nn
    \\
    &\leq\Hc+C\,e^{-R}\,,\label{eq:reg path up}
\end{align}
where, the second line uses $\log(1+x)\leq x, x>0$, and the third line uses $\pih_j,\ph_{j,z}$ are probabilities. 

Next, towards arriving at a contradiction, 
we will show that if $\What_B$ is not in the direction of $\Wmm$, then it incurs a loss that is larger than $\CE(\Wstar_B)$. Concretely, assuming the statement of the theorem is not true, we
we will upper bound 
\begin{align}\label{eq:towards Wb}
\CE(\What_B)-\Hc = \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log\Big(\frac{\ph_{j,z}}{\sfti{z}{\What_B\hd_j}}\Big).
\end{align}
By our assumption, there exists $\eps>0$, such that there exists arbitrarily large $B$ satisfying:
\begin{align}\label{eq:contra eps}
\Big\|\frac{\|\Wmm\|}{B}\What_B-\Wmm\Big\|>\eps.
\end{align}
Define
\[
\What=\frac{1}{R'(B)}\big(\What_B-\Wstar\big),
\]
where, $R'=R'(B)>0$ is chosen so that $\|\What\|=\|\Wmm\|$. Concretely, for large enough $B\geq 2\|\Wmm\|$, set 
\[
R'=\sqrt{\frac{B^2}{\|\Wmm\|^2}-2B\inp{\overline{\W_B}}{\overline\Wmm}+1}\,.
\]
Note that it holds  $\lim_{B\rightarrow\infty}R'/B=1/\|\Wmm\|.$ Thus, we can always choose $B$ large enough so that Eq. \eqref{eq:contra eps} guarantees
$
\|\What-\Wmm\|\geq \eps',
$
for some $\eps'>0$.
Since $\Wmm$ is the unique minimizer of \eqref{eq:SVM} and $\|\What\|=\|\Wmm\|$, it follows that there exists $\delta\in(0,1)$ and $j\in[m]$ such that at least one of the following is true

(i) $\exists z$ and $z'\neq z\in\Sc_{j}$ such that 
\begin{align}
    \label{eq:contra 1}
    |(\eb_z-\eb_{z'})^\top\What\hd_j|\geq \delta\,,
\end{align}

(ii) $\exists z\in\Sc_{j}, v\notin\Sc_{j}$ such that 
\begin{align}\label{eq:contra 2}
(\eb_z-\eb_{v})^\top\What\hd_j\leq 1-\delta.    
\end{align}


\noindent\emph{\underline{Case (i):}}~ Without loss of generality $(\eb_z-\eb_{z'})^\top\What\hd_j\leq -\delta$ (otherwise, flip $z,z'$). Thus, ignoring all but one term in \eqref{eq:towards Wb} gives
\begin{align}\label{eq:towards Wb 2}
\CE(\What_B)-\Hc &\geq \pih_j\ph_{j,z}\log\Big(\frac{\ph_{j,z}}{\sfti{z}{\What_B\hd_j}}\Big)\geq\pih_j\ph_{j,z}\log\Big({\ph_{j,z}}e^{(\ell_{j,z'}-\ell_{j,z})}\Big),
\end{align}
where we use $\ell_{j,v}=\eb_v^\top\What_B\hd_j, v\in\Vc$ to denote logits of $\What_B$. Using \eqref{eq:Wf condition} and \eqref{eq:contra 1}, yields
\begin{align}%\label{eq:contra logits}
\ell_{j,z'}-\ell_{j,z} &= (\eb_{z'}-\eb_z)^\top\big({R'}\,\What+\Wstar\big)\,\hd_j    
\geq {R'}\delta+\log\left(\frac{\ph_{j,z'}}{\ph_{j,z}}\right) \,.\nn
\end{align}
Put in \eqref{eq:towards Wb} and using $ \ph_{j,z}\geq\pih_j\ph_{j,z} \geq 1/n$ shows 
\begin{align}\nn
    \CE(\What_B) &\geq \Hc + \frac{1}{n}\log\Big(\frac{e^{R'\delta}}{n}\,\Big)
\end{align}
Compare this with \eqref{eq:reg path up}. For large enough $B$, it is clear that $\pih_j\ph_{j,z}\log\Big(\ph_{j,z}\,c\,e^{R'\delta}\Big)> C e^{-R}$. Thus, $\CE(\What_B)>\CE(\Wstar_B)$, a contradiction.

\noindent\emph{\underline{Case (ii):}}~We can assume $\What\in\Tc_\perp$,
since otherwise we are in Case (i). Now, again ignoring all but the $(j,z)$ term in the CE loss for which \eqref{eq:contra 2} holds for some $v\notin\Sc_j$, we find
\begin{align}\label{eq:towards Wb 3}
&\CE(\What_B)-\Hc\geq \pih_j\ph_{j,z}\log\Big({\ph_{j,z}}\big(\sum_{z'\in\Sc_j}e^{(\ell_{j,z'}-\ell_{j,z})}+e^{(\ell_{j,v}-\ell_{j,z})}\big)\Big)\nn.
\end{align}
Using $\Pc_\Tc(\What_B)=\Wstar$ yields
\[
\sum_{z'\in\Sc_j}e^{(\ell_{j,z'}-\ell_{j,z})} = \sum_{z'\in\Sc_j}\frac{\ph_{j,z'}}{\ph_{j,z}} = \frac{1}{\ph_{j,z}}\,.
\]
Moreover, by \eqref{eq:contra 2}:
\[
e^{\ell_{j,v}-\ell_{j,z}}\geq e^{-R'(1-\delta)} \,e^{\ellstar_{j,v}-\ellstar_{j,z}} \geq c' e^{-R'(1-\delta)}, 
\]
for constant  (independent of $B$) $c':=e^{-\|\Wstar\|M}$.
Putting the above together yield:
\begin{align}\nn
    \CE(\What_B) - \Hc &\geq \pih_j\ph_{j,z}\log\Big(1+\ph_{j,z}c'e^{-R'(1-\delta)}\Big) \geq \frac{c'e^{-R'(1-\delta)}}{2n^2}\,.
\end{align}
where the second inequality uses $\log(1+x)\geq \frac{x}{1+x}, x>0$. 

Compare this with \eqref{eq:reg path up}. For large enough $B$, (recall $R,R'$ grow at the same rate) it holds $\frac{c'}{2n^2}e^{-R'(1-\delta)}> C e^{-R}$. Thus, $\CE(\What_B)>\CE(\Wstar_B)$, a contradiction.

In either case, we arrive at a contradiction, which completes the proof.

==> Arxiv_NewTempl/sections/proofs_old.tex <==
% \section*{Todo}
% \begin{itemize}
%     \item Define $\Wstar$ as the unique $\W$ on $S$ that satisfies \eqref{eq:Wf condition}.
%     \item check in sims that finite component is indeed $\Wstar$.
%     \item Break \NTP-separability in two? First condition is \NTP-separability: this guarantees that in the limit the model learns the sparsity pattern. Second condition is that \eqref{eq:Wf condition} has a solution -- an option is to call this $\NTP_\Hc$ because if this holds then it opens the way to approach entropy. 
%     \item (Not so improtant rn:) See what it takes to prove that $\CE_S$ is strongly convex on sublevel sets.
%     \item Actually, a better alternative is to just add a rephrasing/reinterpretation of the condition such that it asks that there exist single $\W$ where $S$ component satisfies \eqref{eq:Wf condition} and complement satisfies \eqref{eq:Wmm condition larger}
%     \item say that set S depends on data: features and label

%     \item \ct{are there settings where either of \eqref{eq:Wmm condition} or \eqref{eq:Wf condition} but not both are satisfied?}
%\end{itemize}


\section{Proofs}

\subsection{Notations}\label{sec:notation}
Throughout, lowercase and uppercase bold letters (e.g., $\ab$ and $\A$) represent vectors and matrices, respectively. $\inp{\cdot}{\cdot}$ and $\norm{\cdot}$ denote Euclidean inner product and  norm, respectively. For matrix $\A$, we denote its pseudoinverse as $\A^\dagger$. All logarithms are natural logarithms (base $e$). We denote $\eb_v$ the $v$-th standard basis vector in $R^V$. $\Delta^{V-1}$ denotes the $V$-dimensional unit simplex and $\sft{}:\R^V\rightarrow\Delta^{V-1}$ the softmax map:
\[
\sft{\ab} = [\sfti{1}{\ab},\ldots,\sfti{V}{\ab}]^\top,\qquad \text{with}~~\sfti{v}{\ab}=\frac{e^{\eb_v^\top\ab}}{\sum_{v'\in[V]}e^{\eb_{v'}^\top\ab}}\,.
\]
As explained in Section \ref{sec:setup} we represent a training set as 
\[
\Tc_m:=\{(\hd_j,\pih_j,\ph_{j,z\in\Vc})\}_{j\in[m]}\,.
\]
We assume that embeddings are bounded and denote
\[
M:=\sqrt{2}\max_{j\in[m]}\|\hd_j\|\,.
\]
Given $\Tc_m$, let
\[
{\Ts}=\operatorname{span}\left(\Big\{(\eb_z-\eb_{z'})\hd_j^\top\,:\,z\neq z'\in\Sc_j, j\in[m]\Big\}\right)
\]
a subspace of $V\times d$ matrices and $\Ts^\perp$ its orthogonal complement. Denote $\pt,\ptp$ the orthogonal projections onto $\Ts$ and $\Ts^\perp$, respectively. For convenience, for $\W\in\R^{V\times d}$, we denote
\[
\W_\Ts:=\pt(\W)\qquad\text{and}\qquad\W_\perp=\ptp(\W)\,.
\]
Define
\begin{align}\label{eq:CE_T}
    \CE_\Ts(\W) = \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log\left(1+\sum_{z\neq z}e^{-(\eb_z-\eb_{z'})^\top\W\hd_j}\right)\,.
\end{align}
Clearly, for all $\W\in\R^{V\times d},$ it holds $\CE(\W)\geq \CE_\Ts(\W)$. Note also that for all $\W\in\Ts$ and for all $\Ws\in\Ts^\perp$ that satisfy Eq. \eqref{eq:Wmm condition equal}, it holds $\CE_\Ts(\W)=\lim_{R\rightarrow\infty}\CE(\W+R\Ws)$. Thus, under \NTP compatibility and \NTP separability, 
\begin{align}\label{eq:inf CE_T=ent}
\inf_{\W\in\Ts}\CE_\Ts(\W) = \inf_\W\CE(\W) = \ent.    
\end{align}

\subsection{Gradient Descent}

Throughout we assume GD is ran with step-size $\eta\leq 1/(2L)$ where $L$ is the smoothness of CE loss.  This condition is not explicitly mentioned thereafter.

\subsubsection{Auxiliary Lemmata}

% \begin{lemma}
%     The gradient of the CE objective in \eqref{eq:CE2} is given by
%     \begin{align}
%     \hspace{-0.1in}\inp{-\nabla\CE(\W)}{\Ub}  \label{eq:grad}
% =\sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\Big(\sum_{\stackrel{z'\in\Sc_j}{z'\neq z}}s_{j,z'}\,(\eb_z-\eb_{z'})^\top\Ub\hd_j+\sum_{v\notin\Sc_j}s_{j,v}\,(\eb_z-\eb_v)^\top\Ub\hd_j\Big),
% \end{align}
% where $s_{j,z}:=$
%     In particular, the gradient is $L=$-Lipschitz.
% \end{lemma}


The following result follows from standard optimization analysis  for smooth convex functions specialized to functions that do not attain their infimum. The version presented here is adopted from \cite[Lemma 2]{ji2020directional}.
\begin{lemma}\label{lem:CE reaches min}
    It holds
    \[
    \lim_{k\rightarrow\infty}\CE(\W_k) = \inf_{\W}\CE(\W)
    \]
    and also $\lim_{k\rightarrow\infty}\|\W_k\|=\infty$.
\end{lemma}

In the lemma below, we collect some useful and simple-to-show properties of the GD and regularization paths. Analogous results, for the different setting of one-hot binary classification over general non-separable data have been established in \cite{ji2018risk}. 

\begin{lemma}\label{lem:iterate limit properties}
    Suppose conditions \eqref{eq:Wmm condition} hold for some $\Ws$. Also, that there exists $\Wf=\Wstar\in\Ts$ satisfying condition \eqref{eq:Wf condition}. The following hold:
    \begin{enumerate}
        \item $\CE_\Ts(\Wstar)=\inf_{\W\in\Ts}\CE_\Ts(\W)=\Hc,$
        \item $\Wstar$ is the \emph{unique} minimizer of $\CE_\Ts$ on the subspace $\Ts$,
        \item $\lim_{k\rightarrow\infty}\Pc_\Ts(\W_k) = \Wstar,$ where $\W_k$ are GD iterates,
        \item $\lim_{k\rightarrow\infty}\|\Pc_\perp(\W_k)\| = \infty,$
        \item $\lim_{B\rightarrow\infty}\Pc_\Ts(\What_B) = \Wstar,$ where $\What_B$ is the reguarlized solution \eqref{eq:reg-path},
        \item $\lim_{B\rightarrow\infty}\|\Pc_\perp(\What_B)\| = \infty.$
    \end{enumerate} 
    
\end{lemma}
\begin{proof}
    It is easy to check by direct substitution of $\Wstar$ in \eqref{eq:CE_T} and use of \eqref{eq:Wf condition} that $\CE_\Ts(\Wstar)=\ent$. This and \eqref{eq:inf CE_T=ent} show the first claim.

    The first claim shows $\Wstar$ is a minimizer. Suppose for the sake of contradiction there is a different minimizer $\Wstar\neq \W_1\in\Ts$. Then, since $\CE_\Ts(\W_1)=\ent$, it also holds for $\W_R:=\W_1+\R\Ws$ that $\lim_{R\rightarrow\infty}\CE(\W_R)=\Hc$. In turn, this implies  for all $j\in[m]$:
    
\begin{align}
    \lim_{R\rightarrow\infty}\sfti{z}{\W_R\hd_j}=\ph_{j,z}, \forall z\in\Sc_j\,,\qquad\text{and}\qquad
    \lim_{R\rightarrow\infty}\sfti{v}{\W_R\hd_j}=0, \forall v\notin\Sc_j\,.\nn
\end{align}    
The first condition gives then that $\W_1$ must satisfy \eqref{eq:Wf condition}. Since $\Wstar$ also satisfies these equations, denoting $\W_\Delta=\Wstar-\W_1\neq 0$, it holds:
\[
\inp{\W_\Delta}{(\eb_z-\eb_{z'})^\top\hd_j)} = 0, \,\forall j\in[m], z\neq z'\in\Sc_j.
\]
But $\W_\Delta\in\Ts$, so this forms a contradiction. Hence, $\Wstar$ is unique solution in $\Ts$ of \eqref{eq:Wf condition} and unique minimizer of $\CE_\Ts$ on the subspace $\Ts.$

The proof of the third claim follows the same way as the proof of part (1) of \cite[Thm.~15]{ji2020directional}. For completeness: It follows by theorem assumptions and Lemma \ref{lem:CE reaches min} that $\lim_{k\rightarrow\infty}\CE(\W_k)=\Hc$. Combining with the first claim of the lemma yields $\lim_{k\rightarrow\infty}\CE(\W_k)=\CE_\Ts(\Wstar)$. Since $\CE_\Ts(\W_k)\leq\CE(\W_k)$, this finally gives 
\[\lim_{k\rightarrow\infty}\CE_\Ts(\W_k)=\lim_{k\rightarrow\infty}\CE_\Ts\left(\Pc_\Ts(\W_k)\right)=\CE_\Ts(\Wstar).\]
Since $\Wstar$ is the unique by the second claim, the desired then follows.

For the fourth claim, recall from Lemma \ref{lem:CE reaches min} that $\lim_{k\rightarrow\infty}\|\W_k\|=\infty$. From the previous claim, we also have $\lim_{k\rightarrow\infty}\|\Pc_\Ts(\W_k)\|<C$ for some constant $C>\|\Wstar\|$. Thus, the desired follows by applying the fact that $\|\W_k\|=\|\Pc_\Ts(\W_k)\|+\|\Pc_\perp(\W_k)\|.$

The proof of the last two claim is exactly same as that of the third and fourth claim. Only now use the facts that $\lim_{B\rightarrow\infty}CE(\W_B)=\ent$ and $\lim_{B\rightarrow\infty}\|\W_B\|=\infty$ (see proof of Theorem \ref{thm:reg-path}). 
\end{proof}


\subsubsection{Key Lemma}
\begin{lemma}\label{lem:key}
    Let $\W_k$ denote the GD iterate at iteration $k$. Recall the decomposition $\W_k=\W_{k,\Ts} + \Pc_\perp(\W_k) = \W_{k,\Ts}+\W_{k,\perp}$. Fix any $\alpha\in(0,1)$. There exists large enough $R=R(\alpha)$ and $k_0=k_0(R)$ such that for any $k\geq k_0$, it holds that  $\|\W_{k,\perp}\|\geq R$ and
    \begin{align}\label{eq:main claim}
        \CE\big(\,\W_{k,\Ts}+(1+\alpha){\|\W_{k,\perp}\|}\overline\Wmm\,\big) \leq \CE(\W_k)\,.
    \end{align}
\end{lemma}
\begin{proof}
We drop the subscript $k$ to lighten notation.

First, note by Lemma \ref{lem:iterate limit properties} that, for arbitrary $R$, we can pick $k_1=k_1(R)$ such that for all $k\geq k_1$: $\|\W_\perp\|\geq R$. 


    Thus next, we will prove the main claim, i.e. for large enough $\|\W_\perp\|$ inequality \eqref{eq:main claim} holds. Denote $R'=\frac{\|\W_\perp\|}{\|\Wmm\|}$. Substituting in CE expression \eqref{eq:CE2}, and using the fact that $\Wmm\in\Ts^\perp$ by \eqref{eq:Wmm condition equal} yield:
    \begin{align}\nn
        &\CE\big(\,\W_\Ts+(1+\alpha)R'\Wmm\,\big) \\
        &= \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( \sum_{z'\in\Sc_j}e^{-(\eb_z-\eb_{z'})^\top\W_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-(1+\alpha)R'(\eb_z-\eb_{v})^\top\Wmm\hd_j}\right)\,.\nn
        \\
        &= \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-(1+\alpha)R'(\eb_z-\eb_{v})^\top\Wmm\hd_j}\right)\,.\label{eq:LHS CE comp}
    \end{align}
% Let $\What:=\What_{\|\W\|}$ be the regularized minimizer in \eqref{eq:reg-path} for $B=\|\W\|$. By its optimality, it holds that
% \[
% \CE(\What)\leq \CE(\W).
% \]
    Moreover, decomposing $\W=\W_\Ts+\W_\perp$, and defining
 \[
 \Wt_\perp := \frac{\|\Wmm\|}{\|\W_\perp\|}\W_\perp\ = \frac{1}{R}\W_\perp\,,
 \]
 we have
        \begin{align}
        \CE\big(\W\big) &= \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( \sum_{z'\in\Sc_j}e^{-(\eb_z-\eb_{z'})^\top\W_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wt_\perp\hd_j}\right)\,\nn
        \\
    &=\sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wt_\perp\hd_j}\right)\,\,,
        \label{eq:RHS CE comp}
    \end{align}
    where we used that, by definition, $\W_\perp\in\Ts^\perp$. Thus, our goal becomes showing $\eqref{eq:LHS CE comp}\leq\eqref{eq:RHS CE comp}$, for large enough $R$. To do this, we consider two cases as follows below.

    For the remaining of the proof denote $M:=\max_{j\in[m]}\sqrt{2}\|\hd_j\|$ and use the logits shorthand:
    \[
    \ellt_{j,v} = \eb_v^\top\Wt_\perp\hd_j\qquad\text{and}\qquad\ellmm_{j,v}=\eb_v^\top\Wmm\hd_j\,.
    \]
    
    \vp
    \noindent\underline{\emph{Case 1: $\W_\perp$ is well aligned with $\Wmm$}.} Suppose
    \begin{align}\label{eq:suppose close}
    \|\Wmm - \Wt_\perp\| \leq \eps:=\frac{\alpha}{M}.    
    \end{align}
    Using this, linearity of logits, and Cauchy-Schwartz, yields
        \begin{align}
        \ellt_{j,z}-\ellt_{j,v} \leq \ellmm_{j,z}-\ellmm_{j,v} + \eps M\nn, ~~ \forall j\in[m], z\in\Sc_j, v\notin\Sc_j\,.
    \end{align}
    Thus,
    \begin{align}
        \sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wt_\perp\hd_j} \geq e^{-\eps M R'}\,\sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wmm\hd_j} = e^{-{\alpha R'}}\,\sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wmm\hd_j}\nn
    \end{align}
Also recall by feasibility of $\Wmm$ that 
\begin{align}\label{eq:app lmm property good}
    \ellmm_{j,z}-\ellmm_{j,v}\geq 1, \forall j\in[m], z\in\Sc_j, v\notin\Sc_j\,.
\end{align} Thus,
    \begin{align}
        \sum_{v\notin\Sc_j}e^{-(1+\alpha)R'(\eb_z-\eb_{v})^\top\Wt_\perp\hd_j} \leq e^{-\alpha R'}\,\sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wmm\hd_j}\nn
    \end{align}
    Comparing the above two displays yields 
    \[
    \sum_{v\notin\Sc_j}e^{-(1+\alpha)R'(\eb_z-\eb_{v})^\top\Wt_\perp\hd_j}\leq \sum_{v\notin\Sc_j}e^{-R'(\eb_z-\eb_{v})^\top\Wt_\perp\hd_j},
    \]
    which implies the desired \eqref{eq:LHS CE comp}$\leq$\eqref{eq:RHS CE comp} for any value of $R'$ (eqv. $\|\W_\perp\|$).

 \vp
    \noindent\underline{\emph{Case 2: No alignment}.} Suppose
    now that \eqref{eq:suppose close} does not hold. Note that $\|\Wt_\perp\|=\|\Wmm\|$ and since \eqref{eq:SVM} has a unique solution it must be that $\Wt_\perp$ is not feasible. But $\Wt_\perp\in\Ts_\perp$, thus it satisfies the equality constraints. This then means that there exist $\delta:=\delta(\eps)$ and $j_\star\in[m],v_\star\notin\Sc_{j_\star}$ such that
    \begin{align}\label{eq:violate}
        \ellt_{j_\star,z}-\ellt_{j_\star,v_\star} \leq 1-\delta\,,~~\forall z\in\Sc_{j_\star}.
    \end{align}
    (Note the above holds for all $z\in\Sc_{j_\star}$ because $\ellt_{j_\star,z}=\ellt_{j_\star,z'}$ since $\Wt_\perp\in\Ts_\perp.$)

To continue, we introduce the shorthand notation
\[
A_{j,z}:=A_{j,z}(\W)= \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}
\]
as well as
\[
A_{\min}:=\min_{j\in[m],z\in\Sc_j} A_{j,z},\qquad\text{and}\qquad
A_{\max}:=\max_{j\in[m],z\in\Sc_j}A_{j,z}\,.
\]
    
    Using \eqref{eq:violate} we may lower bound \eqref{eq:RHS CE comp}  as follows:
\begin{align}
\CE(\W) - \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j} \right) &\geq \pih_{j_\star}\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left(1+\frac{e^{-R'(\eb_z-\eb_{v_\star})^\top\Wt_\perp\hd_{j_\star}}}{A_{j_\star,z}}
        \right)\nn\\
        &\geq \pih_{j_\star}\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( 1+\frac{e^{-R'(1-\delta)}}{A_{\max}}\right)\nn
        \\
        &\geq \frac{e^{-R'(1-\delta)}}{n(A_{\max}+1)}
        \label{eq:RHS CE comp 2}\,,
    \end{align}
    where in the last line we used $\pih_{j}\geq 1/n, \forall j\in[m]$ as well as $\log(1+x)\geq \frac{x}{1+x}, x>0$.
    
    On the other hand, using property \eqref{eq:app lmm property good} for max-margin logits,
    we can upper bound \eqref{eq:LHS CE comp} as follows:
    \begin{align}
\CE\big(\,\W_\Ts+(1+\alpha)R'\Wmm\,\big)  - \sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\log
        \left( \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j} \right) &\leq    \log\left(1+\frac{V\,e^{-R'(1+\alpha)}}{A_{\min}}\right)\,\nn
        \\
        &\leq \frac{V\,e^{-R'(1+\alpha)}}{A_{\min}},\label{eq:LHS CE comp 2}
    \end{align}
    where in the last line we used $\log(1+x)\leq x, x>0.$
    
    In view of the two last displays, it suffices that
    \[
    V\,\frac{e^{-R'(1+\alpha)}}{A_{\min}} \leq \frac{e^{-R'(1-\delta)}}{n(A_{\max}+1)} ~~\Longleftrightarrow~~ R;\geq \frac{1}{\delta+\alpha}\log\left(\frac{n V (A_{\max}+1)}{A_{\min}}\right)\,.
    \]
    All it remains is obtaining bounds for $A_{\min}, A_{\max}$ specifically showing that they do not depend on $R$. By Cauchy-Schwartz: 
    \[
    V e^{-M\|\W_\Ts\|}\leq \A_{\min}\leq\A_{\max}\leq V e^{M\|\W_\Ts\|}
    \]
    Further recall by Lemma \ref{lem:iterate limit properties} that if $k$ is large enough then
    \begin{align}\label{eq:W-Wstar}
    \|\W_\Ts-\Wstar\|\leq {\|\Wstar\|} \implies \|\W_{\Ts}\| \leq 2\|\Wstar\|.
    \end{align}
    Thus, there exists $k_\star=k_\star(\|\W_\star\|)$ such that for all $k\geq k_\star$:
    \[
    V e^{-2M\|\W_\star\|}\leq \A_{\min}\leq\A_{\max}\leq V e^{2M\|\W_\star\|}.
    \]
    Hence, the desired \eqref{eq:LHS CE comp 2}$\leq$\eqref{eq:RHS CE comp 2} holds provided
    \begin{align}
    \|\W_\perp\|\geq \frac{\|\Wmm\|}{\alpha}\log\left(2nVe^{4\|\Wstar\|}\right)\,.\label{eq:wperplb}
    \end{align}
    
    Set $R=R(\alpha)=\{\text{RHS of \eqref{eq:wperplb}}\}$ and 
    $k_0(R):=\max\{k_1(R),k_\star\}$. We have shown this guarantees for all $k\geq k_0$: $\|\W_\perp\|\geq R$ and by choice of $R$ also  \eqref{eq:LHS CE comp 2}$\leq$\eqref{eq:RHS CE comp 2}. This in turn implies \eqref{eq:LHS CE comp}$\leq$\eqref{eq:RHS CE comp}, as desired to complete the proof.
\end{proof}



\subsubsection{Proof of Theorem \ref{thm:GD main}}

The key ingredient of the proof is Lemma \ref{lem:key}. After that, the proof follows identically to \cite[Thm. 15(2)]{ji2020directional}. We include the details for completeness.

Let any $\eps\in(0,1)$ and choose $\alpha=\eps/(1-\eps)$. By Lemma \ref{lem:key}, there exists $k_0$ such that for any $k\geq k_0$, we have
\[
\|\W_{k,\perp}\| \geq \max\{R(\alpha),1/2\}
\]
and
\begin{align}
\inp{\nabla\CE(\W_k)}{\W_{k,\perp}-(1+\alpha)\|\W_{k,\perp}\|\overline\Wmm} &=     \inp{\nabla\CE(\W_k)}{\W_{k}-(\W_{k,\Ts}+(1+\alpha)\|\W_{k,\perp}\|\overline\Wmm)}\nn\\
&\geq 
\CE(\W_{k})-\CE(\W_{k,\Ts}+(1+\alpha)\|\W_{k,\perp}\|\overline\Wmm) \geq 0\,,\nn
\end{align}
where we also used convexity of the loss.

Consequently,
\begin{align*}
    \inp{\W_{k+1}-\W_k}{\overline\Wmm}&=\inp{-\eta\nabla\CE(\W_k)}{\overline\Wmm}
    \\
    &\geq (1-\eps)\inp{-\eta\nabla\CE(\W_k)}{\overline{\W_{k,\perp}}}
    \\
    &\geq (1-\eps)\inp{\W_{k+1,\perp}-\W_{k,\perp}}{\overline{\W_{k,\perp}}}
    \\
    &\geq (1-\eps)\inp{\W_{k+1,\perp}-\W_{k,\perp}}{\overline{\W_{k,\perp}}}
    \\
    &= \frac{(1-\eps)}{2\|\W_{k,\perp}\|}\left(\|\W_{k+1,\perp}\|^2-\|\W_{k,\perp}\|^2 - \|\W_{k+1,\perp}-\W_{k,\perp}\|^2\right)
    \\
    &\geq (1-\eps)\left(\|\W_{k+1,\perp}\|-\|\W_{k,\perp}\| - 2\eta(\CE(\W_{k,\perp})-\CE(\W_{k+1,\perp})\right),
\end{align*}
where the last step used $\|\W_{k,\perp}\|\geq 1/2$, the fact that $x^2-y^2\geq 2y(x-y), \forall x,y$ and smoothness of the CE loss.

Telescoping the above expression and rearranging yields
\begin{align*}
    \inp{\overline\W_k}{\overline{\Wmm}} &\geq (1-\eps) \frac{\|\W_{k,\perp}\|}{\|\W_k\|}-\frac{\inp{\W_{k_0}}{\overline\Wmm}-(1-\eps)\|\w_{k_0,\perp}\|-\eta\CE(\W_{k_0})}{\|\W_k\|}
    \\
    &\geq (1-\eps) - \frac{\|\W_{k,\Ts}\|_2+\inp{\W_{k_0}}{\overline\Wmm}-(1-\eps)\|\w_{k_0,\perp}\|-\eta\CE(\W_{k_0})}{\|\W_k\|}
\end{align*}
Now recall from Lemma \ref{lem:iterate limit properties} that $\lim_{k\rightarrow\infty}\|\W_k\|=\infty$ and $\lim_{k\rightarrow\infty}\|\W_{k,\Ts}\|=\|\Wstar\|$. Thus, \\
$\lim\inf_{k\rightarrow\infty}\inp{\overline\W_k}{\overline{\Wmm}}\geq 1-\eps.$ Since $\eps$ is arbitrary, the desired follows.

%     \vspace{2in}
%     We do this in two steps, one for the subspace component consisting of the first two summations inside the parenthesis of the two expressions and one for the orthogonal component consisting of the last summation. 

%     \vp
%     \noindent\underline{\emph{Step 1: Subspace component}.} For the remaining of the proof denote $M:=\max_{j\in[m]}\sqrt{2}\|\hd_j\|$, which we will use to bound logits, and, fix some  
%     $
%     \eps \in (0,\|\Wstar\|/2).$
    
%      Recall by Lemma \ref{lem:iterate limit properties} that the following holds:
    
%     \noindent (i) if $B=\|\W\|$ is larger than some $B_0(\eps)$, then 
%     \begin{align}\label{eq:What-Wstar}
%     \|\What_\Ts-\Wstar\|\leq\frac{\eps}{2}.
%     \end{align}
%     (ii) if $k$ is large enough then
%     \begin{align}\label{eq:W-Wstar}
%     \|\W_\Ts-\Wstar\|\leq\frac{\eps}{2}.
%     \end{align}
%     Pick $R\geq B_0(\eps)$ so that for all large enough $k$, it holds $\|\W_\perp\| \geq R\geq B_0(\eps)$. Then, $B=\|\W\|\geq \|\W_\perp\| \geq B_0(\eps)$, which implies \eqref{eq:What-Wstar}. Since $k$ can be large enough, this also implies \eqref{eq:W-Wstar}. Combined, we find that there exists large enough $R(\eps)$ such that
%     \begin{align}\label{eq:What-W are close}
%         \|\What_\Ts-\W_\Ts\|\leq \eps.
%     \end{align}
%     Using this, linearity of logits, and  Cauchy-Schwartz, we can lower-bound  the subspace component in \eqref{eq:RHS CE comp} as
%     \begin{align}
%     \sum_{v\in\Vc}e^{-(\eb_z-\eb_{z'})^\top\What_\Ts\hd_j}+\sum_{v\notin\Sc_j}e^{-(\eb_z-\eb_{v})^\top\What_\Ts\hd_j} &\geq e^{-\eps M} \cdot \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}\nn
%     \\
%     &= \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}-\left(1- e^{-\eps M}\right)\sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}\nn
%     \\
%     &\geq \sum_{v\in\Vc}e^{-(\eb_z-\eb_{v})^\top\W_\Ts\hd_j}-\left(1- e^{-\eps M}\right)\, V\, e^{2M\|\Wstar\|}
%     \end{align}
%     where in the last inequality we used from \eqref{eq:W-Wstar} and triangle inequality that
%     \[
%     \|\W_\Ts\| \leq \|\Wstar\| + \frac{\eps}{2} \leq 2\|\Wstar\|\,.
%     \]
    
%     Therefore, to prove \eqref{eq:suffices}, it suffices that we  prove the following inequality regarding the orthogonal components: \ct{this below is wrong}
%     \begin{align}\label{eq:suffices}
%           \sum_{v\neq \Sc_j}e^{-(1+\alpha)R'(\ellmm_{z}-\ellmm_{v})} \leq \sum_{v\neq \Sc_j}e^{-R''(\ellt_{z}-\ellt_{v})} - \left(1-\eps^{-\eps M}\right) V e^{2M\|\Wstar\|},
%     \end{align}
%     where we also recalled our notation for the logits of $\Wmm$ and $\Wt$.

%         \vp
%     \noindent\underline{\emph{Step 2: Orthogonal component}.}We can now invoke Theorem \ref{thm:reg-path        } as follows. If $B=\|\W\|$ is larger than some $B_1(\eps)$, then 
%     \begin{align}
%     \Big\|\Wmm - \frac{\|\Wmm\|}{\|\What\|}\What\Big\| &\leq \frac{\eps}{2} \,.
%     \end{align}
%     If in addition to that $B$ is larger than $B_0(\eps)$ so that \eqref{eq:What-Wstar} also holds, then we can deduce by triangle inequality that
%     \begin{align}
%          \Big\|\Wmm - \Wt\Big\| &= \Big\|\Wmm - \frac{\|\Wmm\|}{\|\What\|}\What_\perp\Big\|
%          \leq \frac{\eps}{2} + \frac{\|\Wmm\|\big(\eps/2+\|\Wstar\|\big)}{\|\What\|}\nn
%          \\
%          &= \frac{\eps}{2}+\frac{2\|\Wstar\|}{R''},\label{eq:from reg path}
%     \end{align}
%     where, we also use $\|\What\|=\|\W\|$ and  $\eps<\|\Wstar\|$. Pick now  $R\geq\max\{B_0(\eps),B_1(\eps)\}$ so that $B=\|\W\|\geq\|\W_\perp\|\geq R$; hence, \eqref{eq:from reg path} holds.
    
%     Using \eqref{eq:from reg path}, linearity of logits, and Cauchy-Schwartz, yields
%     \begin{align}
%         \ellt_z-\ellt_v \leq \ellmm_z-\ellmm_v + \Big(\frac{\eps}{2}+\frac{2\|\Wstar\|}{R''}\Big) M\nn, ~~ \forall v\in\Sc_j
%     \end{align}
%     Also recall by feasibility of $\Wmm$ that $\ellmm_z-\ellmm_v\geq 1, v\in\Sc_j$, thus:
%     \[
%     e^{-\alpha R'} \sum_{v\neq \Sc_j}e^{-R'(\ellmm_{z}-\ellmm_{v})}\leq \frac{ V e^{-\alpha R'}}{2} + \frac{e^{-\alpha R'}}{2} \sum_{v\neq \Sc_j}e^{-R'(\ellmm_{z}-\ellmm_{v})}\,.\nn
%     \]
%     Applying those two facts it suffices for \eqref{eq:suffices} that the  inequality below holds:
%          \begin{align}\label{eq:suffices_2}
%           \frac{e^{-\alpha R'}}{2} \sum_{v\neq \Sc_j}e^{-R'(\ellmm_{z}-\ellmm_{v})} \leq V e^{-\eps M} +  e^{-\big(\frac{\eps R''}{2}+{2\|\Wstar\|}\big) M}\sum_{v\neq \Sc_j}e^{-R''(\ellmm_{z}-\ellmm_{v})},
%     \end{align}
%     \ct{I stopped here. needs changes below cause exponents changed now}
%     For this to hold, it remains to show that $R''/R'$ is not so large. Indeed,
%     \[
%     \frac{R''}{R'} = \frac{\|\W\|}{\|\W_\perp\|} = \frac{\|\W_\perp\|+\|\W_\Ts\|}{\|\W_\perp\|} \leq  1+\frac{\|\W_\Ts\|}{\|\W_\perp\|} = 1+\frac{\|\W_\Ts\|}{R'\|\Wmm\|} \leq 1+\frac{2\|\Wstar\|}{R'\|\Wmm\|}
%     \]
%     where in the last inequality we used from \eqref{eq:W-Wstar} that 
%     \[\|\W_\Ts\|\leq \|\Wstar\|+\|\Wstar-\W_\Ts\| \geq \|\Wstar\|+\frac{\eps}{2} \geq \frac{3\|\Wstar\|}{2}.\]
%     From the penultimate display, note then that 
%     \begin{align}
%     e^{-R''(\ellmm_{z}-\ellmm_{v})} &\geq e^{-R'\left(1+\frac{2\|\Wstar\|}{R'\|\Wmm\|}\right)(\ellmm_{z}-\ellmm_{v})} = e^{-\frac{2\|\Wstar\|}{\|\Wmm\|}(\ellmm_{z}-\ellmm_{v})}\cdot e^{-R'(\ellmm_{z}-\ellmm_{v})} \nn
%     \\
%     &\geq e^{-2\|\Wstar\|M}\cdot e^{-R'(\ellmm_{z}-\ellmm_{v})} \label{eq:1}
%     \end{align}

%     To complete the proof, note the following. We can choose large enough $R$ so that:
%     \begin{align}\label{eq:2}
%     e^{-\alpha R'}\leq e^{-R \frac{\alpha}{\|\Wmm\|} } \leq 2e^{-\eps M}
%     \end{align}
%     \ct{is the dependence of R on eps a problem?}
%     and also
%     \begin{align}\label{eq:eq3}
%     e^{-\alpha R'}\leq e^{-R \frac{\alpha}{\|\Wmm\|} } \leq e^{-(\eps+2\|\Wstar\|) M}
%     \end{align}

%     Putting together \eqref{eq:eq1}--\eqref{eq:eq3} shows the RHS inequality in \eqref{eq:suffices_2}, as desired to complete the proof.
















% \newpage
% \begin{lemma}
    
% For any $\alpha>0$, there exists $R=R(\alpha)$ such that for any $\W$ with $\|\W\|\geq R$, it holds
% \begin{align}
%     \inp{-\nabla\CE(\W)}{\frac{\W}{\|\W\|}} \leq (1+\alpha)\inp{-\nabla\CE(\W)}{\frac{\Wmm}{\|\Wmm\|}}
% \end{align}

% \ct{try to prove for $\W$ not aligning with $\Wmm$}

% \begin{align}
%     \inp{-\nabla\CE(\W-\Wf)}{\frac{\W-\Wf}{\|\W-\Wf\|}} \leq (1+\alpha)\inp{-\nabla\CE(\W-\Wf)}{\frac{\Wmm}{\|\Wmm\|}}
% \end{align}
    
% \end{lemma}

% Recall by \eqref{eq:grad} that
% \begin{align}
%     &\inp{-\nabla\CE(\W)}{\Ub} = \label{eq:grad}
%     \\
% &~~~~\sum_{j\in[m]}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}{\sum_{v\notin\Sc_j}s_{j,v}}\,\left(\frac{\sum_{z'\in\Sc,z'\neq z}s_{j,z'}\,(\eb_z-\eb_{z'})^\top\Ub\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}+\frac{\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Ub\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}\right),\nn
% \end{align}
% where we denote the output probabilities at $\W$ as $s_{j,v}:=\sfti{v}{\W\hd_j}, v\in\Vc, j\in[m].$ Thus, it suffices to prove the following
% \begin{align}\label{eq:2prove}
% \frac{\sum_{z'\in\Sc,z'\neq z}s_{j,v}\,(\eb_z-\eb_{z'})^\top\Wt\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}+\frac{\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Wt\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}
% \leq (1+\alpha) \left(\frac{\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Wmm\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}\right),
% \end{align}
% where we used the fact that $\Wmm$ satisfies \eqref{eq:Wmm condition equal} and we denote 
% \[
% R':=\frac{\|\W\|}{\|\Wmm\|} \qquad\text{and}\qquad \Wt= \frac{\W}{R'}.
% \]
% For convenience, we will also denote $\ellt_{j,v}$ and $\ellmm_{j,v}$ the logits correspodning to $\Wt$ and $\Wmm$, respectively. 


% \emph{\underline{Case 1:}}~$\|\Wt-\Wmm\|\leq \epsilon$. Using this together with linearity of the logits with respect to decoder, as well as,  $\|\hd_j\|\leq 1$
% and \eqref{eq:Wmm condition equal} yields
% \begin{align}\label{eq:case 1 2prove}
% \text{LHS of \eqref{eq:2prove}}\leq 
% \eps\sqrt{2}\frac{\sum_{z'\in\Sc,z'\neq z}s_{j,z'}\,}{\sum_{v\notin\Sc_j}s_{j,v}}+\eps\sqrt{2}\frac{\sum_{v\notin \Sc_j}s_{j,v}\,}{\sum_{v\notin\Sc_j}s_{j,v}} + \left(\frac{\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Wmm\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}\right)
% \leq (1+\alpha) \left(\frac{\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Wmm\hd_j}{\sum_{v\notin\Sc_j}s_{j,v}}\right),
% \end{align}
% where we also used the fact that $\text{RHS of \eqref{eq:2prove}}\geq 1$, by \eqref{eq:Wmm condition larger}.
% \ct{incomplete}

% \emph{\underline{Case 2:}}~$\|\Wt-\Wmm\|> \epsilon$. Then, for some $\delta=\delta(\eps)$, we have at least one $j\in[m]$ for which at least one of the following is true:

% (i) $\exists z$ and $z'\neq z\in\Sc_{j}$ such that 
% \begin{align}
%     \label{eq:contra 1 app}
%     |\ellt_{j,z}-\ellt_{j,z'}|\geq \delta.
% \end{align}

% (ii) $\exists z\in\Sc_{j}, v\notin\Sc_{j}$ such that 
% \begin{align}\label{eq:contra 2 app}
% \ellt_{j,z}-\ellt_{j,v}\leq 1-\delta.    
% \end{align}

% \noindent\textbf{Scenario (ii).}~Consider first scenario (ii). Then, we can assume that $\ellt_{j,z}-\ellt_{j,z'}=0$ for all $z\neq z'\in\Sc_j$ and all $j\in[n]$, since otherwise scenario (i) would hold. \ct{Thus, the desired simplifies to  ...}

% Define
% \begin{align*}
% \delta_j^{\min}&:=\min_{v\notin\Sc_j} \ellt_{j,z}-\ellt_{j,v} - 1 \qquad\text{and}\qquad
% \delta_j^{\max}:=\max_{v\notin\Sc_j} \ellt_{j,z}-\ellt_{j,v} - 1    .
% \end{align*}
% Consider three sets as follows
% \begin{align*}
% \Ic_1=\{j\in[m]\,|\,\delta_j^{\min}\leq 0.3 \alpha\} \\ 
% \Ic_2=\{j\in[m]\,|\,0.3\alpha\leq \delta_j^{\min}\leq 0.8 \alpha\} \\ 
% \Ic_3=\{j\in[m]\,|\,\delta_j^{\min}\geq 0.8 \alpha\} .
% \end{align*}
% Note by definition of scenario (ii), that $\Ic_1$ is nonempty. 

% \vp
% \textbf{Set $\Ic_1$.} Suppose $j\in\Ic_1$. We claim that
% \begin{align}\label{eq:desired I1}
%     \sum_{v\neq\Sc_j} s_{j,v} (\ellt_{j,z}-\ellt_{j,v})\leq (1+0.5\alpha) \sum_{v\neq\Sc_j} s_{j,v} \leq (1+0.5\alpha)\, {\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Wmm\hd_j}\,.
% \end{align}
% The second inequality follows easily by \eqref{eq:Wmm condition larger}. Below, we prove the first inequality. 
% The claim is obvious if $\delta_j^{\max}\leq 0.5\alpha$. Suppose the contrary and consider the following non-empty set:
% \[
% \Nc:=\{v\notin\Sc_j \,|\, \ellt_{j,z}-\ellt_{j,v}\leq 1+ 0.4\alpha\}.
% \]
% For later use note that 
% \[
% v\notin\Nc\,:\, s_{j,v} \leq e^{-(\ellt_{j,z}-\ellt_{j,v})} \leq e^{-R'(1+0.4\alpha)}.
% \]
% We then have
% \begin{align}
%     \nn\sum_{v\not\in\Sc_j} s_{j,v} (\ellt_{j,z}-\ellt_{j,v}) &= \sum_{v\not\in\Sc_j\cup\Nc} s_{j,v} (\ellt_{j,z}-\ellt_{j,v}) + \sum_{v\not\in\Sc_j,v\in\Nc} s_{j,v} (\ellt_{j,z}-\ellt_{j,v}) \\
%     &\leq (1+\delta_j^{\max})\sum_{v\not\in\Sc_j\cup\Nc} s_{j,v}+(1+0.4\alpha)\sum_{v\not\in\Sc_j,v\in\Nc} s_{j,v}\nn
%     \\
%     &= 1+0.4\alpha + (\delta_j^{\max}-0.4\alpha) \sum_{v\not\in\Sc_j\cup\Nc} s_{j,v}\,.
%     \nn
% \end{align}
% To satisfy the desired \eqref{eq:desired I1}, it suffices that
% $(\delta_j^{\max}-0.4\alpha)\frac{\sum_{v\not\in\Sc_j\cup\Nc} s_{j,v}}{\sum_{v\not\in\Sc_j} s_{j,v}}\leq0.1\alpha$. But we have
% \[\frac{\sum_{v\not\in\Sc_j\cup\Nc} s_{j,v}}{\sum_{v\not\in\Sc_j} s_{j,v}} 
% \leq \frac{V\,s_{j,v}}{s_{j,{v_{\min}}}} 
% \leq \frac{V e^{-R'(1+0.4\alpha)}}{e^{-R'(1+\delta_{j}^{\min})}}\leq Ve^{-0.1R'\alpha},
% \]
% where, in the second inequality $v\not\in\Nc$ and $v_{\min}$ is such that $\ell_{j,z}-\ell_{j,{v_{\min}}}-1=\delta_j^{\min}$.
% Put together, \eqref{eq:desired I1} holds for large enough $R'$.

% %%%%%%%%%%%%%%%%%%%%%
% \textbf{Set $\Ic_2$.} Suppose $j\in\Ic_2$.
% We will prove that
% \begin{align}\label{eq:desired I1}
%     \sum_{v\not\in\Sc_j} s_{j,v} (\ellt_{j,z}-\ellt_{j,v})\leq (1+\alpha) \sum_{v\not\in\Sc_j} s_{j,v} \leq (1+\alpha)\, {\sum_{v\notin \Sc_j}s_{j,v}\,(\eb_z-\eb_c)^\top\Wmm\hd_j}\,.
% \end{align}
% The claim is trivially true if $\delta_j^{\max}\leq \alpha$. Thus, assume $\delta_j^{\max}> \alpha$ and define set $\Nc=\{j\not\in\Sc_j:\ellt_{j,z}-\ellt_{j,z}\leq 1+ 0.9\alpha\}$. The proof is then exactly same as for set $\Ic_1$ and is thus omitted for brevity.

% %%%%%%%%%%%%%%%%%%%%%
% \textbf{Set $\Ic_3$.} For samples in $\Ic_3$, we will prove a more relaxed inequality compared to the previous two cases. Namely,
% \begin{align}
% \sum_{j\in\Ic_3}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\sum_{v\notin\Sc_j}s_{j,v}(\ellt_{j,z}-\ellt_{j,v}-1-\alpha)&\leq  \|\Wmm\|\sqrt{2} \cdot\sum_{j\in\Ic_3}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\sum_{v\notin\Sc_j}s_{j,v} \nn
% \\
% &\leq 0.5\alpha \sum_{j\in\Ic_1}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\sum_{v\notin\Sc_j}s_{j,v}.
% \end{align}
% The first inequality simply applies Cauchy-schwarz on the logits. Thus, we need to prove the second inequality.

% For the term in the RHS, note (since $\Ic_1$ is nonempty):
% \begin{align}\label{eq:I3 RHS}
% \sum_{j\in\Ic_1}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\sum_{v\notin\Sc_j}s_{j,v} \geq \min_{j\in\Ic_1}\pih_{j}\min_{z\in\Sc_j}\ph_{j,z}\cdot s_{j,z}   \cdot e^{-R'(1+0.3\alpha)}
% \end{align}
% because by definition of $\Ic_1$, there exists 
% $v\not\in\Sc_j$ such that 
% \[\frac{s_{j,v}}{s_{j,z}} = e^{-R'(\ellt_{j,z}-\ellt_{j,v})} =  e^{-R'(1+\delta_j^{\min})} \geq e^{-R'(1+0.3\alpha)}.
% \]

% For the middle term, note that by definition of $\Ic_3$ (if $\Ic_3$ is empty, then there is nothing to prove and so assume is not), for all
% $v\not\in\Sc_j$ it holds that
% \[\frac{s_{j,v}}{s_{j,z}} = e^{-R'(\ellt_{j,z}-\ellt_{j,v})} \leq  e^{-R'(1+\delta_j^{\min})} \leq e^{-R'(1+0.8\alpha)}.
% \]
% Thus, 
% \begin{align}\label{eq:I3 LHS}
% \sum_{j\in\Ic_3}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\sum_{v\notin\Sc_j}s_{j,v} \leq \sum_{j\in\Ic_3}\pih_j\sum_{z\in\Sc_j}\ph_{j,z}\cdot V \cdot s_{j,z}\cdot e^{-R'(1+0.8\alpha)}.
% \end{align}

% Put \eqref{eq:I3 RHS} and \eqref{eq:I3 LHS} together, it suffices to prove that 
% \begin{align}
%     e^{R'\cdot0.5\alpha} \geq \frac{0.5\alpha}{\|\Wmm\|\sqrt{2}} \frac{\max_{j\in[m],z\in\Sc_j}\pih_{j}\ph_{j,z}}{\min_{j\in[m],z\in\Sc_j}\pih_{j}\ph_{j,z}} \cdot \frac{\max_{j\in\Ic_3,z\in\Sc_j}s_{j,z}}{\min_{j\in\Ic_1,z\in\Sc_j}s_{j,z}}\,.\nn
% \end{align}
% By definition of distinct sequences $j\in[m]$ and 
% associated support-set $\Sc_j$, it holds 
% $\pih_j\ph_{j,z}\geq \frac{1}{n}, \forall j\in[m]z\in\Sc_j.$
% Thus, equivalently it suffices that
% \begin{align}
%     e^{R'\cdot0.5\alpha\,n} \geq \frac{0.5\alpha}{\|\Wmm\|\sqrt{2}}  \cdot {\max_{j\in\Ic_1,z\in\Sc_j}\frac{1}{s_{j,z}}}\,.\nn
% \end{align}


==> Arxiv_NewTempl/sections/rank_feas.tex <==
\section{On the feasibility of \eqref{eq:ufm-svm}}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/feas_V=32_m=100.eps} 
\includegraphics[width=0.45\linewidth]{figures/feas_V=32_m=500.eps} 
\captionsetup{width=\textwidth}
    \caption{Numerical study of feasibility of \eqref{eq:ufm-svm} for varying values of embedding dimension $d$ and maximum sparsity $\max_{j\in[m]}S_j$. Yellow indicates feasibility, while blue denotes infeasibility. Refer to the text for further details.\ct{
    \textbf{@Yize:} If you share with me the support-set pattern of your experiments, i.e. send me a $V\times m$ matrix with 1/0 if belong/not in support, then I can check feasibility for $d\leq V-1$.}}
    \label{fig:feasibility}
\end{figure}

o further explore the feasibility of Equation \eqref{eq:ufm-svm} under varying ambient dimensions $d$, we conducted numerical experiments as detailed below. Our objective is to assess the feasibility of the following non-convex problem:
\begin{align}
    &~~~\text{find}~~~~~\Lb\in\R^{V\times m}\label{eq:feas non-convex}
    \\
    &\text{subj. to}~~ \Ebin{j}\ellbb_j = 0, j\in[m]
    \nn 
    \\
    &\qquad\qquad~\Ebout{j}\ellbb_j \geq 1, j\in[m]\nn
    \\
    &\qquad\qquad~\rank{\Lb}\leq d\nn.
\end{align}
We have theoretically established feasibility for $d\geq V-1$, regardless of the support set pattern or size. Specifically, we have proven the existence of $\Lb$ satisfying the affine constraints and $\ones_V^\top\Lb=0$.

For smaller $d$ values, we adopt a numerically efficient heuristic as follows. For a given $d\geq 2$, we generate $V-(d-1)$ random vectors orthogonal to $\ones_V$, ensuring linear independence. These vectors are then arranged as rows in a matrix $\A^{(V-(d-1))\times V}$. We reformulate the problem as a feasibility linear program (LP), replacing the non-convex rank constraint in \eqref{eq:feas non-convex} with $\A\Lb=0$ and $\ones^\top\Lb=0$. If this LP is feasible, indicating a solution, then the original problem is also feasible. However, due to the fixed rows of $\Ab$, infeasibility of the LP does not conclusively imply infeasibility of the original problem. Thus, our experimental results provide conservative estimates of feasibility for the original non-convex program.

In Figure \ref{fig:feasibility}, we present the outcomes of solving the LP feasibility program under the following experimental conditions. We set $V=32$ and $m=100$ and establish a maximum support length $\max_{j\in[m]}S_j$, randomly generating support sets of sizes up to this maximum length. The maximum support length varies from $1$ (representing the one-hot encoding scenario) to $16$.

For each case, we solve the LP feasibility program for $d$ ranging from $V-1=31$ to $7$. We conduct $100$ iterations of the LP feasibility program for each $d$ value, utilizing different realizations of the random matrix $\A$. If a feasible solution is found within these iterations, we denote it with a yellow square ($1$) in the figure; otherwise, a blue square ($0$) is displayed.

\ct{Can we say something analytical about feasibility of \eqref{eq:ufm-svm}?}
\red{Suppose feasible $\Lb$ of rank $d$ exists. Then, there exists $\pb_j>0, j\in[m]$ and
$\bb_j=\ind{S_j^c}\odot \pb_j$ such that
\[
\Pib_j\Eb\ellbb_j = \bb_j
\]
where $\Eb^\top=\begin{bmatrix}
\ones_{V-1} & -\Id_{V-1}
\end{bmatrix}$
and $\Pib_j$ is a permutation matrix. Here, we also used that there exists permutation $\Pib_j$ so that
\[
\begin{bmatrix}
    \Ebin_j
    \\
    \Ebout_j
\end{bmatrix} =  \Eb\Pib_j^\top
\]
%
Can we show that there exists $\pb_j$ such that the matrix with columns
\[
\ellbb_j = \Pib_j\A\left(\ind{S_j^c}\odot \pb_j\right)
\]
has rank $\leq d$? Here,
\[
\A=\Eb^\top(\Eb\Eb^\top)^{-1}=\begin{bmatrix}
    \ones_{V-1}^\top
    \\
    \ones\ones^\top-V\Id_{V-1}
\end{bmatrix}\,.
\]
}


==> Arxiv_NewTempl/sections/rel_long.tex <==
This section expands upon the section on related work in the main body, which we kept brief due to space constraints. 

\subsection{Word embeddings as matrix factorization}
% \noindent\textbf{Word embeddings as matrix factorization.}~
Neural probabilistic language models are designed to predict the probability distribution of a target word $v\in\Vc$ within a given vocabulary 
$\Vc$, based on a sequence of preceding or surrounding words known as the context $\z\in\Vc^*$. In these models, word and context representations (aka embeddings) are parameterized by their internal architecture \citep{neural_language_models_2}. The emergence of energy-based models like the Word2Vec family, particularly through the introduction of training methodologies such as the Skip-Gram with Negative Sampling (SGNS) objective by \citet{word2vec_1,word2vec_2}, marked a significant advancement in this domain; e.g., see \citep{modern_nlp_book}. SGNS aims to optimize the alignment between vectors of common word-context \tina{clarify context} pairs and disassociate those of randomly drawn pairs. While intuitive, the objective remained somewhat mysterious until the seminal analysis by \citet{levy} offered a formal examination of embeddings generated by the SGNS objective, framing it as a form of weighted matrix factorization. Specifically for embeddings of large dimensionality, Levy and Goldberg demonstrated that SGNS implicitly factorizes a shifted version of the Pointwise Mutual Information (PMI) matrix, denoted as 
$\PMI$, which is a measure of association between words and contexts by having entries  $\PMI[z,j]=\log\frac{\rm{Pr}(z|j)}{\rm{Pr}(z)}=\log\frac{\ph_{j,z}}{\rm{Pr}(z)}$ for word $z$ and context $j$. However, this approach presumes non-zero occurrences of all context-word pairs in the training set, a condition not always met, leading to undefined factorization for pairs with zero co-occurrence (resulting in 
$\PMI[z,j]=-\infty$). To address the PMI matrix's potential to include negative infinity values, an approximation involving a positive, sparse, and non-negative PMI (PPMI) matrix was proposed. While this adaptation offered an intriguing alternative to the original training objectives, the geometric characteristics of the resultant embeddings in comparison to those derived from the original loss remain unclear.

Our research intersects with these foundational studies, particularly in our interest in the geometric structures of word and context embeddings. Our approach mirrors that of \citet{levy} to some extent, especially in treating NTP as a soft-label classification across distinct contexts and presuming unconstrained context embeddings (although these concepts are not clearly mentioned in those original works). At a very basic level our work distinguishes itself by focusing on the NTP objective, which, although akin to SGNS and NC objectives, employs cross-entropy loss instead of sigmoid functions. Aside from this distinction, we identify the following conceptual divergences, contributing to our novel perspective on this line of inquiry: \textbf{(i)} Firstly, we aim to characterize the geometry of embeddings as learned directly from the loss function, rather than through approximations. \textbf{(ii)} Secondly, we confront the sparsity in the probabilistic labels of each context head-on, identifying that sparsity leads to diverging embeddings, a scenario where setting the loss gradient to zero is infeasible with finite weights. \textbf{(iii)} Thirdly, by examining embeddings through the lens of the regularization path—a surrogate for gradient descent optimization—we unveil that word and context embeddings emerge from the factorization of a matrix 
$\Lbin+R\Lbmm$. Here, 
$\Lbin$ captures the frequency of word-context occurrences akin to the PMI, setting non-occurring pairs to zero while retaining positive values for occurring pairs, much like the PPMI matrix. The directional component 
$\Lbmm$, becoming dominant as weights diverge, reflects the explicit sparsity patterns of the context-word probability matrix.

The seminal contribution of \citet{levy} has inspired numerous subsequent studies, leveraging the geometric insights of embeddings to uncover linguistic phenomena such as the linear relationships underlying word analogies \citep{allen2019analogies,ethayarajh2019contextual,hashimoto2016word,arora2016latent,ethayarajh2018towards,mikolov2013linguistic}. We envision that our fresh perspective on geometric analysis and our findings could similarly motivate further research in this domain, extending the understanding and application of language model embeddings.



\subsection{Overparameterization and Implicit bias/regularization of GD}
% \noindent\textbf{Overparameterization and Implicit bias/regularization of GD.}
Recent studies on gradient-based optimization methods, such as SGD and its variants, have focused on overparameterized settings in empirical risk minimization without explicit regularization. This interest stems from observations that deep neural networks, especially in image classification, perform exceptionally well even with minimal or no weight decay. This research area, known as ``implicit bias'' or ``implicit regularization'' of GD emerged to explore which among the numerous potential minimizers in overparameterized settings are preferred by algorithms like GD. Notably, \citet{soudry2018implicit,ji2018risk} showed that for linear logistic regression with one-hot labels, GD aligns with the hard-margin SVM solution, essentially becoming the max-margin classifier. Additionally, \citet{ji2020directional} indicated that GD's optimization path in linear models is analogous to the regularization path, which looks at risk minimizers as regularization diminishes. This path is analytically more accessible and offers a useful framework to study GD's behavior.  In our work, we apply this idea to investigate the regularization path of \NTP training.
These foundational results on implicit bias have spurred further research into stochastic and adaptive gradient methods \citep{nacson2019convergence,pesme2021implicit,sun2022mirror,azizan2021stochastic,cattaneo2023implicit}, and more intricate architectures \citep{lyu2020Gradient,ji2020directional,gunasekar2018characterizing,gunasekar2018implicit}) including recent studies on transformers \citep{tarzanagh2023maxmargin,tarzanagh2023transformers}; for a review, refer to \citet{vardi2021implicit}. These insights have also paved the way for generalization analysis, linking GD's generalization to that of SVM-like solutions. This connection has been explored in high-dimensional contexts where traditional margin-based bounds are inadequate, revealing scenarios where no regularization yields optimal outcomes, a phenomenon known as 'harmless interpolation' or 'benign overfitting.' Most of these findings, whether on optimization or generalization, are confined to the one-hot classification framework. A deviation is the work by \citet{ntp} on \NTP as soft-label classification, which partially inspired our research. While their analysis, assuming fixed context embeddings, remains linear, our work extends this by optimizing both word and context embeddings, leading to a nonlinear model. We discover that this nonlinearity yields a preference towards minimizing the nuclear norm of the logits over the Euclidean norm of the word embedding matrix, as seen in \citet{ntp}. Our theoretical contributions thus expand on their findings into the nonconvex domain. Our proof strategies align with the underlying principles found in related implicit bias research \citep{rosset2003margin,ji2020directional}, though we remark the necessity of addressing specific technical nuances in our application of these concepts.


% Those seminal implicit-bias results has inspired extensions to, among others, stochastic and adaptive gradient-based algorithms \cite{nacson2019convergence,pesme2021implicit,sun2022mirror,azizan2021stochastic,cattaneo2023implicit} and more complex architectures  (e.g. \cite{lyu2020Gradient,ji2020directional,gunasekar2018characterizing,gunasekar2018implicit}) even including transformers very recently \cite{tarzanagh2023maxmargin,tarzanagh2023transformers}; see \cite{vardi2021implicit} for a  survey. Notably, it has also provided a means for generalization analysis by translating the question of generalziation of GD to that of generalization properties of SVM-type solutions.  Numerous recent works have studied these properties in high-dimensional settings (where classical margin-based bounds from the 90's fail) and have provably identified settings where zero regularization is indeed optimal leading to what has been termed ``harmless interpolation'' or ``benign overfitting.'' The majority of these results either on optimization or on generalization rely apply to the classical one-hot classification setting. Only recently, \cite{ntp}, who framed \NTP as soft-label-classification, begun investigating implicit regularization in \NTP settings. Their study partly motivated our investigation. While they assume fixed context embeddings, thus study a linear setting, we jointly optimize word and context embeddings giving rise to a nonlinear formulation. We find that this nonlinearity induces a bias towards minimizing the nuclear-norm of the logits, rather than the euclidean norm of word embedding matrix as in \cite{ntp}. Thus, our theoretical results can be seen as an extension of theirs to the nonconvex setting. At a high-level, our proofs follow the same conceptual principles as theirs, which are in fact common in a series of works on implicit bias, e.g. \cite{rosset2003margin,ji2020directional}. However, we note that there are various technical details to be accounted for in specific applications of these ideas to concrete settings. 

\subsection{Neural collapse geometry}
% \noindent\textbf{Neural-collapse geometry.}
A third area of research closely related to our work is the investigation of neural-collapse (NC) geometry, which seeks to understand the geometry of last-layer features and classifier weights in deep networks optimized in the interpolating regime. Initiated by \citet{NC}, this line of research uncovered a universal phenomenon across various architectures and datasets, where classifiers and last-layer features consistently converge to an equiangular tight frame (ETF). This convergence subsumes  the aggregation of same-class features around their class mean, a phenomenon termed NC. The theoretical underpinnings for these empirical findings were later provided by analyzing the unconstrained features model (UFM) \citep{mixon2020neural,fang2021exploring,zhu2021geometric}, suggesting that highly overparameterized networks can produce arbitrary last-layer features. This concept, reminiscent of the early framework used in Word2Vec models \citep{levy} as discussed above, has since spurred extensive research in diverse contexts.

Among the vast body of work on NC geometry--an exhaustive reference of which is beyond our scope--, two studies stand out for their relevance to our research. \citet{seli} first adapted the UFM to describe geometries diverging from symmetric ETF by moving away from the balanced data assumption, demonstrating that logits optimizing the UFM with vanishing regularization align with a nuclear-norm SVM problem. This approach also bridges NC geometry with the implicit bias literature previously discussed. Our work extends their principles to the \NTP objective, differing from the one-hot encoding classification focus of their study. We take a similar approach, but this time applied to the \NTP objective. This is unlike their result which only applies to one-hot encoding classification. In fact, our formulation in \ref{eq:ufm-svm} extends their findings, encompassing them as a specific instance when each context is followed by only one token—a scenario less applicable to the linguistic contexts we focus on. Moreover, we demonstrate (see Theorem~\ref{thm:reg path finite}) that the \NTP framework introduces a finite projection component to the regularization path, a feature absent in one-hot settings.


Our findings also resonate to certain extent with the recent multilabel NC geometry study in \citet{multilabel_nc}, where each example, typically an image, is tagged with multiple correct labels, represented as a $k$-hot vector. In contrast, our \NTP framework, modeled as soft-label classification, associates each context with a probability vector. This distinction makes our framework more versatile, applicable beyond the restrictive case where soft-label classification aligns with multi-label classification—specifically, when all relevant tokens are equally likely. There are also crucial differences in the outcomes. Their analysis assumes an equal number of training samples of multiplicity $k=1$ for each category, a condition that, in our context, would necessitate every vocabulary word to be followed by an identical number of contexts that are only followed by that word—a significantly limiting constraint. Our findings, however, are not bound by this assumption.

\new{In an attempt to extend this line of work to language setups, concurrent work \cite{wu2024linguistic} empirically claims a correlation between the level of convergence to the NC geometry and validation loss for different language models trained on TinyStories for a few epochs. Unlike our approach, they implicitly treat the objective as one-hot classification by suggesting that better \emph{per-class} (i.e., next-token) collapse of the context embeddings leads to improved validation loss. In contrast, our analysis reveals a more intricate result: in the soft-label setup of language models, it is not \emph{per-class} collapse that minimizes the training objective. Instead, the objective is minimized when context embeddings with the same emph{support set} collapse when projected into the \emph{subspace} $\Ts_\perp$, which is defined by the sparsity pattern of the context-word co-occurrence matrix (see Sec.~\ref{}).}



% Our results are also somewhat related to certain extend to the recent work \cite{mutlilabelNC}, where the authors study the NC geometry in multilabel classification. In their setting each example (viewed as image for their focus) shows multiple (say $k$) correct labels, i.e. is associated with a $k$-hot label vector of $0$s and $1$s. Instead, in our framing of \NTP as soft-label classification, each example (here, context) is associated with a probability vector. The two settings are essentially identical only in the spacial case where all on-support tokens are equally likely, making our setting more general. 


% \noindent\textbf{Others.}

% Neural probabilistic language models (NPLMs) specify the distribution for a target word $v\in\Vc$ in a vocabulary $\Vc$, given
% a sequence of words $\z\in\Vc^*$, called the context. The context $\z$ can be a sequence of words that precedes $v$ or it may be comprised by words surrounding $v$ in an $L$-sized window. NPLMs construct word and context  embeddings by parameterizing them in terms of their internal architecture \cite{}. Such models were popularized via a family of energy-based models known as $\rm{word2vec}$ models. Among the first popular versions of these models, \cite{mikolov} proposed training their model with the so-called skip-gram with negative sampling (SGNS) training objective, which tries to maximize the inner-product between vectors of frequently occuring word-context pairs within the training set and minimize it for word-context pairs drawn at random.  In a seminal work \cite{Levy} undertook an analytical investigation of the embeddings produced by the SGNS objective towards developing formal insights behind the reason SGNS is expected to produce good word representations. They framed SGNS as weighted matrix factorization. Concretly, for large embedding dimension they showed that this implies
%  the SGNS implicitly factorizes a (shifted) word-context pointwise mutual information (PMI) matrix. In our notation, $\PMI\in\R^{V\times m}$ with entries $\PMI[z,j]=\log\frac{Pr(z|j)}{Pr(z)}=\log\frac{\ph_{j,z}}{Pr(z)}$ for word $z$ and context $j$. They also showed a similar result for the noise-contrastive (NC) training objective of \cite{Mnih}. These results followed by appropriately expressing the training objective (SGNS or NC) and setting its gradient to zero. However, this argument implicitly assumes that $\ph_{j,z}>0$, i.e. all context-word pairs co-occur in the training set (note in this case the $\PMI[z,j]=-\infty$ so factorization is not well-defined). To circumvent the issue of PMI matrix taking values that are $-\infty$, they propose approximating $\PMI$ with a the so-called positive PMI that is sparse and non-negative. While this yields interesting alternatives to the original training objectives, it is not clear how the resulting embeddings geometry compares to that of the original loss. Our work is closely related to these investigations. We also are interested in the geometry of words and contexts embeddings and we our concepts of (a) framing NTP as soft-label classification over distinct contexts and (b) assuming unconstrained context embeddings, is essentially similar to the approach that they follow (although some of these concepts are not stated explicitly). However, in some respects we argue that our work can be seen as a modern take on their approach. Apart from the difference  that we focus on the NTP objective, which although related to SGNS and NC, uses the CE loss rather than the sigmoid and This difference is not particularly substantial and we believe our approach can be used to revisit from our lens the geometries of other objectives such as SGNS and NC, there are more important conceptual differences attributing to our modern take of the investigation as follows. First, we explicitly focus on understanding the geometry of the embeddings learned by training the loss rather than approximating it with other means. Second, and relatedly, instead of relying on approximation to circumvent sparsity of the probabilistic label of each context, we instead explicitly account for it in our results: We identify that the optimization effect of sparsity is that embeddings diverge (and loss gradient cannot be set to zero for any finite weights). Third, to properly investigate the behavior of diverging weights, we study the behhavior of embeddings through the regularization path, which stands as a proxy to gradient descent optimization. As a result, we find that word and context embeddings result from factorizing a matrix $\Lbin+R\Lbmm$. The finite component $\Lbin$ has entries $\Lbin[z,j]-\Lbin[z',j]=\log\frac{\ph_{j,z}}{\ph_{j,z'}}$ for in-support tokens $z,z'$ and $\Lbin[z,j]=0$ for out-of-support tokens $z$. Thus this matrix captures the frequencies of word/context pairs that appear in the dataset similar to PMI. Also, similar to PPMI it sets the off-support entries to 0 (but allows other on-support positive entries). On the other hand, the directional component $\Lbmm$, which dominates as weights diverge ($R\rightarrow\infty$), captures the explicitly sparsity pattern of the context-word probability matrix. In closing this comparison, the seminal work by \cite{Levy} inspired lots of follow-up works that used these insights in various ways, e.g. using the geometry of these embeddings to reveal interesting linguistic properties such as word analogies being represented as linear translations \cite{}. We anticipate our modern take on the geometry investigation and our results can inspire analogous follow-up investigations.

%Putting the above described concepts together we arrive at a concrete analytical formulation of the task of characterizing the word and context embeddings as that of determining $\GW$, $\GH$ and $\Lb$ for the minimizers of \eqref{eq:NTP intro} with vanishing ridge regularization. We begin by showing a more favorable formulation of \eqref{eq:NTP intro} on the logit space. Specifically, the logit matrix $\Lb$ can be found by minimizing the NTP objective with vanishing \emph{nuclear-norm} regularization and an additional constraint that the rank of $\Lb$ does not exceed the embedding dimension $d$. Given $\Lb$, the word and context matrices $\W$ and $\Hb$ are formed by matrix factorization of $\Lb$. We then focus on large embedding dimension setting $d>V-1=|\Vc|-1$. Here, the nuclear-norm logit minimization becomes convex, and we use this to explicitly characterize its vanishing regularization solution $\Lb_\la$. Concretely, we show that as the regularization $\la\rightarrow 0$ the logit matrix takes the form 
% \[
% \Lb_\la\approx \Lbin + R(\la)\,\Lbmm,
% \]
% where $R(\la)\rightarrow\infty$, $\Lbin$ is a matrix with entries that are zero on off-support tokens and non-zero values that depend on the probability labels on entries corresponding to the on-support tokens, and, finally $\Lbmm$ is the solution to a convex low-rank minimization problem of the logits, wherein in support-logits are constrained to be equal and strictly larger than off-support tokens. The finite component $\Lbin$ depends on the occuring frequencies of the on-support in the dataset, while the value of directional component $\Lbmm$ depends on the sparsity pattern of the support sets. Intuitively, the value of $\Lbmm$ is precisely determined based on the ``company'' that each context keeps'' (in-support tokens) as well as the ``company'' it does \emph{not}.'' 

% First, we adopt framing the NTP training objective over a given training set comprised of context-word pairs as soft-label classification with CE loss over sparse probabilistic labels \cite{ntp}. Concretely, this identifies $m$ \emph{distinct} contexts that may repeat multiple times throughout the training set and associates with each a conditional probability label vector $\pbh_j, j\in[m]$ that captures the frequency with which each token/word appears after context $j$ in the dataset. The sparsity of $\pbh_j$ captures the fact that some words are never follow a given context in the dataset. The second idea allows us to obtain a tractable analysis of context embeddings by assuming that sufficiently large neural-net models can generate embeddings $\hb_j\in\R^d$ for context $j\in[m]$ unconstraindly, i.e. without constraints imposed by the intricacies of the specific model architecture. Thus, this poses NTP training as 
% \begin{align}\label{eq:NTP intro}
% \min_{\W\in\R^{V\times d},\Hb\in\R^{d\times m}} \Lc_{\rm{NTP}}\left(\W\Hb;\Tc=\{\pbh_j\}_{j\in[m]}\right)\,
% \end{align}
% where the word and context embedding matrices $\W,\Hb$ minimize the NTP loss $\Lc$ over the training set $\Tc$ whose relevant statistics are captured by the collection of the sparse probabilistic label vectors $\{\pbh_j\}_{j\in[m]}$ of each distinct context $j$. 
% With this, we frame our goal of determining geometric properties between word-word, context-context and word-context embeddings becomes that of characterizing the gram matrices $\W\W^\top$ and $\Hb\Hb^\top$ and the logit matrix $\Lb=\W\Hb$. Albeit simple to state this task is this challenging owning to the non-convexity of the minimization, the combinatorial nature of the support sets of the probability label vectors but most importantly because of the fact that sparsity of support sets leads to  multiple minimizers making the question of geometry characterization potentially ill-posed. To circumvent this, we leverage the third idea of tracking the specific minimizers (among the multiple many) that are found by the regularization path, i.e. by the path of solutions to \eqref{eq:NTP intro} obtained by minimizing the NTP loss with a vanishing ridge regularization $\lambda\rightarrow 0$ over $W$ and $\Hb$. The core motivation for the relevance of the regularization path is that it is known in various settings that it corresponds to the path followed by gradient-descent optimization.  





\section{Connections to word2Vec}
We can attempt applying the geometry analysis to word2Vec. Consider first the following Skip-gram objective: 
    \[
    \frac{1}{T}\sum_{t\in[T]}\sum_{-c\leq j\leq c, j\neq0} \log p\big(z_{t+j}|z_{t}\big)=\frac{1}{T}\sum_{t\in[T]}\sum_{-c\leq j\leq c, j\neq0} \log p\big(\sfti{z_{t+j}}{\Hb\w_{z_t}}\big)\,,
    \]
    where $\Hb\in\R^{V\times d}$ denotes the embedding matrix of \emph{context} words $z_{t+j}, j\neq 0$ and $\W\in\R^{V\times d}$ denotes the embedding matrix of \emph{target words} $z_t$.
    As presented in \cite{mikolov2013linguistic}, skip-gram actually implements a heuristic of this objective that aims to simplify the computation of the normalizing factor in the softmax. Second, consider the CBOW objective:
    \[
    \frac{1}{T}\sum_{t\in[T]} \log p\big(z_{t}|\{z_{t+j}\}_{\{|j|\in[c],j\neq 0\}}\big)=\frac{1}{T}\sum_{t\in[T]} \log p\left(\sfti{z_{t}}{\W\cdot\frac{1}{2c-1}\sum_{-c\leq j\leq c, j\neq0}\hb_{z_{t+j}}}\right)\,,
    \]
    where $\frac{1}{2c-1}\sum_{-c\leq j\leq c, j\neq0}\hb_{z_{t+j}}$ is the continuous-bags-of-word embedding of the context $\{z_{t+j}\}_{\{|j|\in[c],j\neq 0\}}$. \textbf{Note that in the \NTP setting that we consider, there is \emph{no} explicit parameterization of the embedding of context in terms of the embeddings of its consituent words.} 

    Suppose the CBOW model with context consisting of only the previous word. To keep notation consistent with the rest of the paper, let $j\in[m]=[V]$ denote index of \emph{unique} contexts (aka previous words) and $z\in[V]$ denote index of (next) words. Note the embedding matrix $\Hb\in\R^{d\times V}$ is now of same dimension as $\W^\top$. Let $\pih_j$ denote the marginal of context words and $\ph_{j,z}$ denote the conditional probability of word $z$ following context word $j$. Then, the CBOW objective becomes equivalent to
    \[
\sum_{j\in[V]}\pih_j\sum_{z\in[V]}\ph_{j,z}\log\left(\Sc_{z}\left(\W\hb_j\right)\right)\,.
    \]
    This now fits exactly our framework and the results for NTP apply mutatis mutandis. 

    However, \cite{mikolov2013linguistic}, instead of minimizing the CE objective, they actually use the Negative-Sampling (SGNS) objective. \cite{mikolov2013linguistic} rewrite the SGNS objective as follows:
    \[
    \sum_{j\in[m]}\sum_{z\in[V]} -\Pr(j,z) \log\left(\sigma(\w_z^\top\hb_j)\right)-k\Pr(j)\Pr(w)\log\left(1-\sigma(\w_z^\top\hb_j)\right)\,,
    \]
    where $\Pr(j,z):=\pih_j\ph_{j,z}$, $\Pr(j):=\pih_j$, $\Pr(z)=\sum_{j\in[m]}\pih_j\ph_{j,z}$and $k\in\mathbb{N}$ is a hyperparameter. Defining 
\[q_{j,z}:=\frac{\frac{\Pr(j,z)}{\Pr(j)\Pr(z)}}{k+\frac{\Pr(j,z)}{\Pr(j)\Pr(z)}}\in[0,1]\,,\]
we can rewrite the SGNS objective as 
\[
    \sum_{j\in[m]}\sum_{z\in[V]} \Pr(j)\Pr(w)\left(k+\frac{\Pr(j,z)}{\Pr(j)\Pr(z)}\right)\left(-q_{j,z}  \log\left(\sigma(\w_z^\top\hb_j)\right)-(1-q_{j,z})\log\left(1-\sigma(\w_z^\top\hb_j)\right)\right)\,.
    \]
    For each $(j,z)$-pair, the rightmost term in the expression above is lower bounded by $\ent(q_{j,z}):=-q_{j,z}\log(q_{j,z}) - (1-q_{j,z})\log(1-q_{j,z}).$ 

    By following the same arguments developed for \NTP, it can be checked that the lower bound is attained if and only if the following conditions hold:
    \begin{enumerate}
        \item There exists logit matrix $\Lb_1\in\R^{V\times m}$ (of rank $\leq d$) such that 
        \[
        \Lb_1[z,j]=\text{PMI}(z,j)-\log(k) = \log\left(\frac{\Pr(j,z)}{\Pr(j)\Pr(z)}\right) - \log(k),\quad \forall j\in[m], z\in\Sc_j \].
        \item 
        There exists logit matrix $\Lb_2\in\R^{V\times m}$ (of rank $\leq d$) such that 
        \begin{subequations}
        \begin{align}
        &\Lb_2[z,j]=0,\quad \forall j\in[m], z\in\Sc_j
        \\
        &\Lb_2[v,j]<0,\quad \forall j\in[m], v\notin\Sc_j
        \end{align}
        \end{subequations}
    \end{enumerate}
    

==> Arxiv_NewTempl/sections/related_work.tex <==

\vspace{-0.15in}
\section{Related work}\label{sec:rel work}
\vspace{-0.1in}

\vspace{3pt}\noindent\textbf{Implicit bias of one-hot prediction.} Our work is inspired and is closely related to the literature on implicit bias of CE loss in one-hot supervised classification. \cite{soudry2018implicit} show that for linear models and linearly-separable data, GD converges in direction to the max-margin classifier. This result strengthens older work by \cite{Rosset2003MarginML} who showed that the direction of ridge-regularized CE minimization converges to the same limit as the regularization weight tends to zero. Closer to the nature of our results, \cite{ji2018risk} extend the analysis to encompass general binary data and \cite{ji2020gradient} formalizes the connection the GD and the regularization paths within this broader setting. In that scenario, the training are linearly separable only on a certain subspace, and gradient descent is shown to converge, in direction, towards the max-margin classifier confined within that subspace. On the orthogonal subspace, it converges to a finite point. While operationally similar, our findings for the \NTP objective in Theorems \ref{thm:reg-path} and \ref{thm:GD main} cannot be directly derived from their result since our setting is neither binary nor one-hot. Nevertheless, our proofs follow the same general recipe as these prior works, particularly \cite{ji2020gradient}, and build upon their foundations.

 Numerous other works have also built upon these early influential studies, involving extensions to more complex architectures  (e.g. \cite{lyu2020Gradient,ji2020directional,gunasekar2018characterizing,gunasekar2018implicit}),  stochastic and adaptive gradient-based algorithms \cite{nacson2019convergence,pesme2021implicit,sun2022mirror,andriushchenko2022towards,azizan2021stochastic}, and other supervised learning settings \cite{cattaneo2023implicit,tarzanagh2023maxmargin}; see  \cite{vardi2021implicit} for a  survey.

%In addition a better understanding and interpretability of the optimization properties of GD, 
The implicit bias viewpoint has also created opportunities to study generalization in overparameterized settings. Specifically, a rich line of recent research activity, starting with \cite{hastie2019surprises,bartlett2019benign,montanari2019generalization,deng2019model}, builds on a two-stage approach to generalization analysis of GD. The first stage (optimization), building on implicit bias,  decouples the intricacies of optimization from the generalization query, by describing the solution learnt by GD in terms of a max-margin classifier. The second stage (statistics), investigates the generalization properties of this max-margin classifier under different data and model settings, e.g., \cite{muthukumar2019harmless,chatterji2021does,cao2020generalization,cao2022benign,koehler2021uniform,sur2019modern,frei2022benign}. More recently, this approach has also been leveraged to study the impact of different loss functions on the model fairness \cite{chatterji2021does,kini2021label}. Our results motivate analogous extensions in the richer setting of \NTP training.

%Our work can be seen as the counterpart of the very early works on linear models referenced above, but applied to the NTP classification setting. \ct{talk about relevance to \cite{ji2020directional}} This new setting involves one-hot prediction as a special case ($|\Sc_j|=1, \forall j\in[m]$) and in that sense our results generalize those of previous works. Naturally, they also motivate extensions of these generalizations to more complex settings, as well as, to statistical accuracy and fairness investigations, which we leave to future work.

\vspace{3pt}\noindent\textbf{Implicit bias in transformers.} Our work is also closely related to  \cite{tarzanagh2023transformers}, where the authors investigate the implicit bias of self-attention in transformers. The insight put forth in \cite{tarzanagh2023maxmargin,tarzanagh2023transformers} is that  softmax attention induces implicit-bias behaviors that bear similarities to vanilla implicit bias of one-hot prediction. Concretely, \cite{tarzanagh2023transformers} studies GD optimization of one-layer self-attention with fixed decoder and \emph{one-hot binary} classification. They show that, in the limit, GD finds attention weights that converge in direction to the solution of an SVM problem that separates optimal tokens 
%(those most relevant with the label) 
from non-optimal ones. Their non-convex setting introduces
%In their setting, the landscape is non-convex introducing 
locally optimal SVM directions to which GD may converge depending on initialization. Different to them, the \NTP setting that we study involves predictions over multiple categories and is \emph{not} one-hot. Also, while they fix the decoder, here, we fix the embeddings. In these respects their results are rather different. More similarities arise when \cite{tarzanagh2023transformers} replace the linear decoder  with a MLP, which they note can induce multiple optimal tokens per sequence. This leads them to formulate a more general token-separating SVM program, which similar to ours confines the separation on a certain data subspace. However, the operational nature of the programs remains different as theirs optimizes attention weights and separates tokens within a sequence, while ours optimizes decoder weights and separates context embeddings based on their respective support sets. More importantly, while \cite{tarzanagh2023transformers} only conjectures the convergence of GD to their general SVM program, we leverage convexity in our setting to prove an analogous statement rigorously. Eventually, as we move lower in our top-down approach considering architecture-specific embeddings  generated by attention, we anticipate to see integration of our ideas with  theirs. 

Beyond \cite{tarzanagh2023transformers}, there is growing recent research investigating optimization and generalization principles of transformers %architecture 
\cite{bietti2023birth,sahiner2022unraveling,ergen2022convexifying,edelman2021inductive, likhosherstov2021expressive,Oswald2022TransformersLI, zhang2023trained, akyrek2023what, li2023transformers, tarzanagh2023maxmargin,tarzanagh2023transformers,prompt-attention,tian2023scan}. These efforts predominantly employ a 'bottom-up' approach that  involves isolating shallow transformers, often with simplifications such as removing MLPs, utilizing single heads instead of multiple, and fixing certain parts while training only a subset of trainable parameters. Most of these studies have focused on classical one-hot supervised settings, and only a handful (e.g., \cite{tian2023scan,tian2023joma})  have seeked extending these 'bottom-up' analyses to \NTP settings. Yet, their primary emphasis remains on uncovering the role of attention and how attention weights evolve during training. Instead, our approach uniquely emphasizes the \NTP training paradigm itself, shifting the focus from the intricacies of specific transformer architectures. In a similar vein, interesting work by \cite{malach2023auto} investigates the learning abilities of autoregressive training. Although they share a focus on studying linear predictors, our results primarily concern optimization rather than PAC learnability, as they do.

\vspace{3pt}\noindent\textbf{Classification with Soft Labels.}
Unlike one-hot classification, soft-label classification associates each example with a probability vector, where each entry represents the likelihood of a corresponding label characterizing the example. Although arguably less prevalent than one-hot (or hard-label) classification, soft-label classification arises in various contexts, including modeling human confusion during crowd-sourcing \cite{peterson2019human,soft1,soft2}, knowledge distillation \cite{knowledge-distilation}, and label smoothing \cite{label_smoothing}. Our model of last-token prediction also falls within this setting. Specifically, our approach is most closely related to soft-labels generated by averaging annotators' hard labels \cite{peterson2019human}, rather than following the winner-takes-all rule. \cite{peterson2019human} and follow-up workhave provided empirical evidence that using probabilistic soft labels generated from crowd annotations for training leads to improved performance in terms of model generalization, calibration, and robustness to out-of-distribution data. To the best of our knowledge, no prior work has investigated the implicit bias of gradient descent in this or other soft-label classification settings; thus, our results are of direct relevance to these contexts as well.



%In terms of our framing of \NTP training as supervised classification with a sparse probability vector $\ph_j$ associated with each (distinct) context $\hd_j$, this is resemeblent of classification with probabilistic- or soft- labels \cite{}. In prior literature this setting becomes relevant in modeling uncertainties on the labeling during crowdsourcing, where soft labels (aka frequencies) are formed by fusing multiple annotators' hard labels or by allowing each annotator to specify their own personal probability distribution over the labels. 


==> Arxiv_NewTempl/sections/ufm_do_not_upload.tex <==
% \section{UFM for NTP}



% \subsection{Logits}

\section{UFM \tina{remove}}
    
\subsubsection{Key logit matrices}

\begin{claim}\label{claim:conj}
    For the optimal solution of \eqref{eq:ufm-svm}, we have for all $j\in[m]$ that
    \begin{align*}
        \Lbmm [z,j] = \begin{cases}
            -{|\Sc_j|}/{V}, & z\not\in\Sc_j\,,\\
            {(V-|\Sc_j|)}/{V}, & z\in\Sc_j\,.
        \end{cases}
    \end{align*}
\end{claim}

\begin{definition} 
Define the \NTPH-logit matrix   $\Lbstar=\begin{bmatrix}
    \ellbb^\star_1 & \ellbb^\star_2 & \cdots & \ellbb^\star_m
\end{bmatrix}\in\R^{V\times m}$ as the matrix with columns
\[
\ellbb^\star_j = \Eb_j^\top(\Eb_j\Eb_j^\top)^{-1}\ab_j,\quad j\in[m].
\]
\end{definition}


\begin{lemma}
    The \NTPH-logit and \NTP-SVM logit matrices have mututally orthogonal columns, i.e.
    $\inp{\ellbbstar_j}{\ellbbmm_j}=0, \forall j\in[m].$ This in turn implies $\inp{\Lbstar}{\Lbmm}=0$.
\end{lemma}
\begin{proof}
    Fix any $j\in[m]$. By definition $\ellbbstar_j\in\Rc(\Eb_j^\top)$. Also, by feasibility (specifically \eqref{eq:Wmm condition equal}) in \eqref{eq:ufm-svm}, $\ellbbmm_j\in\Nc(\Eb_j)$. Thus, the desired follows since $\Nc(\Eb_j)\perp \Rc(\Eb_j^\top)$.
\end{proof}


% Let $\Omega=\{(v,j)\in[V]\times[m] \,:\, v\not\in\Sc_j\}$ denote the collection of pair of indices $(\text{word}=v,\text{context}=j)$  such that word $v\in\Vc$ is \emph{not} in the support set of context $j\in[m]$. Further define the operator 
% \[
% \Rc_\Omega(\M) = \sum_{(v,j)\in\Omega} (\eb_v^\top\M\eb_j)\, \eb_v\eb_j^\top\,.
% \]
% Observe that the $(v,j)$ entry of $\M$ is zero unless $(v,j)\in\Omega$. It is easy to see by definition of each column of $\Lstar$ with respect to the matrix $\Eb_j^\top$ that 
% \[
% \Rc_\Omega(\Lbstar) = 0.
% \]


For matrix $\Ab$, let $\Qc_\Omega(\Ab):=\Qc_{\{\Sc_1,\ldots,\Sc_m\}}(\Ab)$ denote a matrix that project each column $\ab_j$ of $\Ab$ onto $\Rc(\Eb_j^\top)$, i.e. $\Qc_\Omega(\Ab)_j=\Eb_j^\top(\Eb_j\Eb_j^\top)^{-1}\Eb_j\ab_j$. Observe that
\[
\Qc_\Omega(\Lbstar)=\Lbstar\qquad\text{and}\qquad\Qc_\Omega(\Lbmm)=0\,.
\]

\begin{lemma}
    $\Lbstar$ has rank at most $V-1$ since $\ones^\top \Lbstar=0$.
\end{lemma}

\begin{lemma} \red{wrong}
    $\Lbstar$ has rank $V-1$ provided that for each token $v\in \Vc$, there exists context $j\in[m]$ with $S_j>2$ such that $v\in\Sc_j$.
\end{lemma}
Onwards, let's assume \footnote{this is merely for simplicity and we should be able to extend to the general case. In any case, the assumption is only very mild.} that the condition of the previous lemma holds. Thus, the column span of $\Lbstar$ is the space orthogonal to $\ones_V$.


\subsubsection{Solution to \eqref{eq:ufm}}

\ct{I want to state part B of this theorem more generally where for $d<V-1$ there is additional rank constraint $\rank{\Vb}\leq d$ in \eqref{eq:ufm-svm}.} \ct{But is this feasible?}

\begin{theorem}
    Denote $\hat\Lb_\la$ the solution of \eqref{eq:ufm relax} for regularization $\la$. Further let $\Lbo_\la:=\frac{\hat\Lb_\la}{\|\hat\Lb_\la\|_*}$. In the limit of vanishing regularization the following are true:
    \begin{enumerate}
        \item Firstly,
         \[
        \lim_{\la\rightarrow0} \Qc_\Omega(\hat\Lb_\la) = \Lbstar
        \]   
        \item Secondly, $\lim_{\la\rightarrow0} \|\hat\Lb_\la\| = +\infty$, and, \footnote{If \eqref{eq:ufm-svm} does not have unique minimum (note objective is not strictly convex) then the claim of the theorem is to be understood as that $\Lbo_\la$ converges to the optimal set of \eqref{eq:ufm-svm}.}
        \[
        \lim_{\la\rightarrow0}\,\Lbo_\la = \overline\Lbmm.
        \]
        \end{enumerate}

        
\end{theorem}

\begin{proof}
    Proof should not be too difficult an extension of linear case. Consider constrained instead of regularized version.
\end{proof}

% \begin{remark}
   The first statement of the theorem guarantees the following that for  all $j\in[m], z\neq z'\in\Sc_j$:
        \[
        \lim_{\la\rightarrow0}\,\hat\Lb_\la[z,j]-\hat\Lb_\la[z',j] = \log\left(\frac{\pih_{j,z}}{\pih_{j,z'}}\right)\,.
        \]
% \end{remark}

More importantly, by combining the two statements of the theorem and recalling that $\Qc_\Omega(\Lbmm)=0$, implies the following approximation for $\hat\Lb_\la$ in the vanishing regularization regime:
\[
\hat\Lb_\la \approx \Lbstar + R_\la \Lbmm,
\]
for a growing $R_\la\rightarrow\infty$ as $\la\rightarrow0$. 

Denote $\Lbmm=\Umm\Smm\Vmmt$ the SVD of $\Lbmm$ and let $\Vmm_\perp$ be a basis to the orthogonal complement of $\Rc(\Vmm)$, i.e. $\Vmmt_\perp\Vmm_\perp=\Id_m$ and $\Vmmt_\perp\Vmm=0$. With this, we can rewrite this approximation as
\[
\hat\Lb_\la \approx \Lbstar\Vmm_\perp\Vmmt_\perp + R_\la \Lbmm,
\]
where we ignored the component of $\hat\Lb_\la$ that is on the same space of $\Lbmm$ since it will be dominated by $R_\la \Lbmm$ for large $R_\la$\footnote{Here, I am assuming that $\Rc(\Ustar)=\Rc(\Umm)=\ones^\perp$. This holds when $m>V$ and the condition of Lemma 4 holds. We can relax this.}.
Note now that the two compoents above belong in orthogonal row spaces.

\subsection{Decoder and Embeddings}
Based on the above, we make the following conjecture. Let $\Util\Stil\Vtilt$ denote the SVD of $\Lbstar\Vmm_\perp\Vmmt_\perp=\Lbstar(\Id_m-\Vmm\Vmmt)$. Further let $\Pbmm=\Vmm\Vmmt$ denote the projection on the subspace $\Rc(\Vmm)$. Finally, let $\Pbmm_\perp$ denote projection to its complement. Finally, write $\Ab\propto\M$ to denote $\overline\Ab=\overline\M$.

\begin{claim} Suppose $d=m\geq V$ \ct{this is  restrictive (particularly the requirement $d\geq m$ -- for simplicity, equality) but in that case I believe we could split $W,\Hb$ in its projections}
Let any solution $(\What_\la,\Hbhat_\la)$ of \eqref{eq:ufm}.
In the limit of vanishing regularization it satisfies the following:
\begin{enumerate}
    \item $\lim_{\laz} \|\What_\la\Pbmm\|=\infty$ and $\lim_{\laz} \What_\la\Pbmm \propto \Umm\sqrt{\Smm}\Vmmt$
    \item $\lim_{\laz} \What_\la\Pbmm_\perp=\Util\sqrt{\Stil}\Vtilt$
    \item $\lim_{\laz} \|\Pbmm\Hbhat_\la\|=\infty$ and $\lim_{\laz} \Pbmm\Hbhat_\la\propto \Vmm\sqrt{\Smm}\Vmmt$
    \item $\lim_{\laz} \Pbmm_\perp\Hbhat_\la=\Vtil\sqrt{\Stil}\Vtilt$
\end{enumerate}
\end{claim}






% Let SVD of the max-margin logit matrix $\Lbmm=\Ub\Sigmab\Vb^\top$. Then, \textbf{assuming $d>V$ (for now)} we claim that any solution of \eqref{eq:ufm} in the limit of vanishing regularization satisfies:
% \begin{enumerate}
%     \item $\W\W^\top=\Ub\Sigmab\Ub^\top$
%     \item $\Hb^\top\Hb=\Vb\Sigmab\Vb^\top$
%     \item $\W\Hb=\Ub\Sigmab\Vb^\top$
% \end{enumerate}
% \ct{there is something missing with this conjecture? How do we ensure $\NTP_\ent$-compatibility?}

% \ct{Question \#1:} It might not be possible to obtain the solution to \eqref{eq:ufm-svm} in closed form in general. However, this might be absolutely doable if we impose some further symmetry. The first thing is to assume support-set of fixed sizes $S_j=|\Sc_j|=S$ for all $j\in[m]$.  




\begin{claim}[(informal) NTP-UFM -- V2]
    Assume \tina{$d>V-1$}.
    Let $\Lbmm$ be the \ct{unique?} solution of \eqref{eq:ufm-svm} with SVD $\Lbmm=\Ub\Sigmab\Vb^\top$. ($\Ub\in\R^{V\times \red{(V-1)}}, \Sigmab\in\R^{\red{(V-1)}\times \red{(V-1)}}, \vb\in\R^{m \times \red{(V-1)}}$). For some partial orthonormal $\Rb\in\R^{\red{(V-1)\times d}}$, the following statements hold.
    \begin{enumerate}
        \item Let $\Hmm := \Rb^\top\Sigmab^{\frac{1}{2}}\Vb$,
        \begin{align*}
                        \lim_{\la\to0} \frac{\hat\Hb_\la}{\norm{\hat\Hb_\la}} = \frac{\Hmm}{\norm{\Hmm}}
        \end{align*}
            \item For $\Fcmm=\rm{span}\big(\big\{(\eb_z-\eb_{z'})\hb_{\rm{mm},j}^\top\,:\,z\neq z'\in\Sc_j, j\in[m]\big\}\big)$, $\|\Pc_\perp(\What_\la)\|\rightarrow\infty$ and 
        \begin{align*}
            \Pc_{\Fcmm}(\hat\W_\la) = \W^{\rm{mm},p},
        \end{align*}
        where $\W^{\rm{mm},p}$ is the unique solution in $\Fcmm$ such that 
        \begin{align*}
            \forall j\in[m],\, z\neq z'\in\Sc_j,\quad (\eb_z-\eb_{z'})^\top\W^p\hb_{\rm{mm},j} = \log\big(\hat p_{j,z}/\hat p_{j,z'}\big)
        \end{align*}
        Further, for $\Wmm := \Ub\Sigmab^{\frac{1}{2}}\Rb$,
        \begin{align*}
                        \lim_{\la\to0} \frac{\hat\W_\la}{\norm{\hat\W_\la}} = \frac{\Wmm}{\norm{\Wmm}}
        \end{align*}
    \end{enumerate}
\end{claim}


% \begin{claim}
%     Assume \tina{$d>V-1$}.
%     Let $\Lbmm$ be the \ct{unique?} solution of \eqref{eq:ufm-svm} with SVD $\Lbmm=\Ub\Sigmab\Vb^\top$. Define $\Wmm$ and $\Hmm$ such that  $\W\W^\top=\Ub\Sigmab\Ub^\top$ and $\Hb^\top\Hb=\Vb\Sigmab\Vb^\top$. In the limit of vanishing regularization for the \eqref{eq:ufm}, we have
%     \begin{enumerate}
%         \item \begin{align}
%             \lim_{\la\to0} \frac{\hat\Hb_\la}{\norm{\hat\Hb_\la}} = \frac{\Hmm}{\norm{\Hmm}}
%         \end{align}
%         \item Define the subspace $\Fc = \text{span}\{(\e_z-\e_{z'})\bar\hb_{\text{mm},j}^\top:\,z\neq z'\in\Sc_j,\,j\in[m]\}$ and let $\W^*$ be the unique solution of the \NTPH-compatibility conditions restricted to subspace $\Fc$. Then,
%         \begin{align*}
%             \lim_{\la\to0} \frac{\hat\W_\la - \W^*}{\norm{\hat\W_\la - \W^*}} = \frac{\Wmm}{\norm{\Wmm}}
%         \end{align*}
%         \ct{Can you also write this as:
%         $\Pc_\Ts(\What_\la)=\W^*$,  $\|\Pc_\perp(\What_\la)\|\rightarrow\infty$ and \[\lim_{\la\to0} \frac{\hat\W_\la}{\norm{\hat\W_\la}} = \frac{\Wmm}{\norm{\Wmm}}
%         \]
%         }
%         \tina{more accurate if written down based on gram matrices. rotation doesn't change the loss. fix!}
%     \end{enumerate}
% \end{claim}

% \subsection{proof -- dual problem}
% Consider the non-convex UFM-SVM below:
% \begin{align*}
%     \min_{\W,\Hb} \frac{1}{2}\norm{\W}_F^2 + \frac{1}{2}\norm{\Hb}_F^2, \quad \text{s.t.} \quad \forall j\in[m], z\neq z'\in\Sc_j~&:~~(\eb_z-\eb_{z'})^\top\W \hb_j =0\,
%         \\
%         \forall j\in[m], v\notin\Sc_j~&:~~(\eb_z-\eb_{v})^\top\W \hb_j \geq 1\,.
% \end{align*}

% For each sample $j$, choose an anchor label $z_j\in\Sc_j$. We can equivalently write the above program as 
% \begin{align*}
%     \min_{\W,\Hb} \frac{1}{2}\norm{\W}_F^2 + \frac{1}{2}\norm{\Hb}_F^2, \quad \text{s.t.} \quad \forall j\in[m], z_j\neq z\in\Sc_j~&:~~(\eb_{z_j}-\eb_{z'})^\top\W \hb_j =0\,
%         \\
%         \forall j\in[m], v\notin\Sc_j~&:~~(\eb_{z_j}-\eb_{v})^\top\W \hb_j \geq 1\,.
% \end{align*}

% Define $\Xb = \begin{bmatrix}
%     \W\\
%     \Hb^\top
% \end{bmatrix}\begin{bmatrix}
%     \W^\top & \Hb
% \end{bmatrix}$ and consider the following convex relaxation of the above program
% \begin{align*}
%     \min_{\Xb\succcurlyeq0}\,\, \frac{1}{2}\tr(\Xb)\quad \text{s.t.}\quad \forall j\in[m], z_j\neq z\in\Sc_j~&:~~\Xb[z_j,V+j] - \Xb[z',V+j] =0\,
%         \\
%         \forall j\in[m], v\notin\Sc_j~&:~~\Xb[z_j,V+j] - \Xb[v,V+j] \geq 1\,. 
% \end{align*}

% Define $\Ab_{V\times m}$ such that $\Ab[z,j] = -\lambdab_{j,z},\,z\neq z_j$ and $\Ab[z_j,j] = \sum_{z\neq z_j}\lambdab_{j,z}$. ($\oneb_V^\top\Ab=0$).

% The dual problem is 
% \begin{align*}
% &
% \max_{\Ab} \,\min_{\Xb\succcurlyeq0} \,\sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} + \frac12\tr\bigg(\begin{bmatrix}
%     \Id & -\Ab\\
%     -\Ab^\top & \Id 
% \end{bmatrix}\Xb\bigg)\,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad \Ab_{j,v}\leq0,\,v\not\in\Sc_j\\
% &\max_{\Ab} \,\sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} \,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad \red{\Ab_{j,v}\leq0,\,v\not\in\Sc_j},\quad \norm{\Ab}_2\leq 1\\
% &\max_{\Ab} \,\,\tr(\Ab^\top\Lbmm) \,\quad\text{s.t.}\quad \oneb_V^\top\Ab=0 \quad \red{\Ab_{j,v}\leq0,\,v\not\in\Sc_j},\quad \norm{\Ab}_2\leq 1
% \end{align*}
% \tina{for $|\Sc_j|=1$ boils down to $\Ab \odot \Lbmm \geq 0$ similar to what we had before.}
% % 
% Last line holds since,
% \begin{align*}
%     \sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} &= \sum_{j\in[m]}\sum_{v\not\in\Sc_j}\lambdab_{j,v} + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v} - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
%     &= \sum_{j\in[m]}\sum_{v\neq z_j}\lambdab_{j,v} - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
%     &= \sum_{j\in[m]} (\frac{1-|\Sc_j|}{V} + \frac{|\Sc_j|}{V}) \sum_{v\neq z_j}\lambdab_{j,v}  - \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\lambdab_{j,v}\\
%     &= \sum_{j\in[m]} \frac{1-|\Sc_j|}{V} \Ab[z_j,j] - \sum_{j\in[m]} \frac{|\Sc_j|}{V} \sum_{v\neq z_j} \Ab[v,j] + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\Ab[v,j]\\
%     &= \sum_{j\in[m]} \Lbmm[z_j,j] \Ab[z_j,j] + \sum_{j\in[m]} \sum_{v\not\in\Sc_j} \Lbmm[v,j]  \Ab[v,j] + \sum_{j\in[m]}\sum_{\substack{v\in\Sc_j \\ v\neq z_j}}\Lbmm[v,j] \Ab[v,j]\\
%     &=\sum_{j\in[m]} \sum_{v\in[V]}\Lbmm[v,j] \Ab[v,j]
% \end{align*}


% \begin{proposition}\label{propo:svm sufficient condition}
%     Let $\Lbmm=\Ub\Sigmab\Vb^\top$ be the SVD of $\Lbmm$ and define $\bar{\Ab}:=\Ub\Vb^\top$. If $\forall j \in [m]$, $v\not\in\Sc_j$,  we have  $\Ab_{j,v}\leq0,\,$, Then, 
% \end{proposition}


\subsection{Logit matrix factorization}
\ct{this section will be removed. please ignore}
% \begin{lemma}
    Suppose $d>2V$. Let $\Lbin=\Ub_1\Sigmab_1\Vb_1^\top$ be the SVD of $\Lbin$. Denote $r:=\rank{\Lbmm}$ and $r_1:=\rank{\Lbin}$. Let $\Qb\in\R^{d\times r}$ and $\Qb_\perp\in\R^{d\times r_1}$ be partial orthonormal matrices with mutually orthogonal columns, i.e. $\Qb^\top\Qb=\Id_r$, $\Qb_\perp^\top\Qb_\perp=\Id_{r_1}$, and $\Qb^\top\Qb_\perp=0, \Qb_\perp^\top\Qb=0$. (It is always possible to select such $\Qb_1,\Qb_2$ since $d\geq2V\geq r_1+r$.) With these define,
    \begin{align}
    \W&:=\Ub_1\sqrt{\Sigmab_1}\Qb_\perp^\top + \sqrt{R}\cdot\Ub\sqrt{\Sigmab}\Qb^\top
    \\
    \Hb&:=\Qb_\perp\sqrt{\Sigmab_1}\Vb_1^\top + \sqrt{R}\cdot\Qb\sqrt{\Sigmab}\Vb^\top
    \end{align}
% \end{lemma}

Note then that
\[
\W\Hb = \Lbin + R\cdot\Lbmm\,.
\]
Additionally,
\begin{align}
    \GW&:=\Ub_1\Sigmab_1\Ub_1^\top + R\cdot\Ub\Sigmab\Ub^\top
    \\
    \GH&:=\Vb_1\Sigmab_1\Vb_1^\top + R\cdot\Vb\Sigmab\Vb^\top
    \end{align}

Let now $\Pbb_{\Ub}^\perp=\Ub_\perp\Ub_\perp^\top$  denote projection matrix to the orthogonal complement of column space of $\Ub$. Similarly, define projections for $\Vb.$

As $R\rightarrow\infty$, we have the following properties:
\[
\overline\GW\propto \Ub\Sigmab\Ub^\top 
\]
and
\begin{align}
\GW\Pbb_{\Ub}^\perp &= \Ub_1\Sigmab_1\Ub_1^\top\Pbb_{\Ub}^\perp
\\
\Pbb_{\Ub}^\perp\GW &= \Pbb_{\Ub}^\perp\Ub_1\Sigmab_1\Ub_1^\top
\\
\Pbb_{\Ub}^\perp\GW\Pbb_{\Ub}^\perp &= \Pbb_{\Ub}^\perp\Ub_1\Sigmab_1\Ub_1^\top\Pbb_{\Ub}^\perp
\end{align}
Similarly,
\[
\overline\GH\propto \Vb\Sigmab\Vb^\top 
\]
and
\begin{align}
\GW\Pbb_{\Vb}^\perp &= \Vb_1\Sigmab_1\Vb_1^\top\Pbb_{\Vb}^\perp
\\
\Pbb_{\Vb}^\perp\GW &= \Pbb_{\Vb}^\perp\Vb_1\Sigmab_1\Vb_1^\top
\\
\Pbb_{\Vb}^\perp\GW\Pbb_{\Vb}^\perp &= \Pbb_{\Vb}^\perp\Vb_1\Sigmab_1\Vb_1^\top\Pbb_{\Vb}^\perp
\end{align}


\subsubsection{Again}
Let $\Lbmm=\Ub\Sigmab\Vb$. Let $\Pbb_{\Ub}^\perp=\Ub_\perp\Ub_\perp^\top$  denote projection matrix to the orthogonal complement of column space of $\Ub$. Also $\Pbb_U=\Ub\Ub^\top$ the projection to $\Ub$. Thus, $\Pbb_U^\perp=\Id_V-\Pbb_U$ Similarly, define projections for $\Vb.$
Finally, define the orthogonal decomposition 
\[
\R^{V\times m}=\Tc\bigoplus\Tc^\perp
\]
 where $\Tc$ is the set of matrices spanned by $\ub\vb^\top$. The projections to the two spaces are given as
 \[
 \Pbb_{\Tc}(\A)=\Pbb_U\A\Pbb_V\,.
 \]
 and
 \[
 \Pbb_{\Ts^\perp}(\A):=\Pbb_{\perp}(\A)=\Pbb_U^\perp\A+\A\Pbb_V^\perp-\Pbb_U^\perp\A\Pbb_V^\perp\,
 \]

 \noindent\textbf{Claim:} In the limit of vanishing regularization, the logit matrix satisfies
 \[
  \|\Pbb_\Ts(\Lb)\|\rightarrow\infty \qquad\text{and}\qquad\Pbb_\Ts(\Lb)\propto\Lbmm
 \]
 \[
  \Pbb_\perp(\Lb)\rightarrow \Lbstar= \ct{???}.
 \]
 
 Then, defining SVD $\Lbstar=\Ub_1\Sigmab_1\Vb_1^\top$ the $\W,\Hb$ decomposition is as follows:
 \begin{align}
    \GW&:=\Ub_1\Sigmab_1\Ub_1^\top + R\cdot\Ub\Sigmab\Ub^\top
    \\
    \GH&:=\Vb_1\Sigmab_1\Vb_1^\top + R\cdot\Vb\Sigmab\Vb^\top
    \end{align}
 or
 \begin{align}
    \GW^*:=(\Id_V-\Ub\Ub^\top)\GW(\Id_m-\Ub\Ub^\top)&:=\Ub_1\Sigmab_1\Ub_1^\top \quad\text{and}\quad (\GW-\GW^*) \propto \Ub\Sigmab\Ub^\top
    \\
    \GH^*:=(\Id_V-\Vb\Vb^\top)\GH(\Id_m-\Vb\Vb^\top)&:=\Vb_1\Sigmab_1\Vb_1^\top \quad\text{and}\quad (\GH-\GH^*) \propto \Vb\Sigmab\Vb^\top
    \end{align}


\subsubsection{Lessons 03/27}

It seems that what we predict is $\Lb_\la$ on the subspace of $\Lbmm$, i.e. on the subspace $\Tc$. Indeed, the error of $\Pbb_\Tc(\Lb_\la-\Lbin)$ to $\Lbmm$ is small, but the component $\Pbb_\perp(\Lb_\la)$ is non-zero. One would hope that this component is equal to $\Pb_\perp(\Lbin)$ but this is not the case. So there is a component of $\Lb_\la$ that we are missing. I suspect this component is coming because to the finite part $\Lbin$, we can in principle add anything that is arbitrary (but finite) on the off-support, i.e. the finite part is $\Lbin$ plus something that is on;y active on the off-support. Then, the part that we are missing from the description of $\Lb_\la$ is $\Pb_\perp(\Lbin+\text{that something}).$





